When Automated Program Repair Meets Regression Testing -- An Extensive Study on 2 Million Patches

In recent years, Automated Program Repair (APR) has been extensively studied in academia and even drawn wide attention from industry. However, APR techniques can be extremely time consuming since (1) a large number of patches can be generated for a given bug, and (2) each patch needs to be executed on the original tests to ensure its correctness. In the literature, various techniques (e.g., based on learning, mining, and constraint solving) have been proposed/studied to reduce the number of patches. Intuitively, every patch can be treated as a software revision during regression testing; thus, traditional Regression Test Selection (RTS) techniques can be leveraged to only execute the tests affected by each patch (as the other tests would keep the same outcomes) to further reduce patch execution time. However, few APR systems actually adopt RTS and there is still a lack of systematic studies demonstrating the benefits of RTS and the impact of different RTS strategies on APR. To this end, this paper presents the first extensive study of widely-used RTS techniques at different levels (i.e., class/method/statement levels) for 12 state-of-the-art APR systems on over 2M patches. Our study reveals various practical guidelines for bridging the gap between APR and regression testing.

==> newrq/rq6.tex <==
\subsection{\yiling{RQ4: Impact of Test Reduction}}~\label{sec:rq_reduction}
\yiling{
So far, we have applied RTS and prioritization techniques based on the whole original test suite, which is shown to be a \textit{safe} way for   APR acceleration without any sacrifice of accuracy, i.e., the repair results remain consistent with/without adopting these regression testing techniques. Besides RTS and prioritization, regression test reduction~\cite{} is another category of regression testing optimization techniques, which has been widely adopted to accelerate regression testing in practice. Generally speaking, regression test reduction aims to find a subset of the original test suite according to certain testing requirements, such as structural coverage~\cite{}. The redundant test cases would be removed and only the remaining tests would be executed then. Existing studies in regression testing scenario have shown that regression test reduction can effectively reduce the size of the regression test suite without substantially reducing its fault-detection capability~\cite{}, and combining RTS and test reduction can enable more significant acceleration.
In this RQ, we make the first attempt to investigate the impact of regression test reduction on the efficiency and the accuracy of APR. 
In particular, for each buggy version, we first perform once test reduction to reduce the size of its original test suite, and for each patch we then apply RTS on the reduced test suite to select the test cases for execution.
We study the traditional greedy reduction algorithm~\cite{} with the coverage requirement, since it is one of the  most widely-used and effective reduction techniques as suggested by previous work~\cite{}. 
Note that we still control all selected tests executed in the default order (i.e., all the originally-failed tests are executed before all the originally-passed tests, and within them all tests are executed in the lexicographic order). 


Table~\ref{} presents the results of 

}


==> newtables/aprinfo.tex <==

\begin{table}[htb]
    \small
    \centering
    \caption{Studied APR systems}\label{tab:aprtools}
    	\begin{adjustbox}{width=\columnwidth}
    \begin{tabular}{|l|l|}
        \cline{1-2}
         \textbf{Tool Category} & \textbf{Tools} \\
         \hline \hline
        Constraint-based & \acs{}\cite{DBLP:conf/icse/XiongWYZH0017/acs},    \dynamoth{}\cite{DBLP:conf/icse/DurieuxM16/dynamoth}  \\          \hline
         Heuristic-based & \arja\cite{DBLP:journals/tse/YuanB20/arja},    \genprog{}\cite{DBLP:journals/tse/YuanB20/arja},  \kali{}\cite{DBLP:journals/tse/YuanB20/arja}, 
        RSRepair-A\cite{DBLP:journals/tse/YuanB20/arja}, 
         \simfix{}\cite{DBLP:conf/issta/JiangXZGC18} \\          \hline
         Template-based & \avatar{}\cite{DBLP:conf/wcre/LiuK0B19/avatar},    \fixminer{}\cite{DBLP:journals/ese/KoyuncuLBKKMT20/fixminer},  \kpar{}\cite{DBLP:conf/icst/LiuKB0KT19/kpar},  \prapr{}\cite{DBLP:conf/issta/GhanbariBZ19},
         \tbar{} \cite{DBLP:conf/issta/LiuK0B19/tbar} \\
                  \hline
    \end{tabular}
    	\end{adjustbox}
\end{table}




==> newtables/newrq_time_metric.tex <==
\begin{comment}
\begin{table}[htb]
    \centering
   \caption{Reduction of test execution time by different RTS strategies}\label{table:cmp_time}

   	\begin{adjustbox}{width=0.8\columnwidth}
    \begin{tabular}{|r|l||rrr|}

    \hline
    
    \textbf{Subject} &  \textbf{RTS Strategy} &  \textbf{\prapr{}} &  \textbf{\simfix{}} & \textbf{\acs{}} \\ \hline \hline
\multirow{8}{*}{Lang} & \#Patch&394.29&275.98&1.00\\
 & \#Test (\norts{})&153,858.02&93,263.22&6,574.80\\
 & \#Test (\rtsclass{})&116,844.34&8,993.52&575.80\\
 & CLASS&33.02\%&37.66\%&52.08\%\\ 
 & \#Test (\rtsmethod{})&115,589.76&8,430.00&2.40\\
 & METHOD&35.09\%&38.93\%&60.00\%\\ 
 & \#Test (\rtsstate{})&115,546.51&8,429.47&2.40\\ \hline
 & ST&35.16\%&38.93\%&60.00\%\\ 
\multirow{8}{*}{Math} & \#Patch&1,891.18&469.45&1.00\\
 & \#Test (\norts{})&1,129,654.75&352,727.61&56,458.83\\
 & \#Test (\rtsclass{})&120,336.31&68,790.68&9,469.17\\
 & CLASS&49.18\%&56.73\%&91.03\%\\ 
 & \#Test (\rtsmethod{})&52,899.96&24,346.36&51.17\\
 & METHOD&52.44\%&63.78\%&99.70\%\\ 
 & \#Test (\rtsstate{})&49,854.26&23,484.15&31.83\\ \hline
 & ST&52.77\%&63.88\%&99.74\%\\ 
\multirow{8}{*}{Time} & \#Patch&2,017.27&396.50&1.00\\
 & \#Test (\norts{})&41,191.96&44,882.04&3,668.00\\
 & \#Test (\rtsclass{})&19,435.08&20,562.21&3,264.00\\
 & CLASS&32.34\%&26.31\%&11.01\%\\ 
 & \#Test (\rtsmethod{})&11,945.23&7,284.42&10.00\\
 & METHOD&46.13\%&39.89\%&99.73\%\\ 
 & \#Test (\rtsstate{})&11,745.04&7,243.04&7.00\\ \hline
 & ST&46.27\%&39.93\%&99.81\%\\ 
\multirow{8}{*}{Chart} & \#Patch&841.44&588.21&-\\
 & \#Test (\norts{})&39,299.96&58,345.12&-\\
 & \#Test (\rtsclass{})&6,278.36&39,192.88&-\\
 & CLASS&49.53\%&33.83\%&-\%\\ 
 & \#Test (\rtsmethod{})&4,434.96&37,390.50&-\\
 & METHOD&51.64\%&36.56\%&-\%\\ 
 & \#Test (\rtsstate{})&4,261.92&37,384.58&-\\ \hline
 & ST&51.96\%&36.56\%&-\%\\ 
\multirow{8}{*}{Closure} & \#Patch&19,365.13&511.03&-\\
 & \#Test (\norts{})&1,102,244.42&550,033.27&-\\
 & \#Test (\rtsclass{})&659,598.94&268,023.56&-\\
 & CLASS&18.79\%&17.75\%&-\%\\ 
 & \#Test (\rtsmethod{})&453,154.02&196,204.06&-\\
 & METHOD&35.41\%&27.58\%&-\%\\ 
 & \#Test (\rtsstate{})&416,499.78&156,750.72&-\\ \hline
 & ST&39.85\%&29.37\%&-\%\\ 
\multirow{8}{*}{Mockito} & \#Patch&2,549.29&-&-\\
 & \#Test (\norts{})&58,223.60&-&-\\
 & \#Test (\rtsclass{})&41,444.49&-&-\\
 & CLASS&12.61\%&-\%&-\%\\ 
 & \#Test (\rtsmethod{})&25,467.77&-&-\\
 & METHOD&26.21\%&-\%&-\%\\ 
 & \#Test (\rtsstate{})&21,014.09&-&-\\ \hline
 & ST&30.44\%&-\%&-\%\\ 
\multirow{8}{*}{Average} & \#Patch&4,509.76&448.23&1.00\\
&\#Test (\norts{})&420,745.45&219,850.25&22,233.88\\
&\#Test (\rtsclass{})&160,656.25&81,112.57&4,436.32\\
&\%&32.58&34.46&51.38\\
&\#Test (\rtsmethod{})&110,581.95&54,731.07&21.19\\
&\%&41.15&41.35&86.48\\
&\#Test (\rtsstate{})&103,153.60&46,658.39&13.74\\
&\%&42.74&41.73&86.52\\



    \end{tabular}
    \end{adjustbox}
    
\end{table} 
\end{comment}

\begin{table}[htb]
    \centering
   \caption{\yiling{Reduction: execution time v.s. \#test executions} \\ \todo{Change it into bar-plot}}\label{table:cmp_time}
   	\begin{adjustbox}{width=1\columnwidth}
    \begin{tabular}{|r|l||rr|rr|rr|}

    \hline
    
\textbf{Subject} &  \textbf{RTS Strategy} &  \multicolumn{2}{c}{\textbf{\prapr{}}} &   \multicolumn{2}{c}{\textbf{\simfix{}}} &  \multicolumn{2}{c|}{\textbf{\acs{}}} \\ \hline \hline

\multirow{3}{*}{Lang}& \rtsclass{}&33.02\% & 33.33\% &30.20\%&35.66\%&52.08\%&56.37\%\\
& \rtsmethod{}&35.09\% & 34.51\% &31.19\%&36.31\%&60.00\%&59.94\%\\
& \rtsstate{}&35.16\% & 34.55\% &31.19\%&36.31\%&60.00\%&59.97\%\\
  \hline\multirow{3}{*}{Math}& \rtsclass{}&49.18\% &48.91\% &46.65\%&52.45\%&90.83\%&90.59\%\\
& \rtsmethod{}&52.44\% &50.41\% &51.35\%&55.81\%&99.60\%&98.86\%\\
& \rtsstate{}&52.77\% &50.50\% &51.41\%&55.89\%&99.66\%&99.63\%\\
  \hline\multirow{3}{*}{Time}& \rtsclass{}&32.34\% &31.25\% &22.18\%&29.42\%&11.01\%&47.56\%\\
& \rtsmethod{}&46.13\%&40.12\% &26.53\%&35.60\%&99.73\%&98.66\%\\
& \rtsstate{}&46.27\% &40.31\% &26.54\%&35.60\%&99.81\%&99.31\%\\
  \hline\multirow{3}{*}{Chart}& \rtsclass{}&49.53\% &58.50\% &28.64\%&33.16\%&&\\
& \rtsmethod{}&51.64\%&62.45\% &30.95\%&34.67\%&&\\
& \rtsstate{}&51.96\% &62.52\% &30.95\%&34.67\%&&\\
  \hline\multirow{3}{*}{Closure}& \rtsclass{}&18.79\% &31.73\% &13.22\%&20.27\%&&\\
& \rtsmethod{}&35.41\%&46.18\% &21.15\%&30.51\%&&\\
& \rtsstate{}&39.85\% &51.80\% &22.16\%&32.01\%&&\\
  \hline\multirow{3}{*}{Mockito}& \rtsclass{}&12.61 &18.03\% &&&&\\
& \rtsmethod{}&26.21 &21.17\% &&&&\\
& \rtsstate{}&30.44 &21.30\% &&&&\\
  \hline\multirow{3}{*}{Average}&\rtsclass{}&32.58\% &36.96\% &28.18\%&34.19\%&51.31\%&64.84\%\\
& \rtsmethod{} & 41.15\% &42.47\% &32.23\%&38.58\%&86.44\%&85.82\%\\
&\rtsstate{}&42.74\% &43.50\% &32.45\%&38.90\%&86.49\%&86.30\%\\


\hline
    \end{tabular}
    \end{adjustbox}
    
\end{table} 



==> newtables/rq0_cmp_all_old.tex <==
\begin{table*}[htb]
    \centering
   \caption{Number of test executions among   APR systems}\label{table:rq0_cmpall}

   	\begin{adjustbox}{width=1.8\columnwidth}
    \begin{tabular}{|r|l||rrrrrrrrrrrr|}

    \hline
    
    \textbf{Subject} &  \textbf{RTS Strategy} &  \textbf{\prapr{}} &  \textbf{\simfix{}} &  \textbf{\avatar{}} &  \textbf{\kpar{}} &  \textbf{\tbar{}} &  \textbf{\fixminer{}} &  \textbf{\dynamoth{}} &  \textbf{\acs{}} &  \textbf{\arja{}} &  \textbf{\kali{}} &  \textbf{\genprog{}} &  \textbf{\rsrepair{}} \\ \hline \hline
    
    \multirow{5}{*}{Lang} & \#Patch&381.27&62.55&4.63&4.79&4.76&4.56&0.16&0.05&522.97&26.92&628.85&289.23\\
 & \#Test (\norts{})&2,117.61&424.75&321.41&163.19&437.52&233.15&1,256.86&608.00&68,448.64&799.43&86,910.25&10,945.44\\
 & \#Test (\rtsclass{})&447.31&85.96&19.48&18.30&24.63&18.88&25.71&17.00&1,571.25&59.54&2,746.19&620.69\\
 & \#Test (\rtsmethod{})&414.15&82.38&12.11&11.89&12.63&11.88&2.86&1.00&1,196.83&51.54&1,376.81&556.39\\
 & \#Test (\rtsstate{})&412.59&82.21&11.44&11.59&11.96&11.50&2.00&1.00&1,176.53&50.63&1,369.64&534.58\\ \hline
\multirow{5}{*}{Math} & \#Patch&1,483.12&30.87&5.84&5.12&5.01&4.76&0.23&0.05&804.09&10.11&858.19&411.58\\
 & \#Test (\norts{})&11,879.77&1,185.13&168.78&237.05&640.65&239.38&2,042.74&789.33&104,804.90&705.64&73,174.10&9,661.55\\
 & \#Test (\rtsclass{})&1,711.16&158.06&12.92&46.66&34.66&9.47&50.79&6.33&4,828.21&22.00&5,231.08&828.93\\
 & \#Test (\rtsmethod{})&1,573.21&56.41&8.20&7.25&8.18&7.03&32.53&6.33&2,105.64&15.97&1,610.38&498.28\\
 & \#Test (\rtsstate{})&1,557.41&55.59&7.81&6.86&7.25&6.23&27.00&1.67&1,382.11&14.10&1,419.85&463.63\\ \hline
\multirow{5}{*}{Time} & \#Patch&1,466.54&22.81&2.50&2.00&2.23&1.08&0.23&0.04&335.92&13.23&380.62&107.46\\
 & \#Test (\norts{})&7,782.19&768.55&1,065.00&4.73&359.09&490.00&1,303.67&1.00&34,310.82&724.00&141,456.00&2,652.50\\
 & \#Test (\rtsclass{})&2,513.88&184.27&232.55&4.73&80.82&107.38&537.33&1.00&7,337.91&325.70&29,401.40&635.00\\
 & \#Test (\rtsmethod{})&1,848.62&58.64&9.73&4.73&6.55&5.25&8.67&1.00&3,822.82&55.30&10,596.50&413.90\\
 & \#Test (\rtsstate{})&1,808.12&56.64&9.73&4.73&6.55&5.25&8.67&1.00&1,781.91&38.50&1,903.60&291.50\\ \hline
\multirow{5}{*}{Chart} & \#Patch&784.88&62.96&5.00&4.56&4.40&4.48&0.40& - &627.76&42.36&729.72&333.16\\
 & \#Test (\norts{})&5,517.96&218.61&272.84&107.61&367.74&102.12&1,640.80&-&202,236.87&2,035.27&104,090.08&9,552.46\\
 & \#Test (\rtsclass{})&1,053.80&73.61&8.26&8.00&8.79&7.12&77.30&-&27,627.48&133.45&5,694.38&758.38\\
 & \#Test (\rtsmethod{})&868.24&72.65&6.89&6.89&6.37&6.59&16.70&-&6,853.48&61.45&2,645.12&450.67\\
 & \#Test (\rtsstate{})&863.96&72.65&6.89&6.89&6.37&6.59&16.30&-&2,356.57&56.82&1,746.42&386.71\\ \hline
\multirow{5}{*}{Closure} & \#Patch&14,725.00&4.30&2.96&2.61&2.94&0.42&-&-&-&-&-&-\\
 & \#Test (\norts{})&86,651.19&4,239.84&342.78&378.73&478.09&2.89&-&-&-&-&-&-\\
 & \#Test (\rtsclass{})&47,374.48&2,329.55&140.81&154.94&197.02&2.89&-&-&-&-&-&-\\
 & \#Test (\rtsmethod{})&28,476.71&449.64&6.17&9.90&6.67&2.89&-&-&-&-&-&-\\
 & \#Test (\rtsstate{})&21,825.07&166.45&4.49&3.92&4.40&2.89&-&-&-&-&-&-\\ \hline
\multirow{5}{*}{Mockito} & \#Patch&2,307.92& - &1.67&2.00&1.81&1.67&-&-&-&-&-&-\\
 & \#Test (\norts{})&3,753.19&-&267.75&41.27&200.27&4.62&-&-&-&-&-&-\\
 & \#Test (\rtsclass{})&2,857.81&-&97.56&26.00&146.47&4.62&-&-&-&-&-&-\\
 & \#Test (\rtsmethod{})&2,555.61&-&7.62&5.80&48.00&4.62&-&-&-&-&-&-\\
 & \#Test (\rtsstate{})&2,547.64&-&7.38&5.80&7.33&4.62&-&-&-&-&-&-\\ \hline
    \end{tabular}
    \end{adjustbox}
    
\end{table*} 





\begin{comment}
\multirow{5}{*}{Average} & \#Patch&3,524.79&30.58&3.77&3.51&3.52&2.83&0.26&0.03&572.69&23.16&649.35&285.36\\
&\#Test (\norts{})&19,616.99&1,367.37&406.43&155.43&413.89&178.69&1,561.02&466.11&102,450.31&1,066.08&101,407.61&8,202.99\\
&\#Test (\rtsclass{})&9,326.41&566.29&85.26&43.10&82.06&25.06&172.78&8.11&10,341.21&135.17&10,768.26&710.75\\
&\#Test (\rtsmethod{})&5,956.09&143.94&8.46&7.74&14.73&6.38&15.19&2.78&3,494.69&46.07&4,057.20&479.81\\
&\#Test (\rtsstate{})&4,835.80&86.71&7.96&6.63&7.31&6.18&13.49&1.22&1,674.28&40.01&1,609.88&419.11\\
\end{comment}

==> newtables/rq1_cmp_ratio_summary_old.tex <==


\begin{table*}
    \centering
   \caption{Reduction of test executions by different RTS strategies }\label{table:rq1_cmpnorts_ratio}

   	\begin{adjustbox}{width=1.8\columnwidth}
    \begin{tabular}{|r|r||rrrrrrrrrrrr|}
    %p{1.4cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}
    
    \hline
    
    \textbf{Subject} &  \textbf{RTS Strategy} &  \textbf{\prapr{}} &  \textbf{\simfix{}} &  \textbf{\avatar{}} &  \textbf{\kpar{}} &  \textbf{\tbar{}} &  \textbf{\fixminer{}} &  \textbf{\dynamoth{}} &  \textbf{\acs{}} &  \textbf{\arja{}} &  \textbf{\kali{}} &  \textbf{\genprog{}} &  \textbf{\rsrepair{}} \\ \hline \hline
    

\multirow{3}{*}{Lang} & \rtsclass{}&33.33\%&18.16\%&17.92\%&10.57\%&21.48\%&14.80\%&69.99\%&32.44\%&36.67\%&22.16\%&26.11\%&30.12\%\\
 & \rtsmethod{}&34.51\%&18.36\%&18.35\%&10.95\%&22.05\%&15.22\%&71.31\%&33.32\%&38.16\%&22.50\%&26.68\%&31.17\%\\
 & \rtsstate{}&34.55\%&18.37\%&18.40\%&10.99\%&22.09\%&15.26\%&71.36\%&33.32\%&38.17\%&22.52\%&26.70\%&31.20\%\\ \hline
\multirow{3}{*}{Math} & \rtsclass{}&48.91\%&29.72\%&5.46\%&5.36\%&19.91\%&8.63\%&92.17\%&33.12\%&38.66\%&16.44\%&28.77\%&31.73\%\\
 & \rtsmethod{}&50.41\%&33.03\%&6.27\%&6.30\%&21.08\%&8.99\%&93.06\%&33.12\%&40.16\%&16.79\%&30.16\%&32.44\%\\
 & \rtsstate{}&50.50\%&33.06\%&6.28\%&6.31\%&21.11\%&9.05\%&93.33\%&33.32\%&40.42\%&16.85\%&30.35\%&32.68\%\\ \hline
\multirow{3}{*}{Time} & \rtsclass{}&31.25\%&14.68\%&7.14\%&0.00\%&7.15\%&9.83\%&19.62\%&0.00\%&19.59\%&17.90\%&7.97\%&16.26\%\\
 & \rtsmethod{}&40.12\%&17.87\%&9.06\%&0.00\%&9.06\%&12.45\%&33.15\%&0.00\%&21.41\%&28.27\%&9.31\%&17.38\%\\
 & \rtsstate{}&40.31\%&17.92\%&9.06\%&0.00\%&9.06\%&12.45\%&33.15\%&0.00\%&22.60\%&29.01\%&9.93\%&18.01\%\\ \hline
\multirow{3}{*}{Chart} & \rtsclass{}&58.50\%&8.36\%&15.68\%&5.49\%&20.88\%&5.85\%&85.96\%&-&53.39\%&40.87\%&34.93\%&39.33\%\\
 & \rtsmethod{}&62.45\%&8.41\%&15.76\%&5.55\%&21.02\%&5.88\%&89.10\%&-&59.10\%&43.78\%&38.81\%&42.02\%\\
 & \rtsstate{}&62.52\%&8.41\%&15.76\%&5.55\%&21.02\%&5.88\%&89.12\%&-&59.67\%&44.10\%&39.22\%&42.45\%\\ \hline
\multirow{3}{*}{Closure} & \rtsclass{}&31.73\%&25.15\%&3.22\%&3.79\%&3.90\%&0.00\%&-&-&-&-&-&-\\
 & \rtsmethod{}&46.18\%&51.50\%&5.28\%&6.56\%&7.38\%&0.00\%&-&-&-&-&-&-\\
 & \rtsstate{}&51.80\%&55.28\%&5.30\%&6.65\%&7.42\%&0.00\%&-&-&-&-&-&-\\ \hline
\multirow{3}{*}{Mockito} & \rtsclass{}&18.03\%&-&21.10\%&2.77\%&5.49\%&0.00\%&-&-&-&-&-&-\\
 & \rtsmethod{}&21.17\%&-&30.69\%&6.43\%&14.82\%&0.00\%&-&-&-&-&-&-\\
 & \rtsstate{}&21.30\%&-&30.72\%&6.43\%&19.67\%&0.00\%&-&-&-&-&-&-\\ \hline
\multirow{3}{*}{Average} & \rtsclass{}&36.96\%&19.21\%&11.75\%&4.66\%&13.13\%&6.52\%&66.93\%&21.85\%&37.08\%&24.34\%&24.45\%&29.36\%\\
&\rtsmethod{}&42.47\%&25.84\%&14.23\%&5.96\%&15.90\%&7.09\%&71.66\%&22.15\%&39.71\%&27.83\%&26.24\%&30.75\%\\
&\rtsstate{}&43.50\%&26.61\%&14.25\%&5.99\%&16.73\%&7.11\%&71.74\%&22.21\%&40.22\%&28.12\%&26.55\%&31.09\%\\
 \hline
 
 
    \end{tabular}
    \end{adjustbox}
    


\end{table*} 


\begin{comment}


\begin{table*}
    \centering
   \caption{Reduction of test executions between different Selection Strategies}\label{table:rq1_cmp_ratio}

   	\begin{adjustbox}{width=1.8\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    %p{1.4cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}
    
    \toprule
    
    Subject & Strategy & \prapr{} & \simfix{} & \avatar{} & \kpar{} & \tbar{} & \fixminer{} & \dynamoth{} & \acs{} & \arja{} & \kali{} & \genprog{} & \rsrepair{} \\ \hline
\multirow{3}{*}{Lang} & Class/State&15.43\%&7.36\%&10.58\%&4.78\%&15.06\%&8.54\%&65.92\%&32.65\%&25.52\%&10.89\%&13.64\%&14.15\%\\
 & Class/Method&13.05\%&7.12\%&8.46\%&3.64\%&12.89\%&6.67\%&61.08\%&32.65\%&24.70\%&9.59\%&12.83\%&12.38\%\\ 
 & Method/State&3.28\%&0.40\%&3.41\%&1.14\%&4.03\%&3.79\%&22.86\%&0.00\%&3.33\%&3.79\%&1.63\%&3.55\%\\ \hline
 
 
\multirow{3}{*}{Math} & Class/State&15.10\%&20.30\%&4.22\%&5.86\%&12.94\%&8.57\%&49.67\%&31.11\%&25.88\%&9.26\%&17.00\%&13.36\%\\
 & Class/Method&12.59\%&18.85\%&2.99\%&4.63\%&10.64\%&6.45\%&28.72\%&0.00\%&19.46\%&5.96\%&12.24\%&8.59\%\\ 
 & Method/State&3.49\%&2.25\%&1.23\%&1.23\%&3.60\%&3.22\%&34.61\%&31.11\%&10.16\%&4.74\%&7.15\%&6.30\%\\ \hline
\multirow{3}{*}{Time} & Class/State&21.67\%&17.03\%&8.93\%&0.00\%&8.93\%&12.27\%&32.90\%&0.00\%&12.69\%&25.67\%&9.64\%&8.84\%\\
 & Class/Method&20.54\%&15.85\%&8.93\%&0.00\%&8.93\%&12.27\%&32.90\%&0.00\%&7.82\%&22.52\%&6.59\%&5.65\%\\ 
 & Method/State&2.91\%&6.67\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&10.15\%&10.66\%&8.94\%&6.36\%\\ \hline
\multirow{3}{*}{Chart} & Class/State&23.86\%&0.81\%&11.35\%&4.83\%&16.21\%&5.29\%&64.47\%&-&45.46\%&25.33\%&22.20\%&20.27\%\\
 & Class/Method&23.63\%&0.81\%&11.35\%&4.83\%&16.21\%&5.29\%&63.39\%&-&43.19\%&24.16\%&20.68\%&18.49\%\\ 
 & Method/State&0.38\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&8.50\%&-&8.56\%&2.67\%&5.55\%&4.45\%\\ \hline
\multirow{3}{*}{Closure} & Class/State&38.84\%&49.14\%&5.17\%&6.58\%&7.27\%&0.00\%&-&-&-&-&-&-\\
 & Class/Method&26.04\%&39.39\%&4.63\%&4.91\%&6.63\%&0.00\%&-&-&-&-&-&-\\ 
 & Method/State&23.28\%&17.69\%&3.14\%&4.62\%&4.86\%&0.00\%&-&-&-&-&-&-\\ \hline
\multirow{3}{*}{Mockito} & Class/State&6.73\%&-&20.94\%&6.25\%&19.56\%&0.00\%&-&-&-&-&-&-\\
 & Class/Method&6.55\%&-&19.47\%&6.25\%&13.20\%&0.00\%&-&-&-&-&-&-\\ 
 & Method/State&0.21\%&-&1.47\%&0.00\%&6.48\%&0.00\%&-&-&-&-&-&-\\ \hline
\multirow{3}{*}{Average} & Class/State&20.27\%&18.93\%&10.20\%&4.72\%&13.33\%&5.78\%&53.24\%&21.25\%&27.39\%&17.79\%&15.62\%&14.15\%\\
&Class/Method&17.07\%&16.40\%&9.30\%&4.05\%&11.42\%&5.11\%&46.52\%&10.88\%&23.79\%&15.56\%&13.09\%&11.28\%\\
&Method/State&5.59\%&5.40\%&1.54\%&1.17\%&3.16\%&1.17\%&16.49\%&10.37\%&8.05\%&5.47\%&5.82\%&5.17\%\\
 \bottomrule
 
    \end{tabular}
    \end{adjustbox}
\end{table*} 
\end{comment}




==> newtables/rq1_cmp_wilcox.tex <==

\begin{comment}

\begin{table*}
    \centering
   \caption{Wilcoxon signed-rank test between reduction achieved by  RTS strategies\lingming{class vs. state may be better changed to No vs class; also why not use macros why call them class, state, method? also, stmt is more widely used than state as the abbreviation for statement} \yiling{>< I don't want to add no v.s class, since the table requires some manual efforts.. }\lingming{you can do it after we are done with all other parts, but you should do it I guess}}\label{table:rq1_cmp_wilcox}
   	\begin{adjustbox}{width=1.8\columnwidth}
    \begin{tabular}{|r|c|| rrrrrrrrrrrr|}
    %p{1.4cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}
    
    %\cellcolor{ggggray} 
    %
    
    \hline
    
    Subject & Strategy & \prapr{} & \simfix{} & \avatar{} & \kpar{} & \tbar{} & \fixminer{} & \dynamoth{} & \acs{} & \arja{} & \kali{} & \genprog{} & \rsrepair{} \\ \hline \hline

\multirow{3}{*}{Lang} & \rtsclass{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}\\ \hline
\multirow{3}{*}{Math} & \rtsclass{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\ \hline
\multirow{3}{*}{Time} & \rtsclass{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}\\ \hline
\multirow{3}{*}{Chart} & \rtsclass{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&-&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&-&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsmethod{} v.s \rtsstate{}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}\\ \hline
\multirow{3}{*}{Closure} & \rtsclass{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&-&-&-&-&-&-\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&-&-&-&-&-&-\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&-&-&-&-&-&-\\ \hline
\multirow{3}{*}{Mockito} & \rtsclass{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&-&-&-&-&-\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&-&-&-&-&-\\
 & \rtsmethod{} v.s \rtsstate{}&\ding{109}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&-&-&-&-&-\\
 \hline
 
    \end{tabular}
    \end{adjustbox}
\end{table*} 

\end{comment}


\begin{table*}
    \centering
   \caption{Wilcoxon signed-rank test between reduction achieved by  RTS strategies\Comment{\lingming{maybe remove no vs class?}}}\label{table:rq1_cmp_wilcox}
   	\begin{adjustbox}{width=1.8\columnwidth}
    \begin{tabular}{|r|c|| rrrrrrrrrrrr|}
    %p{1.4cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}
    
    %\cellcolor{ggggray} 
    %
    
    \hline
    
    \textbf{Subject} &  \textbf{RTS Strategy} &  \textbf{\prapr{}} &  \textbf{\simfix{}} &  \textbf{\avatar{}} &  \textbf{\kpar{}} &  \textbf{\tbar{}} &  \textbf{\fixminer{}} &  \textbf{\dynamoth{}} &  \textbf{\acs{}} &  \textbf{\arja{}} &  \textbf{\kali{}} &  \textbf{\genprog{}} &  \textbf{\rsrepair{}} \\ \hline \hline


\multirow{2}{*}{Lang} 
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}\\ \hline
\multirow{2}{*}{Math}
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\ \hline
\multirow{2}{*}{Time} 
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}\\ \hline
\multirow{2}{*}{Chart} 
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&-&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsmethod{} v.s \rtsstate{}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}\\ \hline
\multirow{2}{*}{Closure} 
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&-&-&-&-&-&-\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&-&-&-&-&-&-\\ \hline
\multirow{2}{*}{Mockito} 
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&-&-&-&-&-\\
 & \rtsmethod{} v.s \rtsstate{}&\ding{109}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&-&-&-&-&-\\ \hline
    \end{tabular}
    \end{adjustbox}
\end{table*} 
%\end{comment}




\begin{comment}
\begin{table*}
    \centering
   \caption{Wilcoxon signed-rank test between RTS strategies based on reduction of test executions\lingming{maybe remove no vs class?}}\label{table:rq1_cmp_wilcox}
   	\begin{adjustbox}{width=1.8\columnwidth}
    \begin{tabular}{|r|c|| rrrrrrrrrrrr|}
    %p{1.4cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}
    
    %\cellcolor{ggggray} 
    %
    
    \hline
    
    \textbf{Subject} &  \textbf{RTS Strategy} &  \textbf{\prapr{}} &  \textbf{\simfix{}} &  \textbf{\avatar{}} &  \textbf{\kpar{}} &  \textbf{\tbar{}} &  \textbf{\fixminer{}} &  \textbf{\dynamoth{}} &  \textbf{\acs{}} &  \textbf{\arja{}} &  \textbf{\kali{}} &  \textbf{\genprog{}} &  \textbf{\rsrepair{}} \\ \hline \hline


\multirow{3}{*}{Lang} & \norts{} v.s \rtsclass{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}\\ \hline
\multirow{3}{*}{Math} & \norts{} v.s \rtsclass{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\ \hline
\multirow{3}{*}{Time} & \norts{} v.s \rtsclass{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}\\ \hline
\multirow{3}{*}{Chart} & \norts{} v.s \rtsclass{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&-&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&-&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}\\
 & \rtsmethod{} v.s \rtsstate{}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\ding{109}\\ \hline
\multirow{3}{*}{Closure} & \norts{} v.s \rtsclass{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&-&-&-&-&-&-\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&-&-&-&-&-&-\\
 & \rtsmethod{} v.s \rtsstate{}&\cellcolor{gggray}\ding{52}&\cellcolor{gggray}\ding{52}&\ding{109}&\ding{109}&\cellcolor{gggray}\ding{52}&\ding{109}&-&-&-&-&-&-\\ \hline
\multirow{3}{*}{Mockito} & \norts{} v.s \rtsclass{}&\cellcolor{gggray}\ding{52}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&-&-&-&-&-\\
 & \rtsclass{} v.s \rtsmethod{}&\cellcolor{gggray}\ding{52}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&-&-&-&-&-\\
 & \rtsmethod{} v.s \rtsstate{}&\ding{109}&-&\ding{109}&\ding{109}&\ding{109}&\ding{109}&-&-&-&-&-&-\\ \hline
    \end{tabular}
    \end{adjustbox}
\end{table*} 

\end{comment}

==> newtables/rq2_edit_ratio.tex <==

\begin{table*}[htb]
    \centering
   \caption{Ratio of patches of different fixing code scales\lingming{change this one into stacked bar plot figs like fig2}}\label{tab:patch_ratio_edit}
   
   	\begin{adjustbox}{width=2.05\columnwidth}
    \begin{tabular}{|r|| rrrrrrrrrrrr|}
         \hline

Ratio&PraPR&SimFix&AvatarFixer&kParFixer&TBarFixer&FixMiner&Dynamoth&ACS&Arja&Kali&GenProg&RSRepair\\ \hline \hline
MC&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&34.05\%&0.00\%&38.70\%&7.98\%\\
MM&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&11.86\%&0.00\%&11.87\%&3.93\%\\
MS&0.00\%&93.49\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&0.00\%&12.68\%&0.00\%&13.28\%&3.98\%\\
SS&100.00\%&6.51\%&100.00\%&100.00\%&100.00\%&100.00\%&100.00\%&100.00\%&41.41\%&100.00\%&36.15\%&84.12\%\\




     \hline

    
    
    \end{tabular}
    \end{adjustbox}
    

\end{table*} 



==> newtables/rq2_patchratio.tex <==

\begin{table*}[htb]
    \centering
   \caption{Ratio of different patch categories on all APR systems\lingming{tables like this one can be changed into stacked bar charts to save space; you only need to show the average results rather than the per-subject results } \yiling{DONE}}\label{tab:patch_ratio}
   
   	\begin{adjustbox}{width=2.05\columnwidth}
    \begin{tabular}{|r|| rrr|rrr|rrr|rrr|rrr|rrr|}

     \hline
    
    \multirow{2}{*}{}  & \multicolumn{3}{c}{Lang} & \multicolumn{3}{|c}{Math} & \multicolumn{3}{|c}{Chart} & \multicolumn{3}{|c}{Time} & \multicolumn{3}{|c}{Closure} & \multicolumn{3}{|c|}{Mockito} \\ \cline{2-19}
    
    APR & \stopfpatch{}  & \stopppatch{} & \plausiblepatch{}  & \stopfpatch{}  & \stopppatch{} & \plausiblepatch{} & \stopfpatch{}  & \stopppatch{} & \plausiblepatch{}  & \stopfpatch{}  & \stopppatch{} & \plausiblepatch{}  & \stopfpatch{}  & \stopppatch{} & \plausiblepatch{}  & \stopfpatch{}  & \stopppatch{} & \plausiblepatch{} \\  \hline  \hline 
    
    
PraPR&95.32\%&0.31\%&4.37\%&94.92\%&1.53\%&3.55\%&98.78\%&0.29\%&0.93\%&97.18\%&0.74\%&2.07\%&98.78\%&0.33\%&0.89\%&96.45\%&0.85\%&2.70\%\\
SimFix&96.38\%&0.00\%&3.62\%&85.13\%&1.02\%&13.85\%&96.86\%&0.11\%&3.03\%&97.34\%&0.00\%&2.66\%&-&-&-&58.44\%&0.00\%&41.56\%\\
AvatarFixer&95.18\%&0.53\%&4.29\%&95.52\%&0.69\%&3.80\%&90.91\%&6.06\%&3.03\%&86.84\%&0.00\%&13.16\%&73.75\%&1.25\%&25.00\%&96.45\%&0.35\%&3.19\%\\
kParFixer&92.33\%&0.26\%&7.41\%&94.80\%&0.00\%&5.20\%&100.00\%&0.00\%&0.00\%&94.44\%&0.00\%&5.56\%&98.67\%&1.33\%&0.00\%&94.37\%&1.19\%&4.44\%\\
TBarFixer&87.13\%&1.35\%&11.52\%&86.54\%&1.17\%&12.29\%&90.91\%&0.00\%&9.09\%&78.95\%&0.00\%&21.05\%&80.00\%&0.00\%&20.00\%&93.40\%&0.21\%&6.38\%\\
FixMiner&88.17\%&0.30\%&11.54\%&92.02\%&0.19\%&7.79\%&87.50\%&0.00\%&12.50\%&94.12\%&0.00\%&5.88\%&100.00\%&0.00\%&0.00\%&100.00\%&0.00\%&0.00\%\\
Dynamoth&28.57\%&0.00\%&71.43\%&14.04\%&7.02\%&78.95\%&66.67\%&0.00\%&33.33\%&10.00\%&0.00\%&90.00\%&-&-&-&-&-&-\\
ACS&66.67\%&0.00\%&33.33\%&66.67\%&0.00\%&33.33\%&100.00\%&0.00\%&0.00\%&-&-&-&-&-&-&-&-&-\\
Arja&84.40\%&5.60\%&10.00\%&79.35\%&9.28\%&11.38\%&93.94\%&6.06\%&0.00\%&78.40\%&11.94\%&9.66\%&-&-&-&-&-&-\\
Kali&93.24\%&0.75\%&6.01\%&93.33\%&2.30\%&4.37\%&97.72\%&1.75\%&0.53\%&89.60\%&1.37\%&9.03\%&-&-&-&-&-&-\\
GenProg&90.65\%&5.54\%&3.81\%&88.62\%&6.23\%&5.15\%&92.11\%&7.89\%&0.00\%&88.57\%&9.84\%&1.59\%&-&-&-&-&-&-\\
RSRepair&95.93\%&0.82\%&3.25\%&95.84\%&1.45\%&2.71\%&99.79\%&0.21\%&0.00\%&96.07\%&2.12\%&1.81\%&-&-&-&-&-&-\\



 \hline

    
    
    \end{tabular}
    \end{adjustbox}
    

\end{table*} 

\begin{comment}
    
PraPR&95.32\%&0.31\%&4.37\%&94.92\%&1.53\%&3.55\%&98.78\%&0.29\%&0.93\%&97.18\%&0.74\%&2.07\%&98.78\%&0.33\%&0.89\%&96.45\%&0.85\%&2.70\%\\
SimFix&96.38\%&0.00\%&3.62\%&85.13\%&1.02\%&13.85\%&96.86\%&0.11\%&3.03\%&97.34\%&0.00\%&2.66\%&-&-&-&58.44\%&0.00\%&41.56\%\\
AvatarFixer&95.18\%&0.53\%&4.29\%&95.52\%&0.69\%&3.80\%&90.91\%&6.06\%&3.03\%&86.84\%&0.00\%&13.16\%&73.75\%&1.25\%&25.00\%&96.45\%&0.35\%&3.19\%\\
kParFixer&92.33\%&0.26\%&7.41\%&94.80\%&0.00\%&5.20\%&100.00\%&0.00\%&0.00\%&94.44\%&0.00\%&5.56\%&98.67\%&1.33\%&0.00\%&94.37\%&1.19\%&4.44\%\\
TBarFixer&87.13\%&1.35\%&11.52\%&86.54\%&1.17\%&12.29\%&90.91\%&0.00\%&9.09\%&78.95\%&0.00\%&21.05\%&80.00\%&0.00\%&20.00\%&93.40\%&0.21\%&6.38\%\\
FixMiner&88.17\%&0.30\%&11.54\%&92.02\%&0.19\%&7.79\%&87.50\%&0.00\%&12.50\%&94.12\%&0.00\%&5.88\%&100.00\%&0.00\%&0.00\%&100.00\%&0.00\%&0.00\%\\
Dynamoth&28.57\%&0.00\%&71.43\%&14.04\%&7.02\%&78.95\%&66.67\%&0.00\%&33.33\%&10.00\%&0.00\%&90.00\%&-&-&-&-&-&-\\
ACS&66.67\%&0.00\%&33.33\%&66.67\%&0.00\%&33.33\%&100.00\%&0.00\%&0.00\%&-&-&-&-&-&-&-&-&-\\
Arja&84.40\%&5.60\%&10.00\%&79.35\%&9.28\%&11.38\%&93.94\%&6.06\%&0.00\%&78.40\%&11.94\%&9.66\%&-&-&-&-&-&-\\
Kali&93.24\%&0.75\%&6.01\%&93.33\%&2.30\%&4.37\%&97.72\%&1.75\%&0.53\%&89.60\%&1.37\%&9.03\%&-&-&-&-&-&-\\
GenProg&90.65\%&5.54\%&3.81\%&88.62\%&6.23\%&5.15\%&92.11\%&7.89\%&0.00\%&88.57\%&9.84\%&1.59\%&-&-&-&-&-&-\\
RSRepair&95.93\%&0.82\%&3.25\%&95.84\%&1.45\%&2.71\%&99.79\%&0.21\%&0.00\%&96.07\%&2.12\%&1.81\%&-&-&-&-&-&-\\
\end{comment}

==> newtables/rq3_bugs.tex <==


\begin{table*}
    \centering
   \caption{Reduction  On plausibly-fixed and partially-fixed bugs}\label{table:rq3_bug}

   	\begin{adjustbox}{width=2\columnwidth}
   	
   	
   	
    \begin{tabular}{r| rrr| rrr| rrr| rrr}\hline
    \toprule
    
    \multirow{3}{*}{APR} & \multicolumn{6}{c|}{Plausibly-fixed Bug} & \multicolumn{6}{c}{Partially-fixed Bug{}}  \\ \cline{2-13}
    
    
    & \multicolumn{3}{c|}{Reduction on \norts{} (\%)}  & \multicolumn{3}{c|}{ Between Strategies (\%)}   & \multicolumn{3}{c|}{Reduction on \norts{} (\%)}  & \multicolumn{3}{c}{ Between Strategies (\%)}  \\   \cline{2-13}
    
    & No/Class & No/Method & No/State &  Class/State &  Class/Method & Method/State   & No/Class & No/Method & No/State &  Class/State & Class/Method & Method/State   \\ \midrule
 
 PraPR&78.65&88.70&90.42&45.02&38.23&12.68&38.91&44.86&45.65&15.52&13.55&2.91\\
SimFix&84.05&96.31&97.76&58.31&51.15&22.63&22.58&30.49&30.49&23.39&23.39&0.00\\
AvatarFixer&82.22&99.32&99.49&75.48&66.35&20.75&65.12&78.62&78.84&60.10&51.68&8.42\\
kParFixer&83.44&99.28&99.77&82.05&67.92&28.31&49.23&72.92&73.29&55.38&47.54&12.78\\
TBarFixer&76.04&95.36&99.52&85.00&75.02&23.58&50.82&73.42&73.79&48.29&42.71&14.09\\
FixMiner&93.28&99.71&99.80&86.58&78.87&13.53&83.67&95.37&97.58&61.61&39.91&44.26\\
Dynamoth&87.50&99.19&99.27&78.82&71.02&19.92&94.52&96.47&96.98&50.45&37.50&22.87\\
ACS&98.34&99.66&99.95&95.65&48.98&46.67&-&-&-&-&-&-\\
Arja&92.71&97.95&98.24&73.61&65.81&16.49&60.90&65.62&67.04&41.10&33.13&17.82\\
Kali&83.85&98.39&98.97&72.57&64.02&31.42&66.50&75.37&76.52&40.69&32.35&12.46\\
GenProg&90.04&94.71&94.95&57.10&48.80&13.80&64.21&70.85&72.85&47.78&37.01&29.75\\
RSRepair&89.53&92.45&92.91&42.16&34.39&12.07&68.01&72.33&73.59&33.70&25.61&15.91\\



 \bottomrule
 
    \end{tabular}
    \end{adjustbox}
    


\end{table*} 


==> newtables/rq4_full_partial_summary.tex <==


\begin{table*}
    \centering
   \caption{Reduction with Full and Partial Matrix}\label{table:rq4_summary}

   	\begin{adjustbox}{width=2\columnwidth}
   
   	
    \begin{tabular}{r| rrr| rrr| rrr| rrr}\hline
    \toprule
    
    \multirow{3}{*}{APR} & \multicolumn{6}{c|}{Partial Matrix} & \multicolumn{6}{c}{Full Matrix}  \\ \cline{2-13}
    
    
    & \multicolumn{3}{c|}{Reduction on \norts{} (\%)}  & \multicolumn{3}{c|}{ Between Strategies (\%)}   & \multicolumn{3}{c|}{Reduction on \norts{} (\%)}  & \multicolumn{3}{c}{ Between Strategies (\%)}  \\   \cline{2-13}
    
    & No/Class & No/Method & No/State &  Class/State &  Class/Method & Method/State   & No/Class & No/Method & No/State &  Class/State & Class/Method & Method/State   \\ \midrule
    
    PraPR&36.96&42.47&43.50&20.27&17.07&5.59&71.70&81.33&82.54&52.87&46.81&14.23\\
SimFix&19.21&25.84&26.61&18.93&16.40&5.40&75.08&96.58&98.09&70.73&64.00&16.44\\
AvatarFixer&11.75&14.23&14.25&10.20&9.30&1.54&76.85&90.97&96.43&80.97&61.99&37.68\\
kParFixer&4.66&5.96&5.99&4.72&4.05&1.17&78.49&91.26&96.50&78.29&60.36&33.84\\
TBarFixer&13.13&15.90&16.73&13.33&11.42&3.16&76.77&90.94&96.96&82.12&62.56&38.79\\
FixMiner&6.52&7.09&7.11&5.78&5.11&1.17&81.55&95.77&99.27&83.77&64.03&35.57\\
Dynamoth&66.93&71.66&71.74&53.24&46.52&16.49&85.27&98.02&98.18&73.21&65.00&18.77\\
ACS&21.85&22.15&22.21&21.25&10.88&10.37&94.94&98.56&99.32&92.82&70.58&28.07\\
Arja&37.08&39.71&40.22&27.39&23.79&8.05&85.34&96.12&96.81&73.69&66.36&21.37\\
Kali&24.34&27.83&28.12&17.79&15.56&5.47&88.25&96.99&97.28&68.38&61.18&22.06\\
GenProg&24.45&26.24&26.55&15.62&13.09&5.82&85.06&96.01&96.71&72.16&63.87&25.13\\
RSRepair&29.36&30.75&31.09&14.15&11.28&5.17&87.10&96.78&97.26&72.69&64.31&26.65\\



 \bottomrule
 
    \end{tabular}
    \end{adjustbox}
    


\end{table*} 


==> newtables/rq5_combine.tex <==
\begin{table}
    \centering
    \caption{Reduction of \ourtool{} on different APR system}\label{table:ourtool}
   	\begin{adjustbox}{width=0.9\columnwidth}
    \begin{tabular}{ r rrrr}
    \toprule{}
    
    %APR & \rtsstate{} & \trp{} & \ourtoolglobal{} & \ourtoolclass{} & \ourtoolmethod{} \ourtoolstate{} \\ \hline
    
    APR & \rtsstate{} & \trp{}  & \ourtoolmethod{} \\ \midrule{}
    PraPR&43.50\%&14.53\%&44.18\%\\
    SimFix&26.61\%&2.18\%&26.62\%\\
    AvatarFixer&14.25\%&0.98\%&14.26\%\\
    kParFixer&5.99\%&-1.75\%&6.00\%\\
    TBarFixer&16.73\%&-1.08\%&16.73\%\\
    FixMiner&7.11\%&-1.44\%&7.11\%\\
    Dynamoth&71.74\%&2.07\%&71.79\%\\
    ACS&22.21\%&0.00\%&22.21\%\\
    Arja&40.22\%&20.58\%&40.74\%\\
    Kali&28.12\%&6.80\%&28.15\%\\
    GenProg&26.55\%&14.03\%&26.63\%\\
    RSRepair&31.09\%&14.31\%&31.11\%\\

    \bottomrule{}
    \end{tabular}
    \end{adjustbox}
    
\end{table} 

==> newtables/subinfo.tex <==

\begin{table}[htb]
	\centering
	\small
	\caption{Benchmark information}\label{table:subinfo}
	
	\begin{adjustbox}{width=0.8\columnwidth}
	   	
	\begin{tabular}{|l|l|r|r|r|}
		\hline
        \textbf{ID} & \textbf{Name}&\textbf{\#Bug} & \textbf{\#Test} &\textbf{LoC}\\ \hline\hline
        
        
	    Lang & Apache commons-lang & 65 & 2,245 & 22K \\ 
	    Math & Apache commons-math & 106 & 3,602 & 85K \\ 
	    Time & Joda-Time & 27 & 4,130 & 28K \\ 
	    Chart & JFreeChart & 26 & 2,205 & 96K \\ 
	    Closure & Google Closure compiler & 133 & 7,927 & 90K \\ 
	    Mockito & Mockito framework & 38 & 1,366 & 23K \\ \hline \hline
	    
	   \multicolumn{2}{|c|}{\textbf{\olddefects{}}} & \textbf{395} & \textbf{21,475} & \textbf{344K}\\
		\hline
	\end{tabular}
	\end{adjustbox}
\end{table}


==> oldrq/rq0.tex <==
\input{newtables/rq0_cmp_all}
\subsection{RQ1: Revisiting APR Efficiency} ~\label{sec:rq0}
%In this research question, our study makes the first attempt to empirically investigate the efficiency of different APR systems (1) based on the number of test executions, and (2) aligned with the same RTS configuration. Therefore, our results provide new insights on APR efficiency.
Table~\ref{table:rq0_cmpall} presents the number of test executions with different RTS strategies. 
We also present the number of validated patches \Comment{before the plausible one is found} (\#Patch) in the table. Note that cells are empty when there is no valid patch generated. Based on the table, we have the following observations.
%\lingming{just realize this: do you also count the number of t executions before the plausible patch? otherwise, it is inconsistent} 

First, measuring APR efficiency by a more precise metric (i.e., the number of test executions) can draw totally different conclusions from the number of validated patches advocated by prior work~\cite{DBLP:conf/icse/0001WKKB0WKMT20}.
For example, for each buggy version of Time, \simfix{} (i.e., 22.81 patches) validates many more patches than \avatar{} (i.e., 2.50 patches), showing that \simfix{} is less efficient than \avatar{} in terms of the number of validated patches. 
Such a conclusion is consistent with the finding in  previous work~\cite{DBLP:conf/icse/0001WKKB0WKMT20}, which also measures APR efficiency by the number of validated patches. 
However, the conclusion can be opposite if these systems are compared by the number of test executions. For example, with class-level RTS, \simfix{} executes 184.27 tests and \avatar{} executes 232.55 tests per buggy version of Time, indicating that \simfix{} is more efficient than \avatar{}. The reason is that although \avatar{} generates less patches than \simfix{}, each patch of \avatar{} executes many more tests than \simfix{}. Such inconsistencies between the number of test executions and patches are prevalent in the table. 
In summary, it is imprecise to measure APR efficiency by simply counting the number of patches, since different patches can execute totally different number of tests. We thus suggest future work on APR efficiency to adopt the number of test executions since it is a more precise metric.



Second, comparing APR efficiency with different RTS strategies can also deliver opposite conclusions.  
For example, on subject Time, \avatar{} executes 232.55 and 9.73 tests with \rtsclass{} and  \rtsmethod{}, while \simfix{} executes 184.27 and 58.64 tests with \rtsclass{} and \rtsmethod{}.
When both systems are configured with method-level RTS, \avatar{} is considered as more efficient than \simfix{}; however, when they are compared  under class-level RTS,  \avatar{} is actually less efficient than \simfix{}. 
Moreover, if APR systems are compared under different RTS strategies respectively, the conclusion may further be skewed.
Therefore, it is important to adopt the same RTS strategy when comparing the repair efficiency among different APR systems. 
In addition, we strongly recommend that future APR work should explicitly describe the RTS strategy adopted in their experimental procedure, so that their follow-up work can mitigate the threats in RTS configuration. 

\finding{\textit{the number of patches widely used for measuring APR efficiency can incur skewed conclusions, and the use of inconsistent RTS configurations can further skew the conclusion. Future APR work should explicitly describe their adopted RTS strategies and the efficiency comparison among multiple APR systems should guarantee a consistent RTS configuration. }}

\Comment{\finding{\textit{Compared to a more precise metric, the number of patches used before can have misleading conclusions on APR efficiency.
RTS strategy is an important configuration associated with APR efficiency measurement. Future work should explicitly describe the RTS strategy used in experiments and the efficiency comparison among APR systems should guarantee a consistent RTS configuration in each APR system.}}}



%Overall, we observe that different APR systems exhibit different number of test executions, e.g., \prapr{}, \genprog{}, and \arja{} remarkably execute more tests than the \avatar{} family. 



==> oldrq/rq1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\begin{figure}[h]
    \centering
    \includegraphics[width=8cm, height= 10cm]{pics/alltest_partial_All_rq1_violin.pdf}
    \caption{The distribution of \ntacc{} with different test selection strategies}
    \label{fig:ntacc_box}
\end{figure}
\end{comment}

\input{newtables/rq1_cmp_ratio_summary}


\subsection{RQ2: Overall Impact of RTS Strategies} ~\label{sec:rq1}
%In this research question, we investigate the impact of RTS strategies on repair efficiency for studied APR systems. We discuss the findings as follows.
Table~\ref{table:rq1_cmpnorts_ratio} presents the reduction of test executions achieved by each RTS strategy compared to no test selection. 
Based on the table, for all the studied APR systems on almost all the subjects, adopting RTS can remarkably reduce the number of test executions in patch validation.
For example, on the subject Math, \dynamoth{} skips 93.33\% of test executions if it adopts \rtsstate{}.
Even for RTS at the coarsest level (i.e., \rtsclass{}), the average reduction ranges from 4.66\% to 66.93\% among different APR systems. Note that at some cases there is no difference among RTS strategies, e.g., ACS on Time, because all generated patches fail at the first executed test (i.e., the first originally-failed test still fails on these patches). We would further analyze the individual impact on different patches in Section~\ref{sec:rq2}.
In summary, our results suggest that RTS can significantly improve the efficiency of patch validation and future APR work should no longer overlook such an important optimization.

\finding{\textit{for all studied APR systems, adopting regression test selection can remarkably improve APR efficiency and should be considered in future APR work.}} 

\yiling{HERE:add results on time metrics}

\input{newtables/rq1_cmp_wilcox}

%%%%%%%%%%%%%%%%%%%

Overall, we can observe a common trend that \rtsstate{} always executes the least tests while \rtsclass{} exhibits the most number of test executions. This is not surprising because class-level coverage is the coarsest selection criterion, based on which more tests would inherently be selected. To further investigate the difference between RTS strategies,  we perform the Wilcoxon Signed-Rank Test~\cite{wilcoxon1992individual} at the significance level of 0.05 to compare the reduction achieved by different selection strategies in Table~\ref{table:rq1_cmp_wilcox}.
We use \ding{109} and \ding{52} to denote ``no statistical difference'' and “significant difference (p-value<0.05)”, respectively. 
From the table, we can observe that RTS strategies cause significant difference on the reduction of test executions. In particular,  both \rtsmethod{} and \rtsstate{} significantly outperform \rtsclass{}. \Comment{, which in turn substantially outperforms \norts{}. }
Meanwhile, interestingly, the difference between \rtsmethod{} and \rtsstate{} is often subtle. For example, as suggested by Table~\ref{table:rq1_cmpnorts_ratio} and Table~\ref{table:rq1_cmp_wilcox}, the average difference between \rtsmethod{} and \rtsstate{} is less than 1\% at most cases and is mostly not significant according to the statistical analysis. In fact, this observation is consistent with prior work in traditional regression testing~\cite{DBLP:conf/icse/Zhang18}, which shows that method-level RTS outperforms class-level RTS but is often not significantly worse than statement-level RTS. The reason is that modern system design principles recommend writing simple method bodies for the ease of maintenance, making the
majority of method body changes directly affect all tests covering the methods (i.e., \rtsstate{} is close to \rtsmethod{}).
In summary, method- and statement-level RTS are more recommended for APR. 



\finding{\textit{different RTS strategies exhibit different reduction performance. \rtsstate{} and \rtsmethod{} perform similarly, but both of them significantly outperform \rtsclass{}\Comment{, which in turn substantially outperforms \norts{}}.}} 


%%%% comparison between strategies 
\begin{comment}
We further calculate the relative reduction between different selection strategies in Table~\ref{table:rq1_cmpnorts_ratio}. For example, on subject Lang, the row ``Class/Method'' means that \prapr{} executes 15.34\% less of tests with \rtsmethod{} than \rtsclass{}. Here ``-'' means no validated patches. Based on the table, it is interesting that \rtsclass{} remarkably executes more tests than the other two selection strategies while the difference between \rtsmethod{} and \rtsstate{} is quite small. For example, in \avatar{}, \rtsstate{} only executes 1.54\% of tests than \rtsmethod{}, while \rtsmethod{} executes 9.30\% tests than \rtsclass{}. Therefore, \textbf{method and statement levels are both recommended strategies for test selection in patch validation.} 
%Furthermore, it is notable that some APR systems are more susceptible to test execution strategies.
\end{comment}



%%%%%%%%%%%%%%%%%%%%%




% 58 (52)
% 3: 14
% 2: 12
% 1 : 2
% 0 : 24 
% invalid: 6

% code example? 
% since it is accumulated -> average, per patch, -> plot -> bias -> ratio-plot

%\textbf{difference between method and class is larger than difference between state and method} % One potential reason might be that, the code scale from statement to class level significantly involve much more code elements compared to the code scale between statement and method level. 



% In other words, rts strategy setting is an significant factor associated with patch validation efficiency which should no longer be unclear in the future evalutation of apr techniques.








==> oldrq/rq2.tex <==


\subsection{RQ3: Impact on Different Patches}~\label{sec:rq2}
We now investigate the impact of RTS strategies on the patches of different characteristics. Based on the intuition that a patch involving more test executions might be more sensitive to RTS strategies, we categorize patches by their fixing capabilities or fixing code scopes. Section~\ref{sec:cate1} and Section~\ref{sec:cate2} present the impact on these patch categorizations respectively.

\input{newtables/rq2_patches_median_mean}

\subsubsection{Impact on patches of different fixing capabilities} \label{sec:cate1}

Based on test execution results, we can categorize patches into groups of different fixing capabilities. (1) \stopfpatch{}: a patch cannot fix all originally-failed tests and thus its validation gets aborted by some originally-failed test; (2) \stopppatch{}: a patch can fix all originally-failed tests but fails on some originally-passed test, and thus its validation gets aborted by some originally-passed test; (3) \plausiblepatch{}: a patch that can pass all originally-failed and originally-passed tests (i.e., plausible patch). Obviously, \stopfpatch{} has the weakest fixing capability and its validation halts extremely early, and thus adopting RTS would not make any difference on its number of test executions. Therefore, we present the impact of RTS strategies on the other two patch groups, i.e., \stopppatch{} and \plausiblepatch{} in Table~\ref{table:rq2_pp}. In particular, each cell shows the reduction ratio of test executions compared to no test selection. Note that since \acs{} generates only \stopfpatch{} and \plausiblepatch{},  its corresponding cells in \stopppatch{} are empty.
Based on the table, we can observe that, compared to the overall reduction on all patches (i.e., the reduction in Table~\ref{table:rq1_cmpnorts_ratio}), the impact of test selection strategies on \plausiblepatch{} and \stopppatch{} is even more remarkable. For example, the reduction ratio ranges from 66.33\% to 99.42\% on \stopppatch{}, and ranges from 76.07\% to 99.95\% on \plausiblepatch{}. In addition, compared to all patches, the difference between RTS strategies is also enlarged on \plausiblepatch{} and \stopppatch{}. In summary, RTS can achieve larger reductions for patches with stronger fixing capabilities.


\finding{\textit{the impact of RTS strategies is even more prominent on \plausiblepatch{} and \stopppatch{}, where an  extremely large portion of tests (e.g., up to 99.95\%) get reduced.}} 



\begin{figure}[htb]
    \centering
    \includegraphics[width=7.5 cm, height= 3.8 cm]{new_pics/rq2_patchratio_preplot_table.pdf}
    \caption{Ratio of patches of different fixing capabilities}
    \label{fig:ratio1}
\end{figure}




Considering the drastic impact of RTS on \plausiblepatch{} and \stopppatch{}, we proceed to check whether an APR system is more susceptible to test selection if it exhibits a higher ratio of \plausiblepatch{} or \stopppatch{}. To this end, we present
the stacked bar plot for the ratio of patch categories of different fixing capabilities in Figure~\ref{fig:ratio1}, from which we can make the following observations.
%Table~\ref{tab:patch_ratio} presents the ratio of each patch category generated by different APR systems.

First, it is noteworthy that almost all the existing APR systems exhibit a very high ratio (e.g., around 90\%) of \stopfpatch{}, indicating that  \stopppatch{} and \plausiblepatch{} are sparse in the space of compilable patches. 
Liu ~\etal{}~\cite{DBLP:conf/icse/0001WKKB0WKMT20} empirically compared the number of un-compilable patches and inplausible patches generated by different APR systems, to measure their costs wasted in patch validation towards generating a valid patch. 
Their work showed that the state-of-the-art APR techniques can avoid generating un-compilable patches.
However in our work, we make the first attempt to investigate patches of different fixing capabilities (e.g., how many tests can pass on each patch).
Our results suggest that for most existing APR systems, the majority of their inplausible patches have a low capability of fixing originally-failed tests and get immediately terminated in the very beginning stage of validation. 
We also find that the two constraint-based APR systems (e.g., \dynamoth{} and \acs{}) generate a lower ratio of \stopfpatch{}. The potential reason may be that constraint-based APR systems target at conditional expressions, which are more likely to impact the test execution outcomes, i.e., making the originally-failed test pass. In addition, \acs{} designs ranking strategies on fixing ingredients for condition synthesis, which might bring the plausible patch forward, end up the whole validation process earlier, and thus reduce the ratio of \stopfpatch{}.
\Comment{In summary, our results call for more efforts from future work to generate less \stopfpatch{}. Otherwise, unnecessary costs would be spent on compiling and validating these patches. }

Second, there is no apparent correlation between the ratio of \stopppatch{} (or \plausiblepatch{}) and the impact degree of RTS strategies. For example, although \prapr{} exhibits a quite low ratio of  \stopppatch{} and \plausiblepatch{} (e.g., 0.29\% and 0.93\%), it reduces a larger portion of test executions than other APR systems. 
One straightforward reason is that the number of originally-failed tests is significantly less than the originally-passed tests. For example, each buggy version in Closure has  2.63 failed tests and 7,180.89 passed tests on average.
The number of skipped originally-passed tests is often significantly larger than the number of originally-failed tests, and thus the impact of RTS on originally-passed tests can still dominate the overall efficiency. 
It also explains why even with such a low ratio of \stopppatch{} and \plausiblepatch{} we can still observe a remarkable impact of RTS on overall  efficiency.


% third, add bugs???
%In indicates that when an APR system generates a lower ratio of \stopfpatch{}, the reduction of test selection strategies would be more significant. For example, \dynamoth{} generates the most ratio of \plausiblepatch{} and \stopppatch{}, and it exhibits the highest reduction against no selection (i.e., Table~\ref{table:rq1_cmpnorts_ratio} or between selection strategies (i.e., Table~\ref{table:rq1_cmp_ratio}). 

\finding{\textit{the majority of compilable patches generated by existing APR systems immediately fail on the originally-failed tests\Comment{, and the constraint-based APR systems generate a higher ratio of patches that can fix originally-failed tests}. Even with such a low ratio of \stopppatch{} and \plausiblepatch{}, the APR efficiency is still sensitive to RTS strategies, since most bugs exhibit substantially more originally-passed tests than originally-failed tests.}} 


\input{newtables/rq2_patches_edit}



\subsubsection{Impact on patches of different fixing scopes} \label{sec:cate2}


Based on the scope of fixed code, patches can be categorized as single-edit or multiple-edit patches. 
In particular, according to the granularity of edited code elements, we categorize patches as: (1) patches editing single class (denoted as \scpatch{}) v.s. patches editing multiple classes (denoted as \mcpatch{}), (2) patches editing single method (denoted as \smpatch{}) v.s.  patches editing multiple methods (denoted as \mmpatch{}), and (3) patches editing single statement (denoted as \sspatch{}) v.s. patches editing multiple statements (denoted as \mspatch{}). 





%\input{newtables/rq2_edit_ratio}
Figure~\ref{fig:ratio2} is a stacked bar plot for the ratio of patch categories of different fixing code scopes.
The figure shows that the majority of generated patches are single-edit patches,  especially when  edited code elements are at coarser granularities (i.e., class or method).
%As suggested by Table~\ref{tab:patch_ratio_edit} 8 APR systems (e.g., \prapr{}, \acs{}, and \kali{})  generate only single-statement patches, \simfix{} generates patches only single-method patches, and \arja{}, \genprog{}, and \rsrepair{} generate multiple-edit patches at all granularities. Overall, the majority of patches generated by existing APR systems are editing only one code element. 




Table~\ref{table:rq2_edit} presents the reduction achieved by RTS at the corresponding granularity on single-edit and multiple-edit patches. For example, the cell in the column ``\rtsclass{}'' and the row ``Lang'' means that on Lang \rtsclass{} can reduce 21.83\% and 27.36\% of test executions on patches that edit multiple classes  (\mcpatch{}) and on patches that edit single class (\scpatch{}), respectively.
Based on the table, at most cases, RTS can reduce more test executions on single-edit patches than multiple-edit patches. The reason is that multiple-edit patches often involve more code elements and thus are covered by more tests, resulting in a lower ratio of reduction. 
Note there are several counter cases, e.g., on Closure the reduction on multiple-statement patches is much larger than on single-statement patches (55.06\% v.s. 17.34\%). We find that at these cases a considerable ratio of generated multiple-edit patches have stronger fixing capabilities (i.e., belong to \stopppatch{} or \plausiblepatch{}) and thus exhibit a higher reduction.



\finding{\textit{most patches generated by existing APR systems are single-edit patches. RTS can reduce more test executions on single-edit patches than on multiple-edit patches, since usually fewer tests can cover the modified code elements of single-edit patches. Meanwhile, for some special cases, multiple-edit patches can have high probabilities in producing high-quality patches passing more tests, leaving more room for RTS.}}

\begin{figure}[htb]
    \centering
    \includegraphics[width=8 cm, height= 3.7 cm]{new_pics/rq2_edits_ratio_preplot.pdf}
    \caption{Ratio of patches of different fixing code scopes}
    \label{fig:ratio2}
\end{figure}







\begin{comment}
We further  present the impact of test selection strategies on \stopppatch{} and  \plausiblepatch{} in Table~\ref{table:rq2_pp}. The column ``Reduction on \norts{}'' means the reduction ratio of test executions against \norts{}, and the column ``Between strategies'' means the reduction ratio between each two test strategies.  Here we leave out the results on \stopfpatch{} because as analyzed in Section~\ref{sec:bound}, no difference would be introduced on this type of patches.


Compared to the overall reduction on all patches (RQ1), the impact of test selection strategies is more significant on \plausiblepatch{} and \stopppatch{}. Compared to no selection, the reduction ratio ranges from 66.33\% to 99.42\% on \stopppatch{}, and from 76.07\% to 99.80\% on \plausiblepatch{}. In addition, the difference between different selection strategies is more remarkable on \plausiblepatch{} and \stopppatch{} than overall patches. In indicates that when an APR system generates a lower ratio of \stopfpatch{}, the reduction of test selection strategies would be more significant. For example, \dynamoth{} generates the most ratio of \plausiblepatch{} and \stopppatch{}, and it exhibits the highest reduction against no selection (i.e., Table~\ref{table:rq1_cmpnorts_ratio} or between selection strategies (i.e., Table~\ref{table:rq1_cmp_ratio}). 



\finding{\textit{a very large ratio of compilable patches generated by existing APR systems still fail on the originally-failed tests, and constraint-based APR systems generate a higher ratio of patches that can pass originally-failed tests.}} 

We first present the ratio of different patch categories generated by each APR system in Table~\ref{tab:patch_ratio}. We observe that existing APR systems exhibit a extremely high ratio (e.g., around 90\%) of \stopfpatch{}; and \stopppatch{} or \plausiblepatch{} are very sparse in the space of compilable patches. Liu et al.~\cite{DBLP:conf/icse/0001WKKB0WKMT20} empirically compared the number of all validated patches, un-compilable patches, and inplausible patches generated by different APR systems, and their work suggested that the state-of-the-art APR techniques can avoid generating un-compilable patches. Our work first investigates the ratio of different patch categories according to the test execution information (e.g., whether the originally-failed tests become pass).  Our results suggest that more efforts should be put to generating less \stopfpatch{}; otherwise, unnecessary costs would be spent on compiling and validating these patches. Furthermore, we find that the two constraint-based APR systems (e.g., \dynamoth{} and \acs{}) generate a lower ratio of \stopfpatch{}.  It indicates that the patches generated by constraint-based APR systems have stronger capability of passing the originally-failed test (i.e., \stopppatch{} or \plausiblepatch{}). One potential reason might be that constraint-based APR systems target at fixing conditional expressions, which are more likely to impact the test execution outcomes, i.e., making the originally-failed test become pass. In addition, \acs{} designs ranking strategies on fixing ingredients for condition synthesis, which brings the validation of the plausible patch forward and reduces the ratio of \stopfpatch{} being validated. 




\finding{\textit{the impact of test selection strategies is extremely significant on \plausiblepatch{} and \stopppatch{}, and a large portion of tests (e.g., 99.80\%) are reduced compared to no test selection.}}

We further  present the impact of test selection strategies on \stopppatch{} and  \plausiblepatch{} in Table~\ref{table:rq2_pp}. The column ``Reduction on \norts{}'' means the reduction ratio of test executions against \norts{}, and the column ``Between strategies'' means the reduction ratio between each two test strategies.  Here we leave out the results on \stopfpatch{} because as analyzed in Section~\ref{sec:bound}, no difference would be introduced on this type of patches.
Compared to the overall reduction on all patches (RQ1), the impact of test selection strategies is more significant on \plausiblepatch{} and \stopppatch{}. Compared to no selection, the reduction ratio ranges from 66.33\% to 99.42\% on \stopppatch{}, and from 76.07\% to 99.80\% on \plausiblepatch{}. In addition, the difference between different selection strategies is more remarkable on \plausiblepatch{} and \stopppatch{} than overall patches. In indicates that when an APR system generates a lower ratio of \stopfpatch{}, the reduction of test selection strategies would be more significant. For example, \dynamoth{} generates the most ratio of \plausiblepatch{} and \stopppatch{}, and it exhibits the highest reduction against no selection (i.e., Table~\ref{table:rq1_cmpnorts_ratio} or between selection strategies (i.e., Table~\ref{table:rq1_cmp_ratio}). 

In summary, the future APR systems are encouraged to generate more patches that can pass more originally-failed tests, where the impact of test selection strategy is more noteworthy. 

\end{comment}

==> oldrq/rq2_old.tex <==



\begin{figure*}[h]
    \centering
    \includegraphics[width=8cm, height= 10cm]{pics/avetest_partial_All_rq1_violin.pdf}
    \caption{The distribution of \ntave{} with different execution strategies}
    \label{fig:nti_box}
\end{figure*}

\input{tables/rq2_patchratio}

\begin{figure*}[htbp]
\centering
\subfigure[\stopppatch{}]{
\includegraphics[scale=0.17]{pics/avetest_partial_StopP_rq1_violin.pdf}
%width=7cm, height=2.5cm
%\caption{fig1}
}
\quad
\subfigure[\plausiblepatch]{
\includegraphics[scale=0.17]{pics/avetest_partial_Plausible_rq1_violin.pdf}
%width=7cm, height=2.3cm
}
\caption{The distribution of \ntave{} with different execution strategies on different patch categories}\label{fig:ntacc_group}
\end{figure*}

\subsection{RQ2: Individual Impact on Each Patch}~\label{sec:rq2}
As discussed in RQ1, the  impact  of test execution strategies on  overall patch validation efficiency is the accumulation of its impact on each patch. Therefore, besides the total number of patches, the overall impact is also dependent on the individual impact on each patch. We present the distribution of the \nti{} (i.e., the number of test executions on each patch) with different execution strategies on all the studied APR systems in Figure~\ref{fig:nti_box}. However, unlike \ntacc{}, \nti{} is in a extremely skewed distribution, i.e., \nti{} of most patches is near one. In other words, on most patches, their validation aborts after only one test execution. As defined in Section~\ref{sec:bond},  \stopfpatch{} is a patch whose validation aborts by an originally-failed test, \stopppatch{} is a patch whose validation aborts by an originally-pass test, and \plausiblepatch{} is a patch whose validation successfully terminates with all the originally-failed/pass tests passing. We further present the ratio of different patch categories generated by each APR system in Table~\ref{tab:patch_ratio}.

\textbf{Finding5: a very large ratio of compilable patches generated by existing APR systems still fail on the originally-failed tests, and constraint-based APR systems generate a higher ratio of patches that can pass originally-failed tests.} Based on Table~\ref{tab:patch_ratio}, existing APR systems exhibit a extremely high ratio (e.g., around 90\%) of \stopfpatch{}; and \stopppatch{} or \plausiblepatch{} are very sparse in the space of compilable patches. Liu et al.~\cite{DBLP:conf/icse/0001WKKB0WKMT20} empirically compared the number of all validated patches, un-compilable patches, and inplausible patches generated by different APR systems, and their work suggested that the state-of-the-art APR techniques can avoid generating un-compilable patches. Our work first investigates the ratio of different patch categories according to the test execution information (e.g., whether the originally-failed tests become pass). In addition, our results suggest that more efforts should be put to generating less \stopfpatch{}; otherwise, unnecessary costs would be spent on compiling and validating these patches. Furthermore, we find that the two constraint-based APR systems (e.g., \dynamoth{} and \acs{}) generate a smaller number of patches but exhibit a lower ratio of \stopfpatch{}.  It indicates that the patches generated by constraint-based APR systems have stronger capability of passing the originally-failed test (i.e., \stopppatch{} or \plausiblepatch{}). One potential reason might be that constraint-based APR systems target at fixing conditional expressions, which are more likely to impact the test execution outcomes, i.e., making the originally-failed test become pass. In addition, \acs{} designs ranking strategies on fixing ingredients for condition synthesis, which brings the validation of the plausible patch forward and reduces the ratio of \stopfpatch{} being validated. 

\textbf{Finding6: execution strategies have large impact on  \plausiblepatch{} and \stopppatch{}, and the APR systems with more \plausiblepatch{} and \stopppatch{} are more susceptible to execution strategies.} 
Figure~\ref{fig:nti_box} presents the distribution of \nti{} with different strategies on \stopfpatch{} and \stopppatch{}, respectively. Here we leave out the results on \stopfpatch{} because as analyzed in Section~\ref{sec:bound}, no difference would be introduced on this type of patches. Compared to the overall distribution over all patches (i.e., Figure~\ref{fig:ntacc_box}), the impact of test execution strategies on  each \plausiblepatch{} or each \stopppatch{} is more noteworthy. Especially on \plausiblepatch{}, the gap between different \rts{} strategies are even wider. As shown in the boundary analysis in Section~\ref{sec:bound}, the impact  is \pTdelta{} on each \plausiblepatch{} and is \pTdeltaexe{} on each \stopppatch{}. Therefore, when the APR system generates more \plausiblepatch{} or \stopppatch{}, it is more susceptible to \rts{} strategies. 
%add an example, explain why rts is so related to patch type/ or move theorical analysis to here


\textbf{Finding7: practical impact is far from its upper bound.}
Our experiment adopts the early exit mechanism and thus the impact is based on the partial matrix of patch executions (i.e., \textit{practical impact}). We further investigate the impact without the early exit mechanism, i.e., continuing each patch validation even when there are test failures. Based on such a full matrix of patch executions, the difference of the number of test executions per patch with different \rts{} strategies can represent the upper bound of impact (i.e., $NPC\times{}|$\pTdelta{}$|$ as analyzed in Section~\ref{sec:bound}).
In Table~\ref{table:full_avet}, for each APR system, the first and the second rows present the average number of test executions on each patch (i.e., \ntave{}) with partial and full matrix, respectively. 
Comparing \ntave{} between different execution strategies, we find that the practical impact of test execution strategies is still far from its upper bound and the upper bound of the impact between \rtsmethod{} and \rtsstate{} is much smaller than that between \rtsmethod{} and \rtsclass{}. 

In addition, we find that the upper bound varies among different subjects. We further collect the code scale of the code elements that modified by the validated patches in different subjects.  In Table~\ref{tab:codelements}, the column ``class'' presents the number of methods contained by the modified classes,  ``method'' presents the number of statements contained by the modified methods per patch, and ``statement'' presents the number of statements modified by per patch. As suggested by the table, when the APR system modifies the more statements that are located in larger scale methods or classes, its upper bound of impact is likely to be higher. 
%\yiling{add some examples based on Table~\ref{table:full_avet} and Table~\ref{tab:codelements}}

\input{tables/rq2_fullmatrix}
\input{tables/rq2_codeelements}


\begin{comment}
We first present the average number of test executions per patch (i.e., \ntave{}) with different \rts{} strategies on all the studies APR systems in Table~\ref{table:all_at_HSD}. For each subject and each APR system,  the columns ``No'', ``Class'', ``Method'', and ``State'' refer to adopting no \rts{}, and \rts{} strategies at the granularities of class, method, and statement, respectively. For example, \prapr{} executes 82.89 tests per patch when  there is no \rts{} adopted during patch validation on the subject Lang.
Overall, we can observe that the number of test executions vary across different \rts{} settings, indicating the \rts{} strategies indeed impact the patch validation efficiency. 
To further confirm our observation, we perform one-way ANOVA analysis~\cite{} at the significance level of 0.05 to investigate whether the \rts{} strategies incur any significant difference on the number of test executions. Furthermore, considering there are multiple groups for multiple test, we perform Tukey HSD post-hoc test~\cite{} to rank the number of test executions when regarding different \rts{} strategies as different groups. 
We further present the statistical analysis results in Table~\ref{table:all_at_HSD}. In the row of each APR system, besides the first sub-row which refers to the number of test executions per patch, the second sub-row refers to the detailed Tukey HSD grouping results (“a” means the group with the largest number of test executions) on using different \rts{} strategies; we also append the number of validated patches per buggy version (i.e., \#patch) and the one-way ANOVA analysis results (i.e., \textit{pvalue}) in the third sub-row. Note that some cells are incomplete since APR system is not applicable to the subject or there is no sufficient or valid sample for statistical analysis. Based on the table, we have the following findings.

% 58
% aaaa: 18
% ab: 26
% abc: 11
% abcd: 3 
\textbf{Finding 1: it is necessary to adopt \rts{}.} At most cases (68.98\%), compared to no \rts{}, adopting any arbitrary \rts{} strategy can significantly reduce the number of test executions during patch validation (rejecting the NULL hypothesis of one-way ANOVA analysis by \textit{p < 0.05}). For example, \arja{} executes 250.72 tests per patch without any \rts{} strategy, but only 1.43 tests are executed when integrating statement-level RTS strategy, i.e., 175.33X speed up regarding to the number of test executions. For the remaining cases (i.e., 31.03\%) that there is no significant difference, we can still observe a drastic reduction of the average test executions after \rts{} adoption. For example, \simfix{} validates 593 patches in total for all the buggy versions of the subject Time. Among the 591 out of 593 patches, only one test is executed no matter with or without \rts{}, while for the remaining 2 patches, \simfix{} without \rts{} executes extremely large number of tests (i.e., 4014 and 3849), and these two exceptional points lift the average number of test executions to 126.87. Overall, \rts{} has a huge impact on patch validation efficiency, and thus future work in APR should no longer overlook \rts{} strategies during the patch validation phase.

\textbf{Finding 2: impact of different \rts{} strategies.} We can observe that at some cases (7.50\%), different \rts{} strategies perform significantly differently. In particular, \rtsstate{} executes the least tests per patch while \rtsclass{} explores the  most test executions. This is not surprising since class-level coverage is the coarsest selection criterion to execute more tests.
It is notable that at most cases (65.00\%), there is no significant difference caused by different \rts{} strategies and at some cases (27.50\%), \rtsmethod{} and \rtsstate{} are executing quite closing number of tests but \rtsclass{} remarkably executes much more tests.
In other words, the impact of the \rts{} strategy varies in different cases (i.e., subjects and APR systems) and we would analyze the factors behind in the following research questions. 



\textbf{Observation 3: impact on different APR systems.} The overall trends are similar on different APR systems in terms of the impact of \rts{}. In addition, within the same subject, we can observe the detailed number of test executions vary among different APR systems. For example, even without any \rts{} strategy, \kpar{} (e.g., 212.5 tests on Math) takes much more tests than \avatar{} (e.g., 122.45 tests on Math), although \kpar{} generates less patches than \avatar{}.
This observation suggests that the number of patches cannot sufficiently indicate the efficiency of patch validation phases, which is the main indicator used in the previous work on APR efficiency. Therefore, it is necessary to investigate the patch validation efficiency in terms of the number of test executions.

\textbf{Observation 4: impact on different subjects.} Although we can find the first two observations still hold almost in every subject, it is interesting to notice that on several subjects there are some counter examples. For example, in Chart, the difference between \rtsstate{} and \rtsmethod{} is very small and even zero sometimes (e.g., in \simfix{}, \avatar{}, or \kpar{}), indicating that in these subjects the strategies of \rts{} induce no impact at all. In addition, even across different subjects, the average number of test executions with \rts{} at finer granularities (e.g., \rtsstate{} or \rtsmethod{}) are quite closing, while they are very different with \rtsclass{} or without \rts{}.  For example, with \rtsstate{}, \kali{} executes 1.21, 1.25, and 1.29 tests per patch on the subjects Lang, Math, and Time, respectively, while  \kali{} executes 113.57, 177.09, and 47.41 tests without \rts{}.




\subsection{RQ3: impact on different patches and bugs} ~\label{sec:rq2}
According to the analysis above, the ratio of different types of patches is one of the factors that might affect the impact of \rts{} on the patch validation efficiency.  
Therefore, we further analyze the ratio of different patch categories to help understand the difference in the number of executed tests caused by \rts{}.

% the difference on different patch group
First, we can observe that the impact of \rts{} on patches of different types is significantly different. For example, all APR systems execute more tests on plausible patches than on other patches, and the impact of \rts{}  on plausible patches is much larger than that on other patches. For example, \prapr{} with \rtsstate{} executes 162.43 tests per plausible patch but it only executes 1.18 patches per non-plausible patch; in addition, \prapr{} with no \rts{} executes 10.27 more tests than \rtsstate{} per non-plausible patch, but \prapr{} with no \rts{} executes 2,963.83 more tests than \rtsstate{} per plausible patch.
% add an example, why rts is so related to patch type

Second, based on the observation above, we can find that for different APR systems, the impact of \rts{} is significantly related to the ratio of different patch types. For example, \prapr{} executes 

% for different apr systems, the impact is different because the ratio of different patch is different; correlation analysis: ratio of patch v.s. impact of RTS



\parabf{Finding 1.2: \rts{} can potentially improve the effectiveness of APR systems for the bugs which have no plausible patches currently.} 
We further investigate the impact of \rts{} on the patch validation efficiency of the bugs with/without plausible patches separately. 
We calculate the total number of test executions on all the patches generated in each buggy version, and present the average number of buggy versions with/without plausible patches in Table~\ref{table:all_test_plausible} and Table~\ref{table:all_test_nonplausible} respectively. 
For the bugs with/without plausible patches, we can observe there is a consistent difference in terms of the total test executions between using \rts{} or not (e.g., extra thousands of test executions).  
In particular, for the bugs that cannot be plausibly fixed by some APR systems (e.g., \arja{}, \genprog{}, and \arja{}), even hundreds of thousands of tests are unnecessarily executed. Considering currently most APR systems usually set time budget for the whole  APR process and abort fixing the bug when the time is exhausted. It implies that, for these bugs, plausible patches might be generated when \rts{} is adopted,  since the patch validation phase would be accelerated to a large extent. \yiling{TODO: merge the four tables~\ref{table:all_test_plausible},~\ref{table:all_test_nonplausible}, ~\ref{table:ave_test_nonplausible}, ~\ref{table:ave_test_plausible} into a big one}


\textbf{Finding 2.1: for all APR systems and subjects, \rtsclass{} significantly execute more tests than \rtsmethod{} and \rtsstate{} during patch validation.}

Secondly, among different APR systems, we observe inconsistent increase in terms of the number of executed tests from \rtsstate{} to \rtsmethod{}. After investigation, we find there might be two  reasons accounting for the inconsistence among different APR systems.
Firstly, the difference of the number of executed tests between \rtsmethod{} and \rtsstate{} is larger for those APR systems that generate multi-locations patches.  For example, for each  \stopppatch{} in Math, \arja{} executes 22.17 originally-passed tests on average while \prapr{} only execute 2.39 originally-passed tests, even they execute similar number of tests 
\end{comment}

==> oldrq/rq3.tex <==




\subsection{RQ4: Impact with the Full Matrix}~\label{sec:rq4}
In previous research questions, we investigate the impact of test selection with the partial validation matrix ($\pMatrixpart{}$), i.e., the early-exit mechanism is enabled and the validation for each patch would be terminated after any test failure. In this RQ, we further study the impact of RTS with the full matrix ($\pMatrixfull{}$), i.e., the validation for each patch would continue even when there are failed tests. A full validation matrix is common in the scenario that execution results of all tests are required, such as  unified debugging~\cite{DBLP:journals/ac/Lou0ZH19, benton2020effectiveness}.







Table~\ref{table:rq3_fullmatrix} shows the accumulated number of test executions $\testnum\pMatrixfull{}$ on each APR system. For space limits, we present the average number of all subjects and buggy versions. It is notable that the full patch validation matrix collection is extremely resource consuming, e.g., from thousands to millions of tests are executed when there is no RTS. 
We can observe a prominent reduction when RTS strategies at finer granularities are integrated in APR systems. For example, on average, \rtsstate{} even reduces millions of test executions for \prapr{}.
%In addition, the number of test executions among APR systems is remarkably different, e.g., \prapr{} executes over twenty millions tests while \acs{} only executes less than one hundred tests on average. 
In summary, our results show that RTS should definitely be applied in the full-matrix scenario.

\finding{\textit{the full validation matrix is extremely resource-consuming, for which RTS has a more remarkable impact by reducing even up to millions of test executions on average.}}

\input{newtables/rq3_fullmatrix_nt}

%Figure~\ref{fig:fulldis} overviews the distribution of test executions with full execution matrix on all studied APR systems.

We further compare the reduction achieved by RTS between full and partial matrices in Figure~\ref{fig:fullpartial}. 
First, the reduction curves of the full matrix are far beyond the partial matrix. For example, with the full matrix, all the RTS strategies can help all APR systems save more than 70\% of test executions. In particular, \rtsstate{} and \rtsmethod{} can save more than 95\% of  test executions at most cases. 
Second, the difference between partial and full matrices varies among different APR systems. For example, \dynamoth{} achieves a slightly larger reduction while \avatar{} achieves a much larger reduction after they switch from partial matrices into full matrices.
\Comment{Third, the reduction curves are more stable among APR systems with the full matrix than with the partial matrix, indicating that RTS plays an essential role in efficiency optimization especially in the full-matrix scenario. }
Furthermore, consistent with the finding for partial matrices, method- and statement-level RTS perform similarly, and both of them substantially outperform class-level RTS. Interestingly, their superiority over class-level RTS is even enlarged with full matrices. 
%Therefore, fine-grained RTS (e.g., \rtsstate{} and \rtsmethod{}) is still more recommended in the full matrix.
In fact, the early-exit mechanism in the partial matrix prevents more tests from executing, which mitigates the impact from test selection strategies. In other words, the reduction achieved in the full-matrix scenario represents the upper bound of the impact.



% talk about the APR system?
\finding{\textit{RTS can remarkably reduce more test executions with full matrices than with partial matrices. Method- and statement-level RTS still perform similarly, but their superiority over class-level RTS is further enlarged with full matrices.  
\Comment{
the difference between different selection strategies is also more prominent with the full matrix. The difference of RTS impact among different APR systems is narrowed when switching from partial to full matrices. } \Comment{The difference among APR systems of the impact caused by RTS strategies, is narrowed when switching from partial matrix to full matrix.}}}

\begin{figure}[htb]
    \centering
   \includegraphics[width=6.5cm, height= 4.3 cm]{new_pics/rq4_fullpartial_summay_line_preplots.pdf}
    \caption{Reduction with full/partial matrices}
    \label{fig:fullpartial}
\end{figure}





\begin{comment}

\input{newtables/rq4_full_partial_summary}
\begin{figure*}[htbp]
\centering
\subfigure[Reduction on No Selection]{
  \includegraphics[width=8.4cm, height= 6.5cm]{new_pics/rq4.png}
%width=7cm, height=2.5cm
}~\label{fig:rq4ab}
\quad
\subfigure[Reduction between Selection Strategies]{
  \includegraphics[width=8.4cm, height= 6.5cm]{new_pics/rq4_rel.png}
%width=7cm, height=2.3cm
}~\label{fig:rq4rel}
\caption{Reduction on with Full Matrix and Partial Matrix }~\label{fig:rq4}
\end{figure*}
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%



==> oldrq/rq3_old.tex <==


\subsection{RQ3: Impact on Different Bugs}~\label{sec:rq3}
Based on the patch categories, we further group bugs into three categories: (1) \textbf{\plausiblebug{}}: at least one plausible patch is generated when the APR system attempts to fix this bug, (2) \textbf{\partialbug{}}: at least one patch that can pass some originally-failed test(s) but not all tests is generated and no plausible patch is generated, (3) \textbf{\nofixbug{}}: no patch that can pass any originally-failed tests is generated.  Table~\ref{table:rq3_bug} presents the reduction of test selection strategies on \plausiblebug{} and \partialbug{}, respectively. 
\input{newtables/rq3_bugs} 

\finding{\textit{ class and statement level test selection strategies can boost APR systems by reducing  nearly 90\% test executions before finding the plausible fix, significantly improving APR efficiency.}}


Based on the table, we can observe a significant reduction achieved by test selection strategies, especially on the \plausiblebug{}s. More than 90\% of test executions are skipped, and in other words, the repair process would be terminate with a plausible patch much earlier if a proper test selection strategy is adopted. In addition, the reduction on \partialbug{}s is also prominent but slightly less remarkable than on \plausiblebug{}s. One potential reason is that the a plausible patch would terminate the repair process, and the ratio of \stopppatch{} and \plausiblepatch{} would be higher on \plausiblebug{}s due to the less number of validated patches. 
As for the impact of different selection strategies, overall we can observe a distinguished difference among strategies on both \plausiblebug{}s and \partialbug{}. It indicates that on the bugs that can be potentially fixed by APR systems, the choice of test selection strategies is important.
In particular, it is notable that the difference between statement and method level strategies on the APR systems \prapr{} and \simfix{} is very smaller (i.e., 2.91\% and 0.00\%) on \partialbug{}s, because these two APR systems both exhibit an extremely low ratio (i.e., 1.49\% and 0.76\%) of \stopppatch{} on their \partialbug{}s. Especially for \simfix{}, all 0.76\% of \stopppatch{} are patching the code in a small-scale method, and thus there is no difference between statement-level and method-level selection strategy.


\input{tables/rq3_ourtool}

\subsection{RQ3: New Test Execution Strategies}~\label{sec:rq3}
The previous RQs suggest that test execution strategies significantly impact the patch validation efficiency and a casual strategy might introduce a huge amount of unnecessary costs in patch validation. Based on our results, test selection strategy at statement-level can remarkably reduce the number of test executions, which should be integrated in the patch validation phase. Therefore, we further propose a new test execution strategy \ourtool{}, which combines statement-level regression test selection and regression test prioritization. For each patch, \ourtool{} first decides the subset of  tests $T'$ to be executed according to statement-level \rts{}; then \ourtool{} adaptively decides the execution order of the tests in $T'$ by their on-the-fly history information. Our intuition is that a test failed on more patches that are more \textit{close} to the current patch has a higher likelihood to fail on the current patch, and therefore executing this test earlier can trigger a failure earlier. Considering APR systems often tentatively fix the code elements according to the fault localization ranking list, we use the patched location to calculate the relevance among patches. Simply speaking, the patches whose patched code locates in the same code element (e.g., class, method, or statement) are regarded as relevant. It also minimizes the  space and time overheads of maintaining the on-the-fly information. We assess the priority of each test according to Equation~\ref{eq:prio}. Here, $P_{rel}(P')$ denotes to all the patches relevant to the current patch $P'$,  $his(P'',t)$ denotes the history information of test $t$ on the patch $P''$, including $Fail$ fail, $Pass$ pass, and $NO$ not executed. $his(P'',t)$ is  empty on the beginning, but would be adaptively updated during the patch validation. 


\begin{equation}\label{eq:prio}
    Prio(t, P') = \frac{\{P'' \in P_{rel}(P') | his(P'',t) = Fail \}}{ \{P'' \in P_{rel}(P')  | his(P'',t) \in \{Fail, Pass\} \}} 
\end{equation}


According to the granularity in relevant patch calculation, \ourtool{} can be configured with statement-level (\ourtoolstate{}), method-level (\ourtoolmethod{}), and class-level (\ourtoolclass{}). For example, \ourtoolstate{} regards the patches modifying the same statements as relevant and \ourtoolclass{} regards the patches modifying the same classes as relevant.

\textbf{Finding 8: the proposed test execution strategy \ourtool{} stably outperforms existing strategies and the acceleration is more remarkable in time consuming fixing cases.} Table~\ref{table:ourtool} present the \ntacc{} of \ourtoolstate{} on each subject and APR system. For comparison, we also present the \ntacc{} of \rtsstate{} and the state-of-the-art test prioritization approach for patch validation \trp{}~\cite{}. In particular, \trp{} decides the priority of each test by its frequency of failing on all history validated patches. On all APR systems and subjects, \ourtoolstate{} can consistently reduce more test executions than both  \rtsstate{}{} and \trp{}. The acceleration is more remarkable especially in the time-consuming cases that more patches and tests are executed. For example, when \prapr{} attempts to fix the bugs in Closure, \ourtool{} can further reduce 5395.20 test executions (24.31\% reduction) than \rtsstate{} strategy. Meanwhile, the benefits from the proposed strategy is weak in the cases that only small number of patches are generated for validation and when the most patches belong to \stopfpatch{}. 





==> oldrq/rq4.tex <==
\subsection{RQ5: Test Selection+Prioritization}~\label{sec:rq5}

\input{newtables/rq4_rtp_rts}


So far we have studied the impact of RTS strategies on APR efficiency controlled in a default test execution order (i.e., the lexicographic order), and our results suggest that test selection can largely reduce the number of test executions and improve APR efficiency. In fact, when the early-exit mechanism is enabled (the default setting for all modern APR systems), the test execution order can also affect the final number of test executions since it decides when the first failure-triggering test would be executed. Therefore, in this RQ, we further combine studied RTS strategies with different test prioritization strategies and study their joint impact on APR efficiency. For each patch, we apply RTS to decide the tests for execution and apply test prioritization to decide their execution order.
We still follow the common practice of all recent APR systems that all the originally-failed tests are executed before all the originally-passed tests, because the former are more likely to fail again on patches. 
Within the originally-failed tests or the originally-passed tests, we further apply the following test prioritization strategies to schedule their execution order. 
\begin{itemize}[leftmargin=10pt, itemindent=0pt, topsep=0pt]
    \item \textbf{Baseline prioritization.} Tests are scheduled by their lexicographic order, which is also the default setting in previous RQs. We denote this prioritization strategy as \priodefault{}.
    \item \textbf{Patch-history-based prioritization.} Qi~\etal{} proposed \trp{}~\cite{DBLP:conf/icsm/QiML13}, a prioritization strategy based on the patch execution history. 
    \trp{} considers the tests that have failed on more validated patches as more likely to fail on the current patch and assigns them a higher execution priority.
    We consider \trp{} since it is the state-of-the-art test prioritization strategy specifically designed for APR, and we make the first attempt to study the performance of its combination with RTS. We denote this prioritization strategy as \priotrp{}.
    \item \textbf{Regression test prioritization.} 
    Test prioritization techniques have also been widely studied in traditional regression testing to reorder regression tests for early detection of regression bugs~\cite{DBLP:journals/tse/LiHH07, DBLP:journals/ac/Lou0ZH19, DBLP:conf/sigsoft/WangNT17}. \Comment{RTP schedules the execution order of regression test cases to advance the time of failure exposure, which can be naturally adopted to boost patch validation.} 
    Since each patch can be treated as a new revision in regression testing, we can also naturally apply regression test prioritization techniques for APR. Note that, surprisingly, we are the first to study regression test prioritization for APR. In particular, we consider two most widely studied approaches, i.e., the \emph{total} and \emph{additional} regression test prioritization techniques based on statement coverage~\cite{DBLP:conf/icsm/RothermelUCH99}. They share the similar intuition that tests covering more statements or more yet-uncovered statements are more likely to detect regression bugs. We denote them as \priototal{} and \prioadd{}, respectively.
 
\end{itemize}


In Table~\ref{table:rq4_combine},  we present the reductions achieved by the combination of different test selection and prioritization strategies when compared to \norts{} with \priodefault{}. The highest reduction within each RTS strategy is highlighted. Based on the table, we have the following observations. 
First, combining test selection with test prioritization can further improve  APR efficiency. However, compared to test selection, test prioritization brings much lower reduction ratios.\Comment{strategies bring smaller benefits in terms of the reduction ratio. In other words, the pure reduction from prioritization is much smaller than from RTS.} For example, when \prapr{} adopts no RTS, the best prioritization (i.e., \prioadd{}) can achieve only 15.21\% reduction, but the worst RTS alone (i.e., \rtsclass{} with \priodefault{}) can achieve 36.96\% reduction. 
\Comment{Furthermore, given a RTS strategy, the reduction differences among different prioritization strategies are often within 1\%. }
This indicates that test selection strategies play a more essential role in efficiency optimization.
Second, the best prioritization strategy varies when combined with different RTS strategies. For most APR systems, surprisingly, \prioadd{} reduces the most test executions when combined with \norts{}, \rtsclass{}, or \rtsmethod{}.
To the best of our knowledge, this is the first study demonstrating that in the APR scenario, the traditional additional prioritization technique even outperforms state-of-the-art APR-specific prioritization technique at the most cases\Comment{ (e.g., without RTS and with coarse-grained RTS)}.
One potential reason may be that the generated patches share little commonality and it is challenging for \priotrp{} to infer the results of un-executed patches from historical patch executions. In contrast, \prioadd{} executes tests with diverse statement coverage as early as possible and thus can advance buggy patch detection.
Furthermore,  it is notable that \prioadd{} becomes less effective than \priotrp{} when combined with \rtsstate{}. 
Intuitively, the tests selected by coarser-grained coverage criteria (e.g., class-level RTS) tend to exhibit a more diverse distribution of statement coverage than the tests selected by the statement-level RTS. Therefore, when combined with \rtsstate{}, \priotrp{} has a stronger capability in distinguishing tests based on their historical execution results.
Third, we can observe that \prioadd{} outperforms \priototal{} in terms of the repair efficiency, which is consistent with the previous findings in traditional regression testing\Comment{, i.e., the additional strategy usually outperforms the total strategy}~\cite{DBLP:conf/icse/LuLCZHZ016, DBLP:conf/icsm/RothermelUCH99}. 


\finding{\textit{ 
this study demonstrates for the first time that test selection outperforms test prioritization for APR, and they can be combined to further improve APR efficiency. Also, surprisingly, traditional regression test prioritization \prioadd{} outperforms state-of-the-art APR-specific test prioritization \priotrp{} for most cases.}}






\begin{comment}


\textbf{Test prioritization strategies.}
Similar as regression test prioritization, the purpose of scheduling the test execution order in patch validation is to execute to failure-triggering test as earlier as possible so that the validation process can immediately switch to the next patch. Before our study, Chen et al.~\cite{} proposed a test prioritization approach \trp{} for patch validation. In particular, \trp{} decides the priority of each test by its frequency of failing on all history validated patches. \trp{} is designed based on the intuition that a test failed more frequently in history is more likely to fail on the next patch. We further refine the intuition by considering a test that fails more frequently on the patches \textit{similar} to the current patch with a higher likelihood to fail on the current patch. 
Considering APR systems often tentatively fix the code elements according to the fault localization ranking list, we use the patched code location to measure the similarity among patches. 
Simply speaking, the patches whose patched code locates in the same code element (e.g., class, method, or statement) are regarded as similar. 
We assess the priority of each test according to Equation~\ref{eq:prio}. Here, $P_{rel}(P')$ denotes to all the patches similar as the current patch $P'$,  $his(P'',t)$ denotes the history information of test $t$ on the patch $P''$, including $Fail$ fail, $Pass$ pass, and $NO$ not executed. $his(P'',t)$ is empty on the beginning, but would be adaptively updated during the patch validation. 

\begin{equation}\label{eq:prio}
    Prio(t, P') = \frac{\{P'' \in P_{rel}(P') | his(P'',t) = Fail \}}{ \{P'' \in P_{rel}(P')  | his(P'',t) \in \{Fail, Pass\} \}} 
\end{equation}


According to the granularity in similar patch calculation, the test prioritization can be configured with statement, method, class, and global levels. Here global level refers to all history patches (i.e.g., the setting of \trp{}), and for example, statement-level prioritization regards the patches modifying the same statements as similar.


\textbf{Combination of test selection and test prioritization.}
Based on our results in previous RQs, test selection strategy at statement-level can remarkably reduce the largest number of test executions, which is the best choice for patch validation. Therefore, we combine the statement-level test selection strategy with four prioritization strategies respectively, denoting them as \ourtoolglobal{}, \ourtoolclass{}, \ourtoolmethod{}, and \ourtoolstate{}.
In particular, for each patch,  statement-level test selection strategy first decides the subset of tests $T'$ to be executed; second, the test prioritization strategy adaptively decides the execution order of tests in $T'$ by their on-the-fly history information. 

\finding{combining test selection and prioritization can further reduce the number of test executions and the acceleration is more remarkable in time consuming fixing cases.}

Table~\ref{table:ourtool} present the \ntacc{} of \ourtoolstate{} on each subject and APR system. For comparison, we also present the \ntacc{} of \rtsstate{} and the state-of-the-art test prioritization approach for patch validation \trp{}~\cite{}. In particular, \trp{} decides the priority of each test by its frequency of failing on all history validated patches. On all APR systems and subjects, \ourtoolstate{} can consistently reduce more test executions than both  \rtsstate{}{} and \trp{}. The acceleration is more remarkable especially in the time-consuming cases that more patches and tests are executed. For example, when \prapr{} attempts to fix the bugs in Closure, \ourtool{} can further reduce 5395.20 test executions (24.31\% reduction) than \rtsstate{} strategy. Meanwhile, the benefits from the proposed strategy is weak in the cases that only small number of patches are generated for validation and when the most patches belong to \stopfpatch{}. 

\input{newtables/rq5_combine}
\input{tables/rq3_ourtool}

\end{comment}

==> oldrq/rq4_old.tex <==
\subsection{RQ4: Impact on Time Cost}~\label{sec:rq3}
In the research questions, we mainly measure the impact of \rts{} in terms of the number of test executions. Considering that the execution time vary among tests and the patch validation costs also consist of patch compilation and test loading test besides test execution time, we further investigate the overall patch validation time of each buggy version with different \rts{} strategies. 


\input{tables/rq4_timecost}

==> tables/All_ave_latex_table.tex <==
\begin{table*}
    \centering
   \caption{(AllBug) Average executed tests with different \rts{} on all APR systems  }\label{table:all_at_summary}
   	\begin{adjustbox}{width=2.1\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 

Lang&NORTS&400.66&400.66&100.00&82.89&80.79&80.79&100.00&66.79&10.63&10.63&100.00&77.84&11.00&11.00&100.00&127.94&10.93&10.93&100.00&219.31&10.88&10.88&100.00&197.21&1.43&1.43&100.00&1256.43&1.00&1.00&100.00&608.00&900.67&900.67&100.00&250.72&47.69&47.69&100.00&113.57&1083.03&1083.03&100.00&136.10&498.11&498.11&100.00&71.01\\ \hline
Lang&CLASS&400.66&400.66&100.00&2.16&80.79&80.79&100.00&1.96&10.63&10.63&100.00&2.77&11.00&11.00&100.00&7.88&10.93&10.93&100.00&8.81&10.88&10.88&100.00&8.57&1.43&1.43&100.00&25.29&1.00&1.00&100.00&17.00&900.67&900.67&100.00&11.62&47.69&47.69&100.00&3.67&1083.03&1083.03&100.00&4.14&498.11&498.11&100.00&2.14\\ \hline
Lang&METHOD&400.66&400.66&100.00&1.30&80.79&80.79&100.00&1.22&10.63&10.63&100.00&1.25&11.00&11.00&100.00&1.48&10.93&10.93&100.00&1.29&10.88&10.88&100.00&1.57&1.43&1.43&100.00&2.43&1.00&1.00&100.00&1.00&900.67&900.67&100.00&1.54&47.69&47.69&100.00&1.33&1083.03&1083.03&100.00&1.30&498.11&498.11&100.00&1.20\\ \hline
Lang&STATE&400.66&400.66&100.00&1.15&80.79&80.79&100.00&1.19&10.63&10.63&100.00&1.17&11.00&11.00&100.00&1.46&10.93&10.93&100.00&1.17&10.88&10.88&100.00&1.47&1.43&1.43&100.00&1.57&1.00&1.00&100.00&1.00&900.67&900.67&100.00&1.43&47.69&47.69&100.00&1.21&1083.03&1083.03&100.00&1.28&498.11&498.11&100.00&1.08\\ \hline
Math&NORTS&1513.39&1513.39&100.00&121.61&35.90&35.90&100.00&384.69&7.39&7.39&100.00&122.45&6.48&6.48&100.00&212.55&6.26&6.26&100.00&459.73&6.18&6.18&100.00&229.94&1.21&1.21&100.00&1891.11&1.67&1.67&100.00&788.67&837.59&837.59&100.00&406.64&11.49&11.49&100.00&177.09&893.95&893.95&100.00&221.55&433.24&433.24&100.00&113.12\\ \hline
Math&CLASS&1513.39&1513.39&100.00&3.57&35.90&35.90&100.00&66.56&7.39&7.39&100.00&2.61&6.48&6.48&100.00&40.86&6.26&6.26&100.00&8.62&6.18&6.18&100.00&3.09&1.21&1.21&100.00&43.46&1.67&1.67&100.00&5.67&837.59&837.59&100.00&12.58&11.49&11.49&100.00&2.78&893.95&893.95&100.00&8.12&433.24&433.24&100.00&3.07\\ \hline
Math&METHOD&1513.39&1513.39&100.00&1.29&35.90&35.90&100.00&11.41&7.39&7.39&100.00&1.55&6.48&6.48&100.00&1.76&6.26&6.26&100.00&2.52&6.18&6.18&100.00&1.67&1.21&1.21&100.00&26.24&1.67&1.67&100.00&5.67&837.59&837.59&100.00&3.74&11.49&11.49&100.00&1.73&893.95&893.95&100.00&2.76&433.24&433.24&100.00&1.62\\ \hline
Math&STATE&1513.39&1513.39&100.00&1.12&35.90&35.90&100.00&11.04&7.39&7.39&100.00&1.16&6.48&6.48&100.00&1.37&6.26&6.26&100.00&1.60&6.18&6.18&100.00&1.02&1.21&1.21&100.00&20.93&1.67&1.67&100.00&1.00&837.59&837.59&100.00&2.23&11.49&11.49&100.00&1.25&893.95&893.95&100.00&1.77&433.24&433.24&100.00&1.10\\ \hline
Time&NORTS&1466.54&1466.54&100.00&40.63&53.91&53.91&100.00&126.87&5.91&5.91&100.00&354.03&4.73&4.73&100.00&1.00&5.27&5.27&100.00&354.82&3.50&3.50&100.00&487.50&2.00&2.00&100.00&1302.67&1.00&1.00&100.00&1.00&794.00&794.00&100.00&44.51&34.40&34.40&100.00&47.41&989.60&989.60&100.00&118.35&279.40&279.40&100.00&4.52\\ \hline
Time&CLASS&1466.54&1466.54&100.00&4.50&53.91&53.91&100.00&7.44&5.91&5.91&100.00&76.55&4.73&4.73&100.00&1.00&5.27&5.27&100.00&76.55&3.50&3.50&100.00&104.88&2.00&2.00&100.00&536.33&1.00&1.00&100.00&1.00&794.00&794.00&100.00&10.25&34.40&34.40&100.00&23.87&989.60&989.60&100.00&24.74&279.40&279.40&100.00&1.53\\ \hline
Time&METHOD&1466.54&1466.54&100.00&1.24&53.91&53.91&100.00&1.85&5.91&5.91&100.00&2.27&4.73&4.73&100.00&1.00&5.27&5.27&100.00&2.27&3.50&3.50&100.00&2.75&2.00&2.00&100.00&7.67&1.00&1.00&100.00&1.00&794.00&794.00&100.00&5.75&34.40&34.40&100.00&1.77&989.60&989.60&100.00&9.03&279.40&279.40&100.00&1.20\\ \hline
Time&STATE&1466.54&1466.54&100.00&1.18&53.91&53.91&100.00&1.18&5.91&5.91&100.00&2.27&4.73&4.73&100.00&1.00&5.27&5.27&100.00&2.27&3.50&3.50&100.00&2.75&2.00&2.00&100.00&7.67&1.00&1.00&100.00&1.00&794.00&794.00&100.00&3.06&34.40&34.40&100.00&1.29&989.60&989.60&100.00&1.76&279.40&279.40&100.00&1.02\\ \hline
Chart&NORTS&784.88&784.88&100.00&42.81&68.43&68.43&100.00&45.64&6.58&6.58&100.00&219.45&6.33&6.33&100.00&101.91&5.79&5.79&100.00&362.76&6.59&6.59&100.00&96.53&1.00&1.00&100.00&1640.80&nan&nan&nan&nan&682.35&682.35&100.00&309.25&48.14&48.14&100.00&171.42&760.12&760.12&100.00&155.70&347.04&347.04&100.00&52.81\\ \hline
Chart&CLASS&784.88&784.88&100.00&4.58&68.43&68.43&100.00&3.54&6.58&6.58&100.00&2.27&6.33&6.33&100.00&2.29&5.79&5.79&100.00&3.82&6.59&6.59&100.00&1.53&1.00&1.00&100.00&77.30&nan&nan&nan&nan&682.35&682.35&100.00&29.51&48.14&48.14&100.00&11.84&760.12&760.12&100.00&12.22&347.04&347.04&100.00&3.87\\ \hline
Chart&METHOD&784.88&784.88&100.00&1.33&68.43&68.43&100.00&3.06&6.58&6.58&100.00&1.24&6.33&6.33&100.00&1.18&5.79&5.79&100.00&1.39&6.59&6.59&100.00&1.00&1.00&1.00&100.00&16.70&nan&nan&nan&nan&682.35&682.35&100.00&5.27&48.14&48.14&100.00&1.88&760.12&760.12&100.00&3.81&347.04&347.04&100.00&1.39\\ \hline
Chart&STATE&784.88&784.88&100.00&1.32&68.43&68.43&100.00&3.06&6.58&6.58&100.00&1.24&6.33&6.33&100.00&1.18&5.79&5.79&100.00&1.39&6.59&6.59&100.00&1.00&1.00&1.00&100.00&16.30&nan&nan&nan&nan&682.35&682.35&100.00&2.58&48.14&48.14&100.00&1.79&760.12&760.12&100.00&2.59&347.04&347.04&100.00&1.26\\ \hline
Mockito&NORTS&2307.92&2307.92&100.00&9.97&nan&nan&nan&nan&3.75&3.75&100.00&233.75&4.80&4.80&100.00&8.29&4.33&4.33&100.00&196.93&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&2307.92&2307.92&100.00&1.46&nan&nan&nan&nan&3.75&3.75&100.00&90.16&4.80&4.80&100.00&5.24&4.33&4.33&100.00&143.13&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&2307.92&2307.92&100.00&1.28&nan&nan&nan&nan&3.75&3.75&100.00&4.78&4.80&4.80&100.00&1.20&4.33&4.33&100.00&44.67&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&2307.92&2307.92&100.00&1.28&nan&nan&nan&nan&3.75&3.75&100.00&4.53&4.80&4.80&100.00&1.20&4.33&4.33&100.00&4.00&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&14725.00&14725.00&100.00&221.41&5.71&5.71&100.00&3106.31&3.94&3.94&100.00&246.71&3.62&3.62&100.00&343.70&3.90&3.90&100.00&469.82&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&14725.00&14725.00&100.00&90.36&5.71&5.71&100.00&1662.97&3.94&3.94&100.00&69.98&3.62&3.62&100.00&142.52&3.90&3.90&100.00&190.08&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&14725.00&14725.00&100.00&12.64&5.71&5.71&100.00&321.93&3.94&3.94&100.00&2.50&3.62&3.62&100.00&7.04&3.90&3.90&100.00&3.66&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&14725.00&14725.00&100.00&1.87&5.71&5.71&100.00&123.59&3.94&3.94&100.00&1.27&3.62&3.62&100.00&1.16&3.90&3.90&100.00&1.45&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&3533.06&3533.06&100.00&86.55&48.95&48.95&100.00&746.06&6.37&6.37&100.00&209.04&6.16&6.16&100.00&132.57&6.08&6.08&100.00&343.90&5.78&5.78&100.00&168.86&1.41&1.41&100.00&1522.75&1.22&1.22&100.00&465.89&803.65&803.65&100.00&252.78&35.43&35.43&100.00&127.37&931.68&931.68&100.00&157.92&389.45&389.45&100.00&60.36\\ \hline
All &CLASS&3533.06&3533.06&100.00&17.77&48.95&48.95&100.00&348.49&6.37&6.37&100.00&40.72&6.16&6.16&100.00&33.30&6.08&6.08&100.00&71.83&5.78&5.78&100.00&20.01&1.41&1.41&100.00&170.60&1.22&1.22&100.00&7.89&803.65&803.65&100.00&15.99&35.43&35.43&100.00&10.54&931.68&931.68&100.00&12.31&389.45&389.45&100.00&2.65\\ \hline
All &METHOD&3533.06&3533.06&100.00&3.18&48.95&48.95&100.00&67.89&6.37&6.37&100.00&2.27&6.16&6.16&100.00&2.28&6.08&6.08&100.00&9.30&5.78&5.78&100.00&1.50&1.41&1.41&100.00&13.26&1.22&1.22&100.00&2.56&803.65&803.65&100.00&4.07&35.43&35.43&100.00&1.68&931.68&931.68&100.00&4.22&389.45&389.45&100.00&1.35\\ \hline
All &STATE&3533.06&3533.06&100.00&1.32&48.95&48.95&100.00&28.01&6.37&6.37&100.00&1.94&6.16&6.16&100.00&1.23&6.08&6.08&100.00&1.98&5.78&5.78&100.00&1.37&1.41&1.41&100.00&11.62&1.22&1.22&100.00&1.00&803.65&803.65&100.00&2.33&35.43&35.43&100.00&1.39&931.68&931.68&100.00&1.85&389.45&389.45&100.00&1.12\\ \hline


    \end{tabular}
    \end{adjustbox}
\end{table*} 

\begin{table*}
    \centering
   \caption{Full-(AllBug) Average executed tests with different \rts{} on all APR systems  }\label{table:full_all_at_summary}
   	\begin{adjustbox}{width=2.1\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 

Lang&NORTS&376.83&376.83&100.00&1866.29&79.40&79.40&100.00&1854.58&10.63&10.63&100.00&1793.33&11.04&11.04&100.00&1801.89&10.78&10.78&100.00&1793.33&10.54&10.54&100.00&1796.54&1.43&1.43&100.00&1753.57&1.00&1.00&100.00&2133.00&830.22&830.22&100.00&1942.56&46.94&46.94&100.00&1944.46&1058.89&1058.89&100.00&1942.56&468.53&468.53&100.00&1942.56\\ \hline
Lang&CLASS&376.83&376.83&100.00&73.85&79.40&79.40&100.00&62.76&10.63&10.63&100.00&52.35&11.04&11.04&100.00&54.13&10.78&10.78&100.00&52.93&10.54&10.54&100.00&55.77&1.43&1.43&100.00&37.00&1.00&1.00&100.00&69.33&830.22&830.22&100.00&66.88&46.94&46.94&100.00&59.15&1058.89&1058.89&100.00&69.07&468.53&468.53&100.00&66.85\\ \hline
Lang&METHOD&376.83&376.83&100.00&15.05&79.40&79.40&100.00&11.10&10.63&10.63&100.00&6.60&11.04&11.04&100.00&7.06&10.78&10.78&100.00&6.04&10.54&10.54&100.00&6.40&1.43&1.43&100.00&9.57&1.00&1.00&100.00&6.00&830.22&830.22&100.00&10.66&46.94&46.94&100.00&10.53&1058.89&1058.89&100.00&11.00&468.53&468.53&100.00&10.21\\ \hline
Lang&STATE&376.83&376.83&100.00&13.36&79.40&79.40&100.00&9.82&10.63&10.63&100.00&4.18&11.04&11.04&100.00&4.97&10.78&10.78&100.00&4.26&10.54&10.54&100.00&4.07&1.43&1.43&100.00&6.86&1.00&1.00&100.00&4.00&830.22&830.22&100.00&8.61&46.94&46.94&100.00&9.14&1058.89&1058.89&100.00&8.65&468.53&468.53&100.00&8.09\\ \hline
Math&NORTS&1141.03&1141.03&100.00&2831.06&35.91&35.91&100.00&2818.73&7.39&7.39&100.00&2798.84&6.48&6.48&100.00&2843.87&6.26&6.26&100.00&2786.79&6.18&6.18&100.00&2738.60&1.21&1.21&100.00&2211.26&1.67&1.67&100.00&2314.33&701.81&701.81&100.00&2783.79&10.78&10.78&100.00&2761.57&800.10&800.10&100.00&2768.45&393.51&393.51&100.00&2775.49\\ \hline
Math&CLASS&1141.03&1141.03&100.00&237.26&35.91&35.91&100.00&366.66&7.39&7.39&100.00&188.06&6.48&6.48&100.00&233.53&6.26&6.26&100.00&180.81&6.18&6.18&100.00&249.40&1.21&1.21&100.00&75.92&1.67&1.67&100.00&198.67&701.81&701.81&100.00&150.85&10.78&10.78&100.00&120.70&800.10&800.10&100.00&186.65&393.51&393.51&100.00&133.06\\ \hline
Math&METHOD&1141.03&1141.03&100.00&69.20&35.91&35.91&100.00&60.63&7.39&7.39&100.00&21.55&6.48&6.48&100.00&26.61&6.26&6.26&100.00&24.20&6.18&6.18&100.00&25.45&1.21&1.21&100.00&34.58&1.67&1.67&100.00&89.00&701.81&701.81&100.00&31.47&10.78&10.78&100.00&24.35&800.10&800.10&100.00&34.06&393.51&393.51&100.00&29.09\\ \hline
Math&STATE&1141.03&1141.03&100.00&60.27&35.91&35.91&100.00&47.81&7.39&7.39&100.00&9.08&6.48&6.48&100.00&12.44&6.26&6.26&100.00&7.82&6.18&6.18&100.00&9.92&1.21&1.21&100.00&25.91&1.67&1.67&100.00&39.67&701.81&701.81&100.00&17.91&10.78&10.78&100.00&13.91&800.10&800.10&100.00&19.04&393.51&393.51&100.00&15.86\\ \hline
Time&NORTS&790.08&790.08&100.00&3923.62&57.11&57.11&100.00&3920.67&5.91&5.91&100.00&3940.27&4.73&4.73&100.00&3941.36&5.27&5.27&100.00&3940.27&3.50&3.50&100.00&3919.38&2.00&2.00&100.00&3888.33&1.00&1.00&100.00&4041.00&714.90&714.90&100.00&3879.70&39.62&39.62&100.00&3885.62&885.44&885.44&100.00&3879.44&235.44&235.44&100.00&3879.44\\ \hline
Time&CLASS&790.08&790.08&100.00&1090.55&57.11&57.11&100.00&1107.55&5.91&5.91&100.00&1248.93&4.73&4.73&100.00&879.82&5.27&5.27&100.00&1059.98&3.50&3.50&100.00&733.62&2.00&2.00&100.00&1869.33&1.00&1.00&100.00&139.00&714.90&714.90&100.00&1513.01&39.62&39.62&100.00&1390.18&885.44&885.44&100.00&1669.57&235.44&235.44&100.00&1429.74\\ \hline
Time&METHOD&790.08&790.08&100.00&303.10&57.11&57.11&100.00&47.98&5.91&5.91&100.00&90.36&4.73&4.73&100.00&45.18&5.27&5.27&100.00&47.56&3.50&3.50&100.00&61.62&2.00&2.00&100.00&166.00&1.00&1.00&100.00&7.00&714.90&714.90&100.00&327.12&39.62&39.62&100.00&250.69&885.44&885.44&100.00&497.07&235.44&235.44&100.00&380.38\\ \hline
Time&STATE&790.08&790.08&100.00&250.44&57.11&57.11&100.00&38.94&5.91&5.91&100.00&9.46&4.73&4.73&100.00&10.70&5.27&5.27&100.00&6.32&3.50&3.50&100.00&8.75&2.00&2.00&100.00&163.67&1.00&1.00&100.00&7.00&714.90&714.90&100.00&281.29&39.62&39.62&100.00&231.32&885.44&885.44&100.00&444.18&235.44&235.44&100.00&355.36\\ \hline
Chart&NORTS&656.40&656.40&100.00&1829.28&68.52&68.52&100.00&1835.39&6.58&6.58&100.00&1853.63&6.33&6.33&100.00&1866.33&5.79&5.79&100.00&1853.63&6.59&6.59&100.00&1873.88&1.00&1.00&100.00&1805.70&nan&nan&nan&nan&436.26&436.26&100.00&1830.78&40.50&40.50&100.00&1835.32&682.29&682.29&100.00&1829.83&239.38&239.38&100.00&1829.83\\ \hline
Chart&CLASS&656.40&656.40&100.00&113.39&68.52&68.52&100.00&108.55&6.58&6.58&100.00&83.89&6.33&6.33&100.00&69.61&5.79&5.79&100.00&71.64&6.59&6.59&100.00&68.01&1.00&1.00&100.00&105.00&nan&nan&nan&nan&436.26&436.26&100.00&121.56&40.50&40.50&100.00&103.63&682.29&682.29&100.00&136.75&239.38&239.38&100.00&121.61\\ \hline
Chart&METHOD&656.40&656.40&100.00&46.01&68.52&68.52&100.00&49.66&6.58&6.58&100.00&11.89&6.33&6.33&100.00&12.54&5.79&5.79&100.00&12.33&6.59&6.59&100.00&13.83&1.00&1.00&100.00&25.00&nan&nan&nan&nan&436.26&436.26&100.00&25.66&40.50&40.50&100.00&33.30&682.29&682.29&100.00&33.69&239.38&239.38&100.00&30.25\\ \hline
Chart&STATE&656.40&656.40&100.00&43.91&68.52&68.52&100.00&48.73&6.58&6.58&100.00&6.14&6.33&6.33&100.00&7.06&5.79&5.79&100.00&6.08&6.59&6.59&100.00&6.34&1.00&1.00&100.00&24.60&nan&nan&nan&nan&436.26&436.26&100.00&16.12&40.50&40.50&100.00&29.78&682.29&682.29&100.00&21.98&239.38&239.38&100.00&23.50\\ \hline
Mockito&NORTS&1990.14&1990.14&100.00&1128.64&nan&nan&nan&nan&3.75&3.75&100.00&1005.31&4.80&4.80&100.00&1048.20&4.33&4.33&100.00&1018.73&4.43&4.43&100.00&1088.43&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&1990.14&1990.14&100.00&699.55&nan&nan&nan&nan&3.75&3.75&100.00&394.65&4.80&4.80&100.00&345.37&4.33&4.33&100.00&427.13&4.43&4.43&100.00&382.94&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&1990.14&1990.14&100.00&560.27&nan&nan&nan&nan&3.75&3.75&100.00&182.91&4.80&4.80&100.00&164.89&4.33&4.33&100.00&194.85&4.43&4.43&100.00&154.32&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&1990.14&1990.14&100.00&539.52&nan&nan&nan&nan&3.75&3.75&100.00&15.80&4.80&4.80&100.00&27.59&4.33&4.33&100.00&16.37&4.43&4.43&100.00&14.84&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&nan&nan&nan&nan&5.71&5.71&100.00&7246.80&3.94&3.94&100.00&7133.26&3.62&3.62&100.00&7200.68&3.90&3.90&100.00&7178.36&2.89&2.89&100.00&7502.06&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&nan&nan&nan&nan&5.71&5.71&100.00&4213.12&3.94&3.94&100.00&3749.01&3.62&3.62&100.00&4075.31&3.90&3.90&100.00&4147.67&2.89&2.89&100.00&3419.44&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&nan&nan&nan&nan&5.71&5.71&100.00&728.99&3.94&3.94&100.00&2062.22&3.62&3.62&100.00&2112.97&3.90&3.90&100.00&2137.47&2.89&2.89&100.00&685.57&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&nan&nan&nan&nan&5.71&5.71&100.00&264.72&3.94&3.94&100.00&1076.41&3.62&3.62&100.00&993.20&3.90&3.90&100.00&924.81&2.89&2.89&100.00&134.63&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&990.90&990.90&100.00&2315.78&49.33&49.33&100.00&3535.23&6.37&6.37&100.00&3087.44&6.17&6.17&100.00&3117.06&6.06&6.06&100.00&3095.19&5.69&5.69&100.00&3153.15&1.41&1.41&100.00&2414.72&1.22&1.22&100.00&2829.44&670.80&670.80&100.00&2609.21&34.46&34.46&100.00&2606.74&856.68&856.68&100.00&2605.07&334.21&334.21&100.00&2606.83\\ \hline
All &CLASS&990.90&990.90&100.00&442.92&49.33&49.33&100.00&1171.73&6.37&6.37&100.00&952.82&6.17&6.17&100.00&942.96&6.06&6.06&100.00&990.03&5.69&5.69&100.00&818.20&1.41&1.41&100.00&521.81&1.22&1.22&100.00&135.67&670.80&670.80&100.00&463.08&34.46&34.46&100.00&418.41&856.68&856.68&100.00&515.51&334.21&334.21&100.00&437.81\\ \hline
All &METHOD&990.90&990.90&100.00&198.73&49.33&49.33&100.00&179.67&6.37&6.37&100.00&395.92&6.17&6.17&100.00&394.87&6.06&6.06&100.00&403.74&5.69&5.69&100.00&157.87&1.41&1.41&100.00&58.79&1.22&1.22&100.00&34.00&670.80&670.80&100.00&98.73&34.46&34.46&100.00&79.72&856.68&856.68&100.00&143.95&334.21&334.21&100.00&112.48\\ \hline
All &STATE&990.90&990.90&100.00&181.50&49.33&49.33&100.00&82.00&6.37&6.37&100.00&186.84&6.17&6.17&100.00&175.99&6.06&6.06&100.00&160.94&5.69&5.69&100.00&29.76&1.41&1.41&100.00&55.26&1.22&1.22&100.00&16.89&670.80&670.80&100.00&80.98&34.46&34.46&100.00&71.04&856.68&856.68&100.00&123.46&334.21&334.21&100.00&100.70\\ \hline


    \end{tabular}
    \end{adjustbox}
\end{table*} 



==> tables/Nonplausible_ave_latex_table.tex <==
\begin{table*}
    \centering
   \caption{(Non Plausible) Average executed tests with different \rts{} on all APR systems  }\label{table:ave_test_summary}
   	\begin{adjustbox}{width=2\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 



Lang&NORTS&400.66&400.36&95.63&5.79&80.79&80.60&96.38&1.00&10.63&10.48&95.71&4.88&11.00&10.93&92.59&3.10&10.93&10.78&88.48&19.74&10.88&10.77&88.46&3.45&1.43&0.71&28.57&1.00&1.00&0.67&66.67&1.00&900.67&900.39&90.00&85.68&47.69&47.54&93.99&13.23&1083.03&1082.89&96.19&72.49&498.11&497.89&96.75&16.94\\ \hline
Lang&CLASS&400.66&400.36&95.63&1.16&80.79&80.60&96.38&1.00&10.63&10.48&95.71&1.06&11.00&10.93&92.59&1.03&10.93&10.78&88.48&1.74&10.88&10.77&88.46&1.04&1.43&0.71&28.57&1.00&1.00&0.67&66.67&1.00&900.67&900.39&90.00&2.06&47.69&47.54&93.99&1.25&1083.03&1082.89&96.19&2.60&498.11&497.89&96.75&1.21\\ \hline
Lang&METHOD&400.66&400.36&95.63&1.12&80.79&80.60&96.38&1.00&10.63&10.48&95.71&1.06&11.00&10.93&92.59&1.03&10.93&10.78&88.48&1.11&10.88&10.77&88.46&1.04&1.43&0.71&28.57&1.00&1.00&0.67&66.67&1.00&900.67&900.39&90.00&1.40&47.69&47.54&93.99&1.22&1083.03&1082.89&96.19&1.29&498.11&497.89&96.75&1.14\\ \hline
Lang&STATE&400.66&400.36&95.63&1.11&80.79&80.60&96.38&1.00&10.63&10.48&95.71&1.02&11.00&10.93&92.59&1.01&10.93&10.78&88.48&1.06&10.88&10.77&88.46&1.01&1.43&0.71&28.57&1.00&1.00&0.67&66.67&1.00&900.67&900.39&90.00&1.37&47.69&47.54&93.99&1.19&1083.03&1082.89&96.19&1.28&498.11&497.89&96.75&1.08\\ \hline
Math&NORTS&1513.39&1513.01&96.45&12.26&35.90&35.57&86.15&17.65&7.39&7.35&96.20&7.26&6.48&6.42&94.80&1.00&6.26&6.10&87.71&10.30&6.18&6.10&92.21&1.77&1.21&0.37&21.05&342.20&1.67&1.33&66.67&1.00&837.59&837.41&88.62&115.37&11.49&11.40&95.63&25.48&893.95&893.78&94.85&91.20&433.24&433.03&97.29&19.35\\ \hline
Math&CLASS&1513.39&1513.01&96.45&1.41&35.90&35.57&86.15&1.38&7.39&7.35&96.20&1.79&6.48&6.42&94.80&1.00&6.26&6.10&87.71&3.37&6.18&6.10&92.21&1.22&1.21&0.37&21.05&24.07&1.67&1.33&66.67&1.00&837.59&837.41&88.62&5.55&11.49&11.40&95.63&1.64&893.95&893.78&94.85&5.57&433.24&433.03&97.29&2.14\\ \hline
Math&METHOD&1513.39&1513.01&96.45&1.10&35.90&35.57&86.15&1.35&7.39&7.35&96.20&1.04&6.48&6.42&94.80&1.00&6.26&6.10&87.71&1.08&6.18&6.10&92.21&1.03&1.21&0.37&21.05&16.60&1.67&1.33&66.67&1.00&837.59&837.41&88.62&2.23&11.49&11.40&95.63&1.18&893.95&893.78&94.85&1.80&433.24&433.03&97.29&1.15\\ \hline
Math&STATE&1513.39&1513.01&96.45&1.07&35.90&35.57&86.15&1.34&7.39&7.35&96.20&1.04&6.48&6.42&94.80&1.00&6.26&6.10&87.71&1.08&6.18&6.10&92.21&1.01&1.21&0.37&21.05&16.13&1.67&1.33&66.67&1.00&837.59&837.41&88.62&1.61&11.49&11.40&95.63&1.14&893.95&893.78&94.85&1.63&433.24&433.03&97.29&1.08\\ \hline
Time&NORTS&1466.54&1466.35&99.07&3.81&53.91&53.82&96.97&5.27&5.91&5.82&96.97&353.64&4.73&4.73&100.00&1.00&5.27&5.18&90.91&1.00&3.50&3.38&87.50&1.00&2.00&1.67&66.67&1.00&1.00&1.00&100.00&1.00&794.00&794.00&100.00&44.51&34.40&34.30&99.47&27.07&989.60&989.60&100.00&118.35&279.40&279.40&100.00&4.52\\ \hline
Time&CLASS&1466.54&1466.35&99.07&1.30&53.91&53.82&96.97&2.41&5.91&5.82&96.97&76.55&4.73&4.73&100.00&1.00&5.27&5.18&90.91&1.00&3.50&3.38&87.50&1.00&2.00&1.67&66.67&1.00&1.00&1.00&100.00&1.00&794.00&794.00&100.00&10.25&34.40&34.30&99.47&13.56&989.60&989.60&100.00&24.74&279.40&279.40&100.00&1.53\\ \hline
Time&METHOD&1466.54&1466.35&99.07&1.14&53.91&53.82&96.97&1.03&5.91&5.82&96.97&2.27&4.73&4.73&100.00&1.00&5.27&5.18&90.91&1.00&3.50&3.38&87.50&1.00&2.00&1.67&66.67&1.00&1.00&1.00&100.00&1.00&794.00&794.00&100.00&5.75&34.40&34.30&99.47&1.25&989.60&989.60&100.00&9.03&279.40&279.40&100.00&1.20\\ \hline
Time&STATE&1466.54&1466.35&99.07&1.12&53.91&53.82&96.97&1.03&5.91&5.82&96.97&2.27&4.73&4.73&100.00&1.00&5.27&5.18&90.91&1.00&3.50&3.38&87.50&1.00&2.00&1.67&66.67&1.00&1.00&1.00&100.00&1.00&794.00&794.00&100.00&3.06&34.40&34.30&99.47&1.17&989.60&989.60&100.00&1.76&279.40&279.40&100.00&1.02\\ \hline
Chart&NORTS&784.88&784.32&97.93&5.78&68.43&68.35&97.34&1.00&6.58&6.42&86.84&1.01&6.33&6.28&94.44&1.08&5.79&5.58&78.95&1.03&6.59&6.53&94.12&1.00&1.00&0.10&10.00&1.00&nan&nan&nan&nan&682.35&681.91&90.34&141.69&48.14&47.86&90.97&21.73&760.12&759.92&98.41&129.38&347.04&346.75&98.19&22.59\\ \hline
Chart&CLASS&784.88&784.32&97.93&1.57&68.43&68.35&97.34&1.00&6.58&6.42&86.84&1.01&6.33&6.28&94.44&1.08&5.79&5.58&78.95&1.03&6.59&6.53&94.12&1.00&1.00&0.10&10.00&1.00&nan&nan&nan&nan&682.35&681.91&90.34&19.41&48.14&47.86&90.97&1.52&760.12&759.92&98.41&11.26&347.04&346.75&98.19&3.58\\ \hline
Chart&METHOD&784.88&784.32&97.93&1.17&68.43&68.35&97.34&1.00&6.58&6.42&86.84&1.01&6.33&6.28&94.44&1.08&5.79&5.58&78.95&1.03&6.59&6.53&94.12&1.00&1.00&0.10&10.00&1.00&nan&nan&nan&nan&682.35&681.91&90.34&4.90&48.14&47.86&90.97&1.11&760.12&759.92&98.41&3.71&347.04&346.75&98.19&1.31\\ \hline
Chart&STATE&784.88&784.32&97.93&1.16&68.43&68.35&97.34&1.00&6.58&6.42&86.84&1.01&6.33&6.28&94.44&1.08&5.79&5.58&78.95&1.03&6.59&6.53&94.12&1.00&1.00&0.10&10.00&1.00&nan&nan&nan&nan&682.35&681.91&90.34&2.28&48.14&47.86&90.97&1.07&760.12&759.92&98.41&2.49&347.04&346.75&98.19&1.20\\ \hline
Mockito&NORTS&2307.92&2307.78&99.11&1.72&nan&nan&nan&nan&3.75&3.50&75.00&11.42&4.80&4.80&100.00&8.29&4.33&4.13&80.00&1.00&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&2307.92&2307.78&99.11&1.21&nan&nan&nan&nan&3.75&3.50&75.00&2.55&4.80&4.80&100.00&5.24&4.33&4.13&80.00&1.00&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&2307.92&2307.78&99.11&1.08&nan&nan&nan&nan&3.75&3.50&75.00&1.03&4.80&4.80&100.00&1.20&4.33&4.13&80.00&1.00&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&2307.92&2307.78&99.11&1.08&nan&nan&nan&nan&3.75&3.50&75.00&1.03&4.80&4.80&100.00&1.20&4.33&4.13&80.00&1.00&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&14725.00&14724.60&97.30&30.01&5.71&5.14&58.44&1.02&3.94&3.89&96.81&10.26&3.62&3.58&95.56&15.06&3.90&3.84&93.62&2.43&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&14725.00&14724.60&97.30&23.97&5.71&5.14&58.44&1.02&3.94&3.89&96.81&3.18&3.62&3.58&95.56&3.96&3.90&3.84&93.62&2.08&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&14725.00&14724.60&97.30&11.13&5.71&5.14&58.44&1.02&3.94&3.89&96.81&1.12&3.62&3.58&95.56&1.07&3.90&3.84&93.62&1.03&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&14725.00&14724.60&97.30&1.35&5.71&5.14&58.44&1.02&3.94&3.89&96.81&1.12&3.62&3.58&95.56&1.05&3.90&3.84&93.62&1.01&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&3533.06&3532.74&97.58&9.90&48.95&48.70&87.06&5.19&6.37&6.24&91.26&64.74&6.16&6.12&96.23&4.92&6.08&5.94&86.61&5.92&5.78&5.71&93.71&1.54&1.41&0.71&31.57&86.30&1.22&1.00&77.78&1.00&803.65&803.43&92.24&96.81&35.43&35.28&95.02&21.88&931.68&931.55&97.36&102.86&389.45&389.27&98.06&15.85\\ \hline
All &CLASS&3533.06&3532.74&97.58&5.10&48.95&48.70&87.06&1.36&6.37&6.24&91.26&14.36&6.16&6.12&96.23&2.22&6.08&5.94&86.61&1.70&5.78&5.71&93.71&1.04&1.41&0.71&31.57&6.77&1.22&1.00&77.78&1.00&803.65&803.43&92.24&9.32&35.43&35.28&95.02&4.49&931.68&931.55&97.36&11.04&389.45&389.27&98.06&2.12\\ \hline
All &METHOD&3533.06&3532.74&97.58&2.79&48.95&48.70&87.06&1.08&6.37&6.24&91.26&1.26&6.16&6.12&96.23&1.06&6.08&5.94&86.61&1.04&5.78&5.71&93.71&1.01&1.41&0.71&31.57&4.90&1.22&1.00&77.78&1.00&803.65&803.43&92.24&3.57&35.43&35.28&95.02&1.19&931.68&931.55&97.36&3.96&389.45&389.27&98.06&1.20\\ \hline
All &STATE&3533.06&3532.74&97.58&1.15&48.95&48.70&87.06&1.08&6.37&6.24&91.26&1.25&6.16&6.12&96.23&1.06&6.08&5.94&86.61&1.03&5.78&5.71&93.71&1.00&1.41&0.71&31.57&4.78&1.22&1.00&77.78&1.00&803.65&803.43&92.24&2.08&35.43&35.28&95.02&1.15&931.68&931.55&97.36&1.79&389.45&389.27&98.06&1.09\\ \hline


  
    \end{tabular}
    \end{adjustbox}
\end{table*} 



\begin{table*}
    \centering
   \caption{Full-(Nonplausible) Average executed tests with different \rts{} on all APR systems  }\label{table:full_nonplausible_at_summary}
   	\begin{adjustbox}{width=2.1\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 
    
    
    Lang&NORTS&376.83&376.49&95.40&1869.09&79.40&79.17&96.31&1855.21&10.63&10.48&95.71&1793.33&11.04&10.93&92.22&1810.96&10.78&10.59&87.86&1798.33&10.54&10.38&84.62&1816.95&1.43&0.71&28.57&1741.00&1.00&0.67&66.67&2288.50&830.22&829.86&87.19&1948.91&46.94&46.77&93.53&1960.48&1058.89&1058.72&93.42&1956.41&468.53&468.25&95.23&1950.31\\ \hline
Lang&CLASS&376.83&376.49&95.40&76.12&79.40&79.17&96.31&63.54&10.63&10.48&95.71&52.35&11.04&10.93&92.22&50.98&10.78&10.59&87.86&51.42&10.54&10.38&84.62&53.59&1.43&0.71&28.57&42.00&1.00&0.67&66.67&79.50&830.22&829.86&87.19&66.62&46.94&46.77&93.53&60.23&1058.89&1058.72&93.42&69.48&468.53&468.25&95.23&68.41\\ \hline
Lang&METHOD&376.83&376.49&95.40&15.40&79.40&79.17&96.31&11.17&10.63&10.48&95.71&6.60&11.04&10.93&92.22&7.06&10.78&10.59&87.86&6.49&10.54&10.38&84.62&6.66&1.43&0.71&28.57&26.00&1.00&0.67&66.67&8.50&830.22&829.86&87.19&11.41&46.94&46.77&93.53&10.95&1058.89&1058.72&93.42&11.53&468.53&468.25&95.23&10.41\\ \hline
Lang&STATE&376.83&376.49&95.40&13.79&79.40&79.17&96.31&9.83&10.63&10.48&95.71&4.18&11.04&10.93&92.22&4.81&10.78&10.59&87.86&4.58&10.54&10.38&84.62&4.04&1.43&0.71&28.57&19.50&1.00&0.67&66.67&5.50&830.22&829.86&87.19&9.24&46.94&46.77&93.53&9.60&1058.89&1058.72&93.42&9.07&468.53&468.25&95.23&8.30\\ \hline
Math&NORTS&1141.03&1140.51&95.31&2818.48&35.91&35.57&85.56&2836.13&7.39&7.35&96.20&2789.29&6.48&6.42&94.80&2775.16&6.26&6.10&87.71&2659.69&6.18&6.10&92.21&2722.42&1.21&0.37&21.05&2078.60&1.67&1.33&66.67&2289.50&701.81&701.44&85.87&2775.77&10.78&10.67&94.78&2731.18&800.10&799.80&92.96&2757.52&393.51&393.20&93.79&2710.97\\ \hline
Math&CLASS&1141.03&1140.51&95.31&241.88&35.91&35.57&85.56&363.03&7.39&7.35&96.20&194.57&6.48&6.42&94.80&203.99&6.26&6.10&87.71&199.62&6.18&6.10&92.21&268.34&1.21&0.37&21.05&175.80&1.67&1.33&66.67&290.50&701.81&701.44&85.87&163.76&10.78&10.67&94.78&123.76&800.10&799.80&92.96&192.53&393.51&393.20&93.79&137.44\\ \hline
Math&METHOD&1141.03&1140.51&95.31&70.59&35.91&35.57&85.56&58.73&7.39&7.35&96.20&21.83&6.48&6.42&94.80&27.18&6.26&6.10&87.71&25.64&6.18&6.10&92.21&26.82&1.21&0.37&21.05&73.80&1.67&1.33&66.67&126.00&701.81&701.44&85.87&34.06&10.78&10.67&94.78&24.77&800.10&799.80&92.96&34.84&393.51&393.20&93.79&29.68\\ \hline
Math&STATE&1141.03&1140.51&95.31&61.46&35.91&35.57&85.56&44.94&7.39&7.35&96.20&9.28&6.48&6.42&94.80&12.66&6.26&6.10&87.71&8.11&6.18&6.10&92.21&10.66&1.21&0.37&21.05&49.67&1.67&1.33&66.67&59.00&701.81&701.44&85.87&19.25&10.78&10.67&94.78&14.28&800.10&799.80&92.96&19.70&393.51&393.20&93.79&16.25\\ \hline
Time&NORTS&790.08&789.54&98.99&3923.62&57.11&56.89&93.98&3920.67&5.91&5.82&96.97&3940.27&4.73&4.73&100.00&3941.36&5.27&5.18&90.91&3945.00&3.50&3.38&87.50&3923.14&2.00&1.67&66.67&3879.50&1.00&1.00&100.00&4041.00&714.90&714.70&99.58&3879.70&39.62&39.62&100.00&3885.62&885.44&885.33&99.98&3879.44&235.44&235.33&99.96&3879.44\\ \hline
Time&CLASS&790.08&789.54&98.99&1089.09&57.11&56.89&93.98&1097.44&5.91&5.82&96.97&1248.93&4.73&4.73&100.00&879.82&5.27&5.18&90.91&1082.77&3.50&3.38&87.50&719.57&2.00&1.67&66.67&2000.50&1.00&1.00&100.00&139.00&714.90&714.70&99.58&1507.09&39.62&39.62&100.00&1390.18&885.44&885.33&99.98&1669.57&235.44&235.33&99.96&1429.74\\ \hline
Time&METHOD&790.08&789.54&98.99&302.88&57.11&56.89&93.98&46.47&5.91&5.82&96.97&90.36&4.73&4.73&100.00&45.18&5.27&5.18&90.91&50.82&3.50&3.38&87.50&68.29&2.00&1.67&66.67&238.50&1.00&1.00&100.00&7.00&714.90&714.70&99.58&326.90&39.62&39.62&100.00&250.69&885.44&885.33&99.98&497.06&235.44&235.33&99.96&380.28\\ \hline
Time&STATE&790.08&789.54&98.99&250.36&57.11&56.89&93.98&38.64&5.91&5.82&96.97&9.46&4.73&4.73&100.00&10.70&5.27&5.18&90.91&5.45&3.50&3.38&87.50&7.86&2.00&1.67&66.67&235.00&1.00&1.00&100.00&7.00&714.90&714.70&99.58&281.28&39.62&39.62&100.00&231.32&885.44&885.33&99.98&444.18&235.44&235.33&99.96&355.35\\ \hline
Chart&NORTS&656.40&655.72&89.92&1827.22&68.52&68.43&97.34&1835.39&6.58&6.42&86.84&1880.82&6.33&6.28&94.44&1869.29&5.79&5.58&78.95&1889.47&6.59&6.53&94.12&1889.44&1.00&0.10&10.00&1650.00&nan&nan&nan&nan&436.26&435.65&82.23&1836.62&40.50&40.09&90.03&1845.57&682.29&681.96&96.05&1829.83&239.38&238.88&93.59&1827.22\\ \hline
Chart&CLASS&656.40&655.72&89.92&100.47&68.52&68.43&97.34&108.55&6.58&6.42&86.84&92.65&6.33&6.28&94.44&72.35&5.79&5.58&78.95&86.95&6.59&6.53&94.12&71.64&1.00&0.10&10.00&278.00&nan&nan&nan&nan&436.26&435.65&82.23&122.54&40.50&40.09&90.03&100.13&682.29&681.96&96.05&136.14&239.38&238.88&93.59&108.00\\ \hline
Chart&METHOD&656.40&655.72&89.92&48.67&68.52&68.43&97.34&48.27&6.58&6.42&86.84&12.94&6.33&6.28&94.44&13.10&5.79&5.58&78.95&14.88&6.59&6.53&94.12&14.63&1.00&0.10&10.00&84.00&nan&nan&nan&nan&436.26&435.65&82.23&30.44&40.50&40.09&90.03&34.49&682.29&681.96&96.05&33.64&239.38&238.88&93.59&27.54\\ \hline
Chart&STATE&656.40&655.72&89.92&46.39&68.52&68.43&97.34&47.34&6.58&6.42&86.84&6.51&6.33&6.28&94.44&7.29&5.79&5.58&78.95&6.97&6.59&6.53&94.12&6.68&1.00&0.10&10.00&84.00&nan&nan&nan&nan&436.26&435.65&82.23&17.87&40.50&40.09&90.03&30.89&682.29&681.96&96.05&21.95&239.38&238.88&93.59&23.34\\ \hline
Mockito&NORTS&1990.14&1989.89&99.08&1128.64&nan&nan&nan&nan&3.75&3.50&75.00&1040.17&4.80&4.80&100.00&1048.20&4.33&4.13&80.00&1028.25&4.43&4.36&96.43&1088.43&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&1990.14&1989.89&99.08&699.72&nan&nan&nan&nan&3.75&3.50&75.00&408.53&4.80&4.80&100.00&345.37&4.33&4.13&80.00&356.00&4.43&4.36&96.43&391.72&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&1990.14&1989.89&99.08&560.31&nan&nan&nan&nan&3.75&3.50&75.00&238.55&4.80&4.80&100.00&164.89&4.33&4.13&80.00&188.73&4.43&4.36&96.43&190.71&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&1990.14&1989.89&99.08&539.50&nan&nan&nan&nan&3.75&3.50&75.00&16.07&4.80&4.80&100.00&27.59&4.33&4.13&80.00&16.47&4.43&4.36&96.43&14.84&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&nan&nan&nan&nan&5.71&5.14&58.44&7109.74&3.94&3.89&96.81&7123.15&3.62&3.58&95.56&7190.97&3.90&3.84&93.62&7168.38&2.89&2.89&100.00&7502.06&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&nan&nan&nan&nan&5.71&5.14&58.44&4314.90&3.94&3.89&96.81&3827.19&3.62&3.58&95.56&4119.66&3.90&3.84&93.62&4229.50&2.89&2.89&100.00&3419.44&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&nan&nan&nan&nan&5.71&5.14&58.44&669.15&3.94&3.89&96.81&2106.11&3.62&3.58&95.56&2204.95&3.90&3.84&93.62&2280.32&2.89&2.89&100.00&685.57&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&nan&nan&nan&nan&5.71&5.14&58.44&231.78&3.94&3.89&96.81&1099.68&3.62&3.58&95.56&1039.23&3.90&3.84&93.62&987.33&2.89&2.89&100.00&134.63&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&990.90&990.43&95.74&2313.41&49.33&49.04&86.33&3511.43&6.37&6.24&91.26&3094.51&6.17&6.12&96.17&3105.99&6.06&5.90&86.51&3081.52&5.69&5.61&92.48&3157.07&1.41&0.71&31.57&2337.28&1.22&1.00&77.78&2873.00&670.80&670.41&88.72&2610.25&34.46&34.29&94.58&2605.71&856.68&856.45&95.60&2605.80&334.21&333.91&95.64&2591.99\\ \hline
All &CLASS&990.90&990.43&95.74&441.46&49.33&49.04&86.33&1189.49&6.37&6.24&91.26&970.70&6.17&6.12&96.17&945.36&6.06&5.90&86.51&1001.04&5.69&5.61&92.48&820.72&1.41&0.71&31.57&624.08&1.22&1.00&77.78&169.67&670.80&670.41&88.72&465.00&34.46&34.29&94.58&418.57&856.68&856.45&95.60&516.93&334.21&333.91&95.64&435.90\\ \hline
All &METHOD&990.90&990.43&95.74&199.57&49.33&49.04&86.33&166.76&6.37&6.24&91.26&412.73&6.17&6.12&96.17&410.39&6.06&5.90&86.51&427.82&5.69&5.61&92.48&165.45&1.41&0.71&31.57&105.58&1.22&1.00&77.78&47.17&670.80&670.41&88.72&100.71&34.46&34.29&94.58&80.23&856.68&856.45&95.60&144.27&334.21&333.91&95.64&111.97\\ \hline
All &STATE&990.90&990.43&95.74&182.30&49.33&49.04&86.33&74.50&6.37&6.24&91.26&190.86&6.17&6.12&96.17&183.71&6.06&5.90&86.51&171.49&5.69&5.61&92.48&29.78&1.41&0.71&31.57&97.04&1.22&1.00&77.78&23.83&670.80&670.41&88.72&81.91&34.46&34.29&94.58&71.52&856.68&856.45&95.60&123.72&334.21&333.91&95.64&100.81\\ \hline

    
    
    \end{tabular}
    \end{adjustbox}
\end{table*} 


==> tables/Plausible_ave_latex_table.tex <==
\begin{table*}
    \centering
   \caption{(Plausible) Average executed tests with different \rts{} on all APR systems  }\label{table:ave_test_summary}
   	\begin{adjustbox}{width=2\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 


Lang&NORTS&400.66&0.31&4.37&1818.94&80.79&0.19&3.62&1834.78&10.63&0.15&4.29&1731.75&11.00&0.07&7.41&1688.50&10.93&0.15&11.52&1737.50&10.88&0.12&11.54&1682.67&1.43&0.71&71.43&1758.60&1.00&0.33&33.33&1822.00&900.67&0.28&10.00&1803.20&47.69&0.14&6.01&1811.20&1083.03&0.14&3.81&1895.20&498.11&0.22&3.25&1862.25\\ \hline
Lang&CLASS&400.66&0.31&4.37&83.22&80.79&0.19&3.62&27.89&10.63&0.15&4.29&54.75&11.00&0.07&7.41&93.50&10.93&0.15&11.52&51.50&10.88&0.12&11.54&66.33&1.43&0.71&71.43&35.00&1.00&0.33&33.33&49.00&900.67&0.28&10.00&104.80&47.69&0.14&6.01&43.00&1083.03&0.14&3.81&69.20&498.11&0.22&3.25&83.38\\ \hline
Lang&METHOD&400.66&0.31&4.37&11.56&80.79&0.19&3.62&8.78&10.63&0.15&4.29&5.00&11.00&0.07&7.41&7.00&10.93&0.15&11.52&4.50&10.88&0.12&11.54&5.67&1.43&0.71&71.43&3.00&1.00&0.33&33.33&1.00&900.67&0.28&10.00&3.90&47.69&0.14&6.01&3.00&1083.03&0.14&3.81&3.40&498.11&0.22&3.25&3.25\\ \hline
Lang&STATE&400.66&0.31&4.37&9.22&80.79&0.19&3.62&7.89&10.63&0.15&4.29&4.50&11.00&0.07&7.41&7.00&10.93&0.15&11.52&4.00&10.88&0.12&11.54&5.00&1.43&0.71&71.43&1.80&1.00&0.33&33.33&1.00&900.67&0.28&10.00&3.40&47.69&0.14&6.01&2.20&1083.03&0.14&3.81&2.60&498.11&0.22&3.25&1.75\\ \hline
Math&NORTS&1513.39&0.38&3.55&2742.68&35.90&0.33&13.85&2518.68&7.39&0.04&3.80&3040.67&6.48&0.06&5.20&3644.00&6.26&0.16&12.29&3618.46&6.18&0.08&7.79&2930.00&1.21&0.84&78.95&2301.31&1.67&0.33&33.33&2364.00&837.59&0.19&11.38&2664.28&11.49&0.09&4.37&3439.12&893.95&0.17&5.15&2656.62&433.24&0.21&2.71&2694.00\\ \hline
Math&CLASS&1513.39&0.38&3.55&91.81&35.90&0.33&13.85&360.79&7.39&0.04&3.80&23.33&6.48&0.06&5.20&635.80&6.26&0.16&12.29&123.62&6.18&0.08&7.79&25.33&1.21&0.84&78.95&52.12&1.67&0.33&33.33&15.00&837.59&0.19&11.38&75.33&11.49&0.09&4.37&54.25&893.95&0.17&5.15&80.12&433.24&0.21&2.71&82.00\\ \hline
Math&METHOD&1513.39&0.38&3.55&17.81&35.90&0.33&13.85&49.86&7.39&0.04&3.80&14.33&6.48&0.06&5.20&13.20&6.26&0.16&12.29&10.85&6.18&0.08&7.79&9.17&1.21&0.84&78.95&33.06&1.67&0.33&33.33&15.00&837.59&0.19&11.38&21.72&11.49&0.09&4.37&22.00&893.95&0.17&5.15&28.50&433.24&0.21&2.71&34.40\\ \hline
Math&STATE&1513.39&0.38&3.55&14.73&35.90&0.33&13.85&47.86&7.39&0.04&3.80&4.00&6.48&0.06&5.20&7.00&6.26&0.16&12.29&5.15&6.18&0.08&7.79&1.17&1.21&0.84&78.95&26.81&1.67&0.33&33.33&1.00&837.59&0.19&11.38&13.61&11.49&0.09&4.37&11.25&893.95&0.17&5.15&15.38&433.24&0.21&2.71&17.55\\ \hline
Time&NORTS&1466.54&0.19&0.93&3907.40&53.91&0.09&3.03&4014.00&5.91&0.09&3.03&3893.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&3893.00&3.50&0.12&12.50&3893.00&2.00&0.33&33.33&3906.00&1.00&0.00&0.00&nan&794.00&0.00&0.00&nan&34.40&0.10&0.53&3866.00&989.60&0.00&0.00&nan&279.40&0.00&0.00&nan\\ \hline
Time&CLASS&1466.54&0.19&0.93&1101.00&53.91&0.09&3.03&167.00&5.91&0.09&3.03&832.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&832.00&3.50&0.12&12.50&832.00&2.00&0.33&33.33&1607.00&1.00&0.00&0.00&nan&794.00&0.00&0.00&nan&34.40&0.10&0.53&1961.00&989.60&0.00&0.00&nan&279.40&0.00&0.00&nan\\ \hline
Time&METHOD&1466.54&0.19&0.93&28.40&53.91&0.09&3.03&28.00&5.91&0.09&3.03&15.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&15.00&3.50&0.12&12.50&15.00&2.00&0.33&33.33&21.00&1.00&0.00&0.00&nan&794.00&0.00&0.00&nan&34.40&0.10&0.53&100.00&989.60&0.00&0.00&nan&279.40&0.00&0.00&nan\\ \hline
Time&STATE&1466.54&0.19&0.93&11.40&53.91&0.09&3.03&6.00&5.91&0.09&3.03&15.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&15.00&3.50&0.12&12.50&15.00&2.00&0.33&33.33&21.00&1.00&0.00&0.00&nan&794.00&0.00&0.00&nan&34.40&0.10&0.53&23.00&989.60&0.00&0.00&nan&279.40&0.00&0.00&nan\\ \hline
Chart&NORTS&784.88&0.56&2.07&1852.21&68.43&0.09&2.66&1728.00&6.58&0.16&13.16&1687.00&6.33&0.06&5.56&1816.00&5.79&0.21&21.05&1719.25&6.59&0.06&5.88&1625.00&1.00&0.90&90.00&1823.00&nan&nan&nan&nan&682.35&0.43&9.66&1876.70&48.14&0.27&9.03&1839.67&760.12&0.21&1.59&1890.60&347.04&0.29&1.81&1921.00\\ \hline
Chart&CLASS&784.88&0.56&2.07&125.71&68.43&0.09&2.66&60.50&6.58&0.16&13.16&11.33&6.33&0.06&5.56&23.00&5.79&0.21&21.05&14.25&6.59&0.06&5.88&10.00&1.00&0.90&90.00&85.78&nan&nan&nan&nan&682.35&0.43&9.66&187.40&48.14&0.27&9.03&160.00&760.12&0.21&1.59&191.20&347.04&0.29&1.81&96.29\\ \hline
Chart&METHOD&784.88&0.56&2.07&27.64&68.43&0.09&2.66&49.50&6.58&0.16&13.16&2.67&6.33&0.06&5.56&3.00&5.79&0.21&21.05&2.75&6.59&0.06&5.88&1.00&1.00&0.90&90.00&18.44&nan&nan&nan&nan&682.35&0.43&9.66&27.60&48.14&0.27&9.03&12.67&760.12&0.21&1.59&12.40&347.04&0.29&1.81&19.00\\ \hline
Chart&STATE&784.88&0.56&2.07&27.14&68.43&0.09&2.66&49.50&6.58&0.16&13.16&2.67&6.33&0.06&5.56&3.00&5.79&0.21&21.05&2.75&6.59&0.06&5.88&1.00&1.00&0.90&90.00&18.00&nan&nan&nan&nan&682.35&0.43&9.66&18.50&48.14&0.27&9.03&12.17&760.12&0.21&1.59&12.20&347.04&0.29&1.81&9.71\\ \hline
Mockito&NORTS&2307.92&0.14&0.89&1015.00&nan&nan&nan&nan&3.75&0.25&25.00&900.75&4.80&0.00&0.00&nan&4.33&0.20&20.00&980.67&4.62&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&2307.92&0.14&0.89&24.60&nan&nan&nan&nan&3.75&0.25&25.00&353.00&4.80&0.00&0.00&nan&4.33&0.20&20.00&711.67&4.62&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&2307.92&0.14&0.89&21.20&nan&nan&nan&nan&3.75&0.25&25.00&16.00&4.80&0.00&0.00&nan&4.33&0.20&20.00&219.33&4.62&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&2307.92&0.14&0.89&21.20&nan&nan&nan&nan&3.75&0.25&25.00&15.00&4.80&0.00&0.00&nan&4.33&0.20&20.00&16.00&4.62&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&14725.00&0.40&2.70&7408.02&5.71&0.57&41.56&7371.44&3.94&0.04&3.19&7325.00&3.62&0.04&4.44&7409.50&3.90&0.06&6.38&7324.83&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&14725.00&0.40&2.70&2166.88&5.71&0.57&41.56&4046.13&3.94&0.04&3.19&3067.25&3.62&0.04&4.44&3121.75&3.90&0.06&6.38&2947.50&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&14725.00&0.40&2.70&825.30&5.71&0.57&41.56&773.69&3.94&0.04&3.19&45.00&3.62&0.04&4.44&135.25&3.90&0.06&6.38&42.33&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&14725.00&0.40&2.70&558.60&5.71&0.57&41.56&280.72&3.94&0.04&3.19&5.50&3.62&0.04&4.44&3.50&3.90&0.06&6.38&7.83&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&3533.06&0.33&2.42&3124.04&48.95&0.25&12.94&3493.38&6.37&0.12&8.74&3096.36&6.16&0.04&3.77&3639.50&6.08&0.15&13.39&3212.29&5.78&0.06&6.29&2532.67&1.41&0.70&68.43&2447.23&1.22&0.22&22.22&2093.00&803.65&0.23&7.76&2114.73&35.43&0.15&4.98&2739.00&931.68&0.13&2.64&2147.47&389.45&0.18&1.94&2159.08\\ \hline
All &CLASS&3533.06&0.33&2.42&598.87&48.95&0.25&12.94&932.46&6.37&0.12&8.74&723.61&6.16&0.04&3.77&968.51&6.08&0.15&13.39&780.09&5.78&0.06&6.29&233.42&1.41&0.70&68.43&444.98&1.22&0.22&22.22&32.00&803.65&0.23&7.76&122.51&35.43&0.15&4.98&554.56&931.68&0.13&2.64&113.51&389.45&0.18&1.94&87.22\\ \hline
All &METHOD&3533.06&0.33&2.42&155.32&48.95&0.25&12.94&181.96&6.37&0.12&8.74&16.33&6.16&0.04&3.77&39.61&6.08&0.15&13.39&49.13&5.78&0.06&6.29&7.71&1.41&0.70&68.43&18.88&1.22&0.22&22.22&8.00&803.65&0.23&7.76&17.74&35.43&0.15&4.98&34.42&931.68&0.13&2.64&14.77&389.45&0.18&1.94&18.88\\ \hline
All &STATE&3533.06&0.33&2.42&107.05&48.95&0.25&12.94&78.39&6.37&0.12&8.74&7.78&6.16&0.04&3.77&5.12&6.08&0.15&13.39&8.46&5.78&0.06&6.29&5.54&1.41&0.70&68.43&16.90&1.22&0.22&22.22&1.00&803.65&0.23&7.76&11.84&35.43&0.15&4.98&12.15&931.68&0.13&2.64&10.06&389.45&0.18&1.94&9.67\\ \hline



    \end{tabular}
    \end{adjustbox}
\end{table*} 


\begin{table*}
    \centering
   \caption{Full-(plausible) Average executed tests with different \rts{} on all APR systems  }\label{table:full_nonplausible_at_summary}
   	\begin{adjustbox}{width=2.1\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 
    
    
    Lang&NORTS&376.83&0.34&4.60&1812.00&79.40&0.23&3.69&1838.09&10.63&0.15&4.29&1731.75&11.04&0.11&7.78&1688.67&10.78&0.19&12.14&1727.80&10.54&0.15&15.38&1684.25&1.43&0.71&71.43&1758.60&1.00&0.33&33.33&1822.00&830.22&0.36&12.81&1862.38&46.94&0.17&6.47&1886.50&1058.89&0.17&6.58&1860.83&468.53&0.28&4.77&1881.40\\ \hline
Lang&CLASS&376.83&0.34&4.60&83.35&79.40&0.23&3.69&45.64&10.63&0.15&4.29&54.75&11.04&0.11&7.78&86.33&10.78&0.19&12.14&55.60&10.54&0.15&15.38&67.75&1.43&0.71&71.43&35.00&1.00&0.33&33.33&49.00&830.22&0.36&12.81&89.62&46.94&0.17&6.47&36.50&1058.89&0.17&6.58&69.67&468.53&0.28&4.77&76.20\\ \hline
Lang&METHOD&376.83&0.34&4.60&14.10&79.40&0.23&3.69&7.82&10.63&0.15&4.29&5.00&11.04&0.11&7.78&6.00&10.78&0.19&12.14&4.40&10.54&0.15&15.38&5.00&1.43&0.71&71.43&3.00&1.00&0.33&33.33&1.00&830.22&0.36&12.81&6.15&46.94&0.17&6.47&3.17&1058.89&0.17&6.58&3.33&468.53&0.28&4.77&6.20\\ \hline
Lang&STATE&376.83&0.34&4.60&13.05&79.40&0.23&3.69&7.09&10.63&0.15&4.29&4.50&11.04&0.11&7.78&5.33&10.78&0.19&12.14&3.60&10.54&0.15&15.38&4.25&1.43&0.71&71.43&1.80&1.00&0.33&33.33&1.00&830.22&0.36&12.81&5.46&46.94&0.17&6.47&2.33&1058.89&0.17&6.58&2.50&468.53&0.28&4.77&4.90\\ \hline
Math&NORTS&1141.03&0.52&4.69&2871.75&35.91&0.34&14.44&2597.14&7.39&0.04&3.80&3040.67&6.48&0.06&5.20&3644.00&6.26&0.16&12.29&3618.46&6.18&0.08&7.79&2930.00&1.21&0.84&78.95&2301.31&1.67&0.33&33.33&2364.00&701.81&0.38&14.13&2723.89&10.78&0.11&5.22&3440.90&800.10&0.30&7.04&2751.83&393.51&0.31&6.21&2760.10\\ \hline
Math&CLASS&1141.03&0.52&4.69&112.49&35.91&0.34&14.44&353.90&7.39&0.04&3.80&23.33&6.48&0.06&5.20&635.80&6.26&0.16&12.29&123.62&6.18&0.08&7.79&25.33&1.21&0.84&78.95&52.12&1.67&0.33&33.33&15.00&701.81&0.38&14.13&158.50&10.78&0.11&5.22&34.70&800.10&0.30&7.04&251.93&393.51&0.31&6.21&88.90\\ \hline
Math&METHOD&1141.03&0.52&4.69&32.67&35.91&0.34&14.44&48.21&7.39&0.04&3.80&14.33&6.48&0.06&5.20&13.20&6.26&0.16&12.29&10.85&6.18&0.08&7.79&9.17&1.21&0.84&78.95&33.06&1.67&0.33&33.33&15.00&701.81&0.38&14.13&40.50&10.78&0.11&5.22&11.40&800.10&0.30&7.04&56.55&393.51&0.31&6.21&41.17\\ \hline
Math&STATE&1141.03&0.52&4.69&19.04&35.91&0.34&14.44&46.28&7.39&0.04&3.80&4.00&6.48&0.06&5.20&7.00&6.26&0.16&12.29&5.15&6.18&0.08&7.79&1.17&1.21&0.84&78.95&26.81&1.67&0.33&33.33&1.00&701.81&0.38&14.13&17.03&10.78&0.11&5.22&5.00&800.10&0.30&7.04&22.55&393.51&0.31&6.21&14.76\\ \hline
Time&NORTS&790.08&0.54&1.01&3921.93&57.11&0.22&6.02&3940.00&5.91&0.09&3.03&3893.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&3893.00&3.50&0.12&12.50&3893.00&2.00&0.33&33.33&3906.00&1.00&0.00&0.00&nan&714.90&0.20&0.42&3899.50&39.62&0.00&0.00&nan&885.44&0.11&0.02&3893.00&235.44&0.11&0.04&3893.00\\ \hline
Time&CLASS&790.08&0.54&1.01&1335.57&57.11&0.22&6.02&721.50&5.91&0.09&3.03&832.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&832.00&3.50&0.12&12.50&832.00&2.00&0.33&33.33&1607.00&1.00&0.00&0.00&nan&714.90&0.20&0.42&2092.50&39.62&0.00&0.00&nan&885.44&0.11&0.02&832.00&235.44&0.11&0.04&832.00\\ \hline
Time&METHOD&790.08&0.54&1.01&357.50&57.11&0.22&6.02&28.50&5.91&0.09&3.03&15.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&15.00&3.50&0.12&12.50&15.00&2.00&0.33&33.33&21.00&1.00&0.00&0.00&nan&714.90&0.20&0.42&170.00&39.62&0.00&0.00&nan&885.44&0.11&0.02&326.00&235.44&0.11&0.04&298.00\\ \hline
Time&STATE&790.08&0.54&1.01&227.86&57.11&0.22&6.02&17.50&5.91&0.09&3.03&15.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&15.00&3.50&0.12&12.50&15.00&2.00&0.33&33.33&21.00&1.00&0.00&0.00&nan&714.90&0.20&0.42&34.00&39.62&0.00&0.00&nan&885.44&0.11&0.02&97.00&235.44&0.11&0.04&26.00\\ \hline
Chart&NORTS&656.40&0.68&10.08&1840.41&68.52&0.09&2.66&1728.00&6.58&0.16&13.16&1687.00&6.33&0.06&5.56&1816.00&5.79&0.21&21.05&1719.25&6.59&0.06&5.88&1625.00&1.00&0.90&90.00&1823.00&nan&nan&nan&nan&436.26&0.61&17.77&1847.71&40.50&0.41&9.97&1855.44&682.29&0.33&3.95&1851.12&239.38&0.50&6.41&1862.50\\ \hline
Chart&CLASS&656.40&0.68&10.08&147.12&68.52&0.09&2.66&60.50&6.58&0.16&13.16&11.33&6.33&0.06&5.56&23.00&5.79&0.21&21.05&14.25&6.59&0.06&5.88&10.00&1.00&0.90&90.00&85.78&nan&nan&nan&nan&436.26&0.61&17.77&195.57&40.50&0.41&9.97&146.56&682.29&0.33&3.95&223.75&239.38&0.50&6.41&161.92\\ \hline
Chart&METHOD&656.40&0.68&10.08&29.41&68.52&0.09&2.66&49.50&6.58&0.16&13.16&2.67&6.33&0.06&5.56&3.00&5.79&0.21&21.05&2.75&6.59&0.06&5.88&1.00&1.00&0.90&90.00&18.44&nan&nan&nan&nan&436.26&0.61&17.77&32.14&40.50&0.41&9.97&22.89&682.29&0.33&3.95&28.88&239.38&0.50&6.41&27.67\\ \hline
Chart&STATE&656.40&0.68&10.08&24.35&68.52&0.09&2.66&49.50&6.58&0.16&13.16&2.67&6.33&0.06&5.56&3.00&5.79&0.21&21.05&2.75&6.59&0.06&5.88&1.00&1.00&0.90&90.00&18.00&nan&nan&nan&nan&436.26&0.61&17.77&15.86&40.50&0.41&9.97&13.78&682.29&0.33&3.95&12.25&239.38&0.50&6.41&9.33\\ \hline
Mockito&NORTS&1990.14&0.25&0.92&1078.67&nan&nan&nan&nan&3.75&0.25&25.00&900.75&4.80&0.00&0.00&nan&4.33&0.20&20.00&980.67&4.43&0.07&3.57&1324.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&1990.14&0.25&0.92&298.33&nan&nan&nan&nan&3.75&0.25&25.00&353.00&4.80&0.00&0.00&nan&4.33&0.20&20.00&711.67&4.43&0.07&3.57&783.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&1990.14&0.25&0.92&201.56&nan&nan&nan&nan&3.75&0.25&25.00&16.00&4.80&0.00&0.00&nan&4.33&0.20&20.00&219.33&4.43&0.07&3.57&4.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&1990.14&0.25&0.92&201.56&nan&nan&nan&nan&3.75&0.25&25.00&15.00&4.80&0.00&0.00&nan&4.33&0.20&20.00&16.00&4.43&0.07&3.57&4.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&nan&nan&nan&nan&5.71&0.57&41.56&7371.44&3.94&0.04&3.19&7325.00&3.62&0.04&4.44&7409.50&3.90&0.06&6.38&7324.83&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&nan&nan&nan&nan&5.71&0.57&41.56&4046.13&3.94&0.04&3.19&3067.25&3.62&0.04&4.44&3121.75&3.90&0.06&6.38&2947.50&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&nan&nan&nan&nan&5.71&0.57&41.56&773.69&3.94&0.04&3.19&45.00&3.62&0.04&4.44&135.25&3.90&0.06&6.38&42.33&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&nan&nan&nan&nan&5.71&0.57&41.56&280.72&3.94&0.04&3.19&5.50&3.62&0.04&4.44&3.50&3.90&0.06&6.38&7.83&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&990.90&0.47&4.26&2304.95&49.33&0.29&13.67&3494.93&6.37&0.12&8.74&3096.36&6.17&0.05&3.83&3639.54&6.06&0.15&13.49&3210.67&5.69&0.08&7.52&2291.25&1.41&0.70&68.43&2447.23&1.22&0.22&22.22&2093.00&670.80&0.39&11.28&2583.37&34.46&0.17&5.42&2394.28&856.68&0.23&4.40&2589.20&334.21&0.30&4.36&2599.25\\ \hline
All &CLASS&990.90&0.47&4.26&395.37&49.33&0.29&13.67&1045.53&6.37&0.12&8.74&723.61&6.17&0.05&3.83&966.72&6.06&0.15&13.49&780.77&5.69&0.08&7.52&343.62&1.41&0.70&68.43&444.98&1.22&0.22&22.22&32.00&670.80&0.39&11.28&634.05&34.46&0.17&5.42&72.59&856.68&0.23&4.40&344.34&334.21&0.30&4.36&289.75\\ \hline
All &METHOD&990.90&0.47&4.26&127.05&49.33&0.29&13.67&181.54&6.37&0.12&8.74&16.33&6.17&0.05&3.83&39.36&6.06&0.15&13.49&49.11&5.69&0.08&7.52&6.83&1.41&0.70&68.43&18.88&1.22&0.22&22.22&8.00&670.80&0.39&11.28&62.20&34.46&0.17&5.42&12.49&856.68&0.23&4.40&103.69&334.21&0.30&4.36&93.26\\ \hline
All &STATE&990.90&0.47&4.26&97.17&49.33&0.29&13.67&80.22&6.37&0.12&8.74&7.78&6.17&0.05&3.83&4.71&6.06&0.15&13.49&8.39&5.69&0.08&7.52&5.08&1.41&0.70&68.43&16.90&1.22&0.22&22.22&1.00&670.80&0.39&11.28&18.09&34.46&0.17&5.42&7.04&856.68&0.23&4.40&33.58&334.21&0.30&4.36&13.75\\ \hline


    \end{tabular}
    \end{adjustbox}
\end{table*} 

==> tables/StopF_ave_latex_table.tex <==
\begin{table*}
    \centering
   \caption{(StopF) Average executed tests with different \rts{} on all APR systems  }\label{table:ave_test_summary}
   	\begin{adjustbox}{width=2\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 


Lang&NORTS&nan&nan&nan&nan&80.79&80.60&96.38&1.00&10.63&10.41&95.18&1.00&11.00&10.89&92.33&1.00&10.93&10.63&87.13&1.00&10.88&10.73&88.17&1.00&1.43&0.71&28.57&1.00&1.00&0.67&66.67&1.00&900.67&857.53&84.40&1.14&47.69&47.20&93.24&1.15&1083.03&1021.50&90.65&1.04&498.11&492.31&95.93&1.04\\ \hline
Lang&CLASS&nan&nan&nan&nan&80.79&80.60&96.38&1.00&10.63&10.41&95.18&1.00&11.00&10.89&92.33&1.00&10.93&10.63&87.13&1.00&10.88&10.73&88.17&1.00&1.43&0.71&28.57&1.00&1.00&0.67&66.67&1.00&900.67&857.53&84.40&1.14&47.69&47.20&93.24&1.15&1083.03&1021.50&90.65&1.04&498.11&492.31&95.93&1.04\\ \hline
Lang&METHOD&nan&nan&nan&nan&80.79&80.60&96.38&1.00&10.63&10.41&95.18&1.00&11.00&10.89&92.33&1.00&10.93&10.63&87.13&1.00&10.88&10.73&88.17&1.00&1.43&0.71&28.57&1.00&1.00&0.67&66.67&1.00&900.67&857.53&84.40&1.14&47.69&47.20&93.24&1.15&1083.03&1021.50&90.65&1.04&498.11&492.31&95.93&1.04\\ \hline
Lang&STATE&nan&nan&nan&nan&80.79&80.60&96.38&1.00&10.63&10.41&95.18&1.00&11.00&10.89&92.33&1.00&10.93&10.63&87.13&1.00&10.88&10.73&88.17&1.00&1.43&0.71&28.57&1.00&1.00&0.67&66.67&1.00&900.67&857.53&84.40&1.14&47.69&47.20&93.24&1.15&1083.03&1021.50&90.65&1.04&498.11&492.31&95.93&1.04\\ \hline
Math&NORTS&nan&nan&nan&nan&35.90&35.33&85.13&1.03&7.39&7.30&95.52&1.00&6.48&6.42&94.80&1.00&6.26&6.04&86.54&1.00&6.18&6.09&92.02&1.00&1.21&0.26&14.04&1.00&1.67&1.33&66.67&1.00&837.59&735.18&79.35&1.04&11.49&11.06&93.33&1.00&893.95&843.50&88.62&1.01&433.24&427.38&95.84&1.00\\ \hline
Math&CLASS&nan&nan&nan&nan&35.90&35.33&85.13&1.03&7.39&7.30&95.52&1.00&6.48&6.42&94.80&1.00&6.26&6.04&86.54&1.00&6.18&6.09&92.02&1.00&1.21&0.26&14.04&1.00&1.67&1.33&66.67&1.00&837.59&735.18&79.35&1.04&11.49&11.06&93.33&1.00&893.95&843.50&88.62&1.01&433.24&427.38&95.84&1.00\\ \hline
Math&METHOD&nan&nan&nan&nan&35.90&35.33&85.13&1.03&7.39&7.30&95.52&1.00&6.48&6.42&94.80&1.00&6.26&6.04&86.54&1.00&6.18&6.09&92.02&1.00&1.21&0.26&14.04&1.00&1.67&1.33&66.67&1.00&837.59&735.18&79.35&1.04&11.49&11.06&93.33&1.00&893.95&843.50&88.62&1.01&433.24&427.38&95.84&1.00\\ \hline
Math&STATE&nan&nan&nan&nan&35.90&35.33&85.13&1.03&7.39&7.30&95.52&1.00&6.48&6.42&94.80&1.00&6.26&6.04&86.54&1.00&6.18&6.09&92.02&1.00&1.21&0.26&14.04&1.00&1.67&1.33&66.67&1.00&837.59&735.18&79.35&1.04&11.49&11.06&93.33&1.00&893.95&843.50&88.62&1.01&433.24&427.38&95.84&1.00\\ \hline
Time&NORTS&nan&nan&nan&nan&53.91&53.73&96.86&1.00&5.91&5.64&90.91&1.00&4.73&4.73&100.00&1.00&5.27&5.18&90.91&1.00&3.50&3.38&87.50&1.00&2.00&1.67&66.67&1.00&1.00&1.00&100.00&1.00&794.00&757.36&93.94&1.03&34.40&34.10&97.72&1.00&989.60&895.10&92.11&1.00&279.40&278.00&99.79&1.00\\ \hline
Time&CLASS&nan&nan&nan&nan&53.91&53.73&96.86&1.00&5.91&5.64&90.91&1.00&4.73&4.73&100.00&1.00&5.27&5.18&90.91&1.00&3.50&3.38&87.50&1.00&2.00&1.67&66.67&1.00&1.00&1.00&100.00&1.00&794.00&757.36&93.94&1.03&34.40&34.10&97.72&1.00&989.60&895.10&92.11&1.00&279.40&278.00&99.79&1.00\\ \hline
Time&METHOD&nan&nan&nan&nan&53.91&53.73&96.86&1.00&5.91&5.64&90.91&1.00&4.73&4.73&100.00&1.00&5.27&5.18&90.91&1.00&3.50&3.38&87.50&1.00&2.00&1.67&66.67&1.00&1.00&1.00&100.00&1.00&794.00&757.36&93.94&1.03&34.40&34.10&97.72&1.00&989.60&895.10&92.11&1.00&279.40&278.00&99.79&1.00\\ \hline
Time&STATE&nan&nan&nan&nan&53.91&53.73&96.86&1.00&5.91&5.64&90.91&1.00&4.73&4.73&100.00&1.00&5.27&5.18&90.91&1.00&3.50&3.38&87.50&1.00&2.00&1.67&66.67&1.00&1.00&1.00&100.00&1.00&794.00&757.36&93.94&1.03&34.40&34.10&97.72&1.00&989.60&895.10&92.11&1.00&279.40&278.00&99.79&1.00\\ \hline
Chart&NORTS&nan&nan&nan&nan&68.43&68.35&97.34&1.00&6.58&6.42&86.84&1.01&6.33&6.28&94.44&1.08&5.79&5.58&78.95&1.03&6.59&6.53&94.12&1.00&1.00&0.10&10.00&1.00&nan&nan&nan&nan&682.35&505.48&78.40&1.09&48.14&46.82&89.60&1.01&760.12&687.21&88.57&1.05&347.04&340.46&96.07&1.01\\ \hline
Chart&CLASS&nan&nan&nan&nan&68.43&68.35&97.34&1.00&6.58&6.42&86.84&1.01&6.33&6.28&94.44&1.08&5.79&5.58&78.95&1.03&6.59&6.53&94.12&1.00&1.00&0.10&10.00&1.00&nan&nan&nan&nan&682.35&505.48&78.40&1.09&48.14&46.82&89.60&1.01&760.12&687.21&88.57&1.05&347.04&340.46&96.07&1.01\\ \hline
Chart&METHOD&nan&nan&nan&nan&68.43&68.35&97.34&1.00&6.58&6.42&86.84&1.01&6.33&6.28&94.44&1.08&5.79&5.58&78.95&1.03&6.59&6.53&94.12&1.00&1.00&0.10&10.00&1.00&nan&nan&nan&nan&682.35&505.48&78.40&1.09&48.14&46.82&89.60&1.01&760.12&687.21&88.57&1.05&347.04&340.46&96.07&1.01\\ \hline
Chart&STATE&nan&nan&nan&nan&68.43&68.35&97.34&1.00&6.58&6.42&86.84&1.01&6.33&6.28&94.44&1.08&5.79&5.58&78.95&1.03&6.59&6.53&94.12&1.00&1.00&0.10&10.00&1.00&nan&nan&nan&nan&682.35&505.48&78.40&1.09&48.14&46.82&89.60&1.01&760.12&687.21&88.57&1.05&347.04&340.46&96.07&1.01\\ \hline
Mockito&NORTS&nan&nan&nan&nan&nan&nan&nan&nan&3.75&3.44&73.75&1.00&4.80&4.73&98.67&1.00&4.33&4.13&80.00&1.00&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&nan&nan&nan&nan&nan&nan&nan&nan&3.75&3.44&73.75&1.00&4.80&4.73&98.67&1.00&4.33&4.13&80.00&1.00&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&nan&nan&nan&nan&nan&nan&nan&nan&3.75&3.44&73.75&1.00&4.80&4.73&98.67&1.00&4.33&4.13&80.00&1.00&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&nan&nan&nan&nan&nan&nan&nan&nan&3.75&3.44&73.75&1.00&4.80&4.73&98.67&1.00&4.33&4.13&80.00&1.00&4.62&4.62&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&nan&nan&nan&nan&5.71&5.14&58.44&1.02&3.94&3.88&96.45&1.00&3.62&3.53&94.37&1.00&3.90&3.83&93.40&1.00&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&nan&nan&nan&nan&5.71&5.14&58.44&1.02&3.94&3.88&96.45&1.00&3.62&3.53&94.37&1.00&3.90&3.83&93.40&1.00&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&nan&nan&nan&nan&5.71&5.14&58.44&1.02&3.94&3.88&96.45&1.00&3.62&3.53&94.37&1.00&3.90&3.83&93.40&1.00&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&nan&nan&nan&nan&5.71&5.14&58.44&1.02&3.94&3.88&96.45&1.00&3.62&3.53&94.37&1.00&3.90&3.83&93.40&1.00&2.89&2.89&100.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&nan&nan&nan&nan&48.95&48.63&86.83&1.01&6.37&6.18&89.78&1.00&6.16&6.10&95.77&1.01&6.08&5.90&86.15&1.01&5.78&5.71&93.63&1.00&1.41&0.69&29.82&1.00&1.22&1.00&77.78&1.00&803.65&713.89&84.02&1.08&35.43&34.79&93.47&1.04&931.68&861.83&89.99&1.02&389.45&384.54&96.91&1.01\\ \hline
All &CLASS&nan&nan&nan&nan&48.95&48.63&86.83&1.01&6.37&6.18&89.78&1.00&6.16&6.10&95.77&1.01&6.08&5.90&86.15&1.01&5.78&5.71&93.63&1.00&1.41&0.69&29.82&1.00&1.22&1.00&77.78&1.00&803.65&713.89&84.02&1.08&35.43&34.79&93.47&1.04&931.68&861.83&89.99&1.02&389.45&384.54&96.91&1.01\\ \hline
All &METHOD&nan&nan&nan&nan&48.95&48.63&86.83&1.01&6.37&6.18&89.78&1.00&6.16&6.10&95.77&1.01&6.08&5.90&86.15&1.01&5.78&5.71&93.63&1.00&1.41&0.69&29.82&1.00&1.22&1.00&77.78&1.00&803.65&713.89&84.02&1.08&35.43&34.79&93.47&1.04&931.68&861.83&89.99&1.02&389.45&384.54&96.91&1.01\\ \hline
All &STATE&nan&nan&nan&nan&48.95&48.63&86.83&1.01&6.37&6.18&89.78&1.00&6.16&6.10&95.77&1.01&6.08&5.90&86.15&1.01&5.78&5.71&93.63&1.00&1.41&0.69&29.82&1.00&1.22&1.00&77.78&1.00&803.65&713.89&84.02&1.08&35.43&34.79&93.47&1.04&931.68&861.83&89.99&1.02&389.45&384.54&96.91&1.01\\ \hline


    \end{tabular}
    \end{adjustbox}
\end{table*} 


\begin{table*}
    \centering
   \caption{Full-(StopF) Average executed tests with different \rts{} on all APR systems  }\label{table:full_nonplausible_at_summary}
   	\begin{adjustbox}{width=2.1\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 
    
    
    Lang&NORTS&376.83&376.27&95.24&1869.09&79.40&79.17&96.31&1855.21&10.63&10.41&95.18&1793.33&11.04&10.89&91.96&1810.96&10.78&10.44&86.51&1798.33&10.54&10.35&84.32&1816.95&1.43&0.71&28.57&1741.00&1.00&0.67&66.67&2288.50&830.22&814.97&83.21&1948.91&46.94&46.11&92.01&1960.48&1058.89&1016.69&90.02&1956.41&468.53&464.56&93.91&1950.31\\ \hline
Lang&CLASS&376.83&376.27&95.24&76.12&79.40&79.17&96.31&63.54&10.63&10.41&95.18&52.35&11.04&10.89&91.96&50.98&10.78&10.44&86.51&51.42&10.54&10.35&84.32&53.59&1.43&0.71&28.57&42.00&1.00&0.67&66.67&79.50&830.22&814.97&83.21&65.78&46.94&46.11&92.01&60.08&1058.89&1016.69&90.02&69.50&468.53&464.56&93.91&68.11\\ \hline
Lang&METHOD&376.83&376.27&95.24&15.40&79.40&79.17&96.31&11.17&10.63&10.41&95.18&6.60&11.04&10.89&91.96&7.06&10.78&10.44&86.51&6.49&10.54&10.35&84.32&6.66&1.43&0.71&28.57&26.00&1.00&0.67&66.67&8.50&830.22&814.97&83.21&11.02&46.94&46.11&92.01&10.92&1058.89&1016.69&90.02&11.49&468.53&464.56&93.91&10.11\\ \hline
Lang&STATE&376.83&376.27&95.24&13.81&79.40&79.17&96.31&9.83&10.63&10.41&95.18&4.22&11.04&10.89&91.96&4.85&10.78&10.44&86.51&4.72&10.54&10.35&84.32&4.07&1.43&0.71&28.57&19.50&1.00&0.67&66.67&5.50&830.22&814.97&83.21&9.18&46.94&46.11&92.01&9.63&1058.89&1016.69&90.02&9.05&468.53&464.56&93.91&8.29\\ \hline
Math&NORTS&1141.03&1136.77&94.36&2818.48&35.91&35.10&84.41&2836.13&7.39&7.30&95.52&2789.29&6.48&6.42&94.80&2775.16&6.26&6.04&86.54&2659.69&6.18&6.09&92.02&2722.42&1.21&0.26&14.04&2044.25&1.67&1.33&66.67&2289.50&701.81&664.39&80.24&2773.42&10.78&10.53&92.82&2731.18&800.10&771.31&88.39&2757.52&393.51&389.01&92.50&2708.03\\ \hline
Math&CLASS&1141.03&1136.77&94.36&241.96&35.91&35.10&84.41&363.11&7.39&7.30&95.52&194.57&6.48&6.42&94.80&203.99&6.26&6.04&86.54&199.62&6.18&6.09&92.02&268.34&1.21&0.26&14.04&175.50&1.67&1.33&66.67&290.50&701.81&664.39&80.24&164.06&10.78&10.53&92.82&123.74&800.10&771.31&88.39&192.02&393.51&389.01&92.50&136.47\\ \hline
Math&METHOD&1141.03&1136.77&94.36&70.54&35.91&35.10&84.41&58.74&7.39&7.30&95.52&21.83&6.48&6.42&94.80&27.18&6.26&6.04&86.54&25.64&6.18&6.09&92.02&26.82&1.21&0.26&14.04&67.25&1.67&1.33&66.67&126.00&701.81&664.39&80.24&33.92&10.78&10.53&92.82&24.75&800.10&771.31&88.39&34.78&393.51&389.01&92.50&29.75\\ \hline
Math&STATE&1141.03&1136.77&94.36&61.41&35.91&35.10&84.41&44.87&7.39&7.30&95.52&9.28&6.48&6.42&94.80&12.66&6.26&6.04&86.54&8.11&6.18&6.09&92.02&10.66&1.21&0.26&14.04&38.75&1.67&1.33&66.67&59.00&701.81&664.39&80.24&19.36&10.78&10.53&92.82&14.29&800.10&771.31&88.39&19.56&393.51&389.01&92.50&16.37\\ \hline
Time&NORTS&790.08&788.00&98.81&3923.62&57.11&56.89&93.98&3920.67&5.91&5.64&90.91&3945.00&4.73&4.73&100.00&3941.36&5.27&5.18&90.91&3945.00&3.50&3.38&87.50&3923.14&2.00&1.67&66.67&3879.50&1.00&1.00&100.00&4041.00&714.90&714.00&98.00&3879.70&39.62&39.38&97.81&3885.62&885.44&836.44&90.72&3879.44&235.44&235.33&99.96&3879.44\\ \hline
Time&CLASS&790.08&788.00&98.81&1090.54&57.11&56.89&93.98&1097.44&5.91&5.64&90.91&1290.62&4.73&4.73&100.00&879.82&5.27&5.18&90.91&1082.77&3.50&3.38&87.50&719.57&2.00&1.67&66.67&2000.50&1.00&1.00&100.00&139.00&714.90&714.00&98.00&1478.66&39.62&39.38&97.81&1377.44&885.44&836.44&90.72&1663.95&235.44&235.33&99.96&1429.74\\ \hline
Time&METHOD&790.08&788.00&98.81&302.80&57.11&56.89&93.98&46.47&5.91&5.64&90.91&97.90&4.73&4.73&100.00&45.18&5.27&5.18&90.91&50.82&3.50&3.38&87.50&68.29&2.00&1.67&66.67&238.50&1.00&1.00&100.00&7.00&714.90&714.00&98.00&326.23&39.62&39.38&97.81&250.43&885.44&836.44&90.72&483.52&235.44&235.33&99.96&380.28\\ \hline
Time&STATE&790.08&788.00&98.81&250.21&57.11&56.89&93.98&38.64&5.91&5.64&90.91&8.91&4.73&4.73&100.00&10.70&5.27&5.18&90.91&5.45&3.50&3.38&87.50&7.86&2.00&1.67&66.67&235.00&1.00&1.00&100.00&7.00&714.90&714.00&98.00&281.22&39.62&39.38&97.81&231.39&885.44&836.44&90.72&440.45&235.44&235.33&99.96&355.35\\ \hline
Chart&NORTS&656.40&655.40&89.78&1827.22&68.52&68.35&96.67&1835.39&6.58&6.42&86.84&1880.82&6.33&6.28&94.44&1869.29&5.79&5.58&78.95&1889.47&6.59&6.53&94.12&1889.44&1.00&0.10&10.00&1650.00&nan&nan&nan&nan&436.26&435.61&82.22&1836.62&40.50&40.00&89.96&1845.57&682.29&644.25&92.65&1829.83&239.38&238.83&93.46&1827.22\\ \hline
Chart&CLASS&656.40&655.40&89.78&100.52&68.52&68.35&96.67&108.38&6.58&6.42&86.84&92.65&6.33&6.28&94.44&72.35&5.79&5.58&78.95&86.95&6.59&6.53&94.12&71.64&1.00&0.10&10.00&278.00&nan&nan&nan&nan&436.26&435.61&82.22&122.55&40.50&40.00&89.96&100.14&682.29&644.25&92.65&135.57&239.38&238.83&93.46&108.00\\ \hline
Chart&METHOD&656.40&655.40&89.78&48.69&68.52&68.35&96.67&47.88&6.58&6.42&86.84&12.94&6.33&6.28&94.44&13.10&5.79&5.58&78.95&14.88&6.59&6.53&94.12&14.63&1.00&0.10&10.00&84.00&nan&nan&nan&nan&436.26&435.61&82.22&30.44&40.50&40.00&89.96&34.51&682.29&644.25&92.65&33.06&239.38&238.83&93.46&27.54\\ \hline
Chart&STATE&656.40&655.40&89.78&46.39&68.52&68.35&96.67&46.95&6.58&6.42&86.84&6.51&6.33&6.28&94.44&7.29&5.79&5.58&78.95&6.97&6.59&6.53&94.12&6.68&1.00&0.10&10.00&84.00&nan&nan&nan&nan&436.26&435.61&82.22&17.87&40.50&40.00&89.96&30.91&682.29&644.25&92.65&21.37&239.38&238.83&93.46&23.34\\ \hline
Mockito&NORTS&1990.14&1983.92&98.67&1128.64&nan&nan&nan&nan&3.75&3.44&73.75&1040.17&4.80&4.73&98.67&1048.20&4.33&4.13&80.00&1028.25&4.43&4.36&96.43&1088.43&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&1990.14&1983.92&98.67&700.04&nan&nan&nan&nan&3.75&3.44&73.75&406.02&4.80&4.73&98.67&345.37&4.33&4.13&80.00&356.00&4.43&4.36&96.43&391.72&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&1990.14&1983.92&98.67&560.80&nan&nan&nan&nan&3.75&3.44&73.75&238.55&4.80&4.73&98.67&164.89&4.33&4.13&80.00&188.73&4.43&4.36&96.43&190.71&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&1990.14&1983.92&98.67&540.06&nan&nan&nan&nan&3.75&3.44&73.75&16.03&4.80&4.73&98.67&27.59&4.33&4.13&80.00&16.47&4.43&4.36&96.43&14.84&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&nan&nan&nan&nan&5.71&5.14&58.44&7109.74&3.94&3.88&96.45&7123.15&3.62&3.53&94.37&7190.97&3.90&3.83&93.40&7168.38&2.89&2.89&100.00&7502.06&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&nan&nan&nan&nan&5.71&5.14&58.44&4314.90&3.94&3.88&96.45&3827.19&3.62&3.53&94.37&4119.66&3.90&3.83&93.40&4229.50&2.89&2.89&100.00&3419.44&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&nan&nan&nan&nan&5.71&5.14&58.44&669.15&3.94&3.88&96.45&2106.11&3.62&3.53&94.37&2204.95&3.90&3.83&93.40&2280.32&2.89&2.89&100.00&685.57&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&nan&nan&nan&nan&5.71&5.14&58.44&231.78&3.94&3.88&96.45&1099.68&3.62&3.53&94.37&1039.23&3.90&3.83&93.40&987.33&2.89&2.89&100.00&134.63&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&990.90&988.07&95.37&2313.41&49.33&48.93&85.96&3511.43&6.37&6.18&89.78&3095.29&6.17&6.10&95.71&3105.99&6.06&5.87&86.05&3081.52&5.69&5.60&92.40&3157.07&1.41&0.69&29.82&2328.69&1.22&1.00&77.78&2873.00&670.80&657.24&85.92&2609.66&34.46&34.01&93.15&2605.71&856.68&817.18&90.45&2605.80&334.21&331.93&94.96&2591.25\\ \hline
All &CLASS&990.90&988.07&95.37&441.83&49.33&48.93&85.96&1189.48&6.37&6.18&89.78&977.23&6.17&6.10&95.71&945.36&6.06&5.87&86.05&1001.04&5.69&5.60&92.40&820.72&1.41&0.69&29.82&624.00&1.22&1.00&77.78&169.67&670.80&657.24&85.92&457.76&34.46&34.01&93.15&415.35&856.68&817.18&90.45&515.26&334.21&331.93&94.96&435.58\\ \hline
All &METHOD&990.90&988.07&95.37&199.65&49.33&48.93&85.96&166.68&6.37&6.18&89.78&413.99&6.17&6.10&95.71&410.39&6.06&5.87&86.05&427.82&5.69&5.60&92.40&165.45&1.41&0.69&29.82&103.94&1.22&1.00&77.78&47.17&670.80&657.24&85.92&100.40&34.46&34.01&93.15&80.15&856.68&817.18&90.45&140.71&334.21&331.93&94.96&111.92\\ \hline
All &STATE&990.90&988.07&95.37&182.38&49.33&48.93&85.96&74.41&6.37&6.18&89.78&190.77&6.17&6.10&95.71&183.72&6.06&5.87&86.05&171.51&5.69&5.60&92.40&29.79&1.41&0.69&29.82&94.31&1.22&1.00&77.78&23.83&670.80&657.24&85.92&81.91&34.46&34.01&93.15&71.55&856.68&817.18&90.45&122.61&334.21&331.93&94.96&100.84\\ \hline



    \end{tabular}
    \end{adjustbox}
\end{table*} 

==> tables/StopP_ave_latex_table.tex <==
\begin{table*}
    \centering
   \caption{(StopP) Average executed tests with different \rts{} on all APR systems  }\label{table:ave_test_summary}
   	\begin{adjustbox}{width=2\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 
    
Lang&NORTS&400.66&0.97&4.68&1686.33&80.79&0.19&3.62&1834.78&10.63&0.22&4.82&1532.40&11.00&0.11&7.67&1370.67&10.93&0.30&12.87&1539.67&10.88&0.15&11.83&1445.75&1.43&0.71&71.43&1758.60&1.00&0.33&33.33&1822.00&900.67&43.14&15.60&1619.66&47.69&0.49&6.76&1681.56&1083.03&61.53&9.35&1669.48&498.11&5.81&4.07&1820.55\\ \hline
Lang&CLASS&400.66&0.97&4.68&64.05&80.79&0.19&3.62&27.89&10.63&0.22&4.82&46.40&11.00&0.11&7.67&66.67&10.93&0.30&12.87&48.67&10.88&0.15&11.83&53.00&1.43&0.71&71.43&35.00&1.00&0.33&33.33&49.00&900.67&43.14&15.60&70.31&47.69&0.49&6.76&32.73&1083.03&61.53&9.35&45.43&498.11&5.81&4.07&64.76\\ \hline
Lang&METHOD&400.66&0.97&4.68&8.06&80.79&0.19&3.62&8.78&10.63&0.22&4.82&6.60&11.00&0.11&7.67&9.00&10.93&0.30&12.87&6.00&10.88&0.15&11.83&7.50&1.43&0.71&71.43&3.00&1.00&0.33&33.33&1.00&900.67&43.14&15.60&3.94&47.69&0.49&6.76&5.12&1083.03&61.53&9.35&5.73&498.11&5.81&4.07&5.21\\ \hline
Lang&STATE&400.66&0.97&4.68&6.88&80.79&0.19&3.62&7.89&10.63&0.22&4.82&4.60&11.00&0.11&7.67&6.33&10.93&0.30&12.87&4.33&10.88&0.15&11.83&5.00&1.43&0.71&71.43&1.80&1.00&0.33&33.33&1.00&900.67&43.14&15.60&3.53&47.69&0.49&6.76&3.46&1083.03&61.53&9.35&4.43&498.11&5.81&4.07&3.04\\ \hline
Math&NORTS&1513.39&8.12&5.08&1897.75&35.90&0.57&14.87&2417.57&7.39&0.09&4.48&2137.00&6.48&0.06&5.20&3644.00&6.26&0.23&13.46&2955.41&6.18&0.09&7.98&2566.14&1.21&0.95&85.96&2155.94&1.67&0.33&33.33&2364.00&837.59&102.42&20.65&1773.15&11.49&0.43&6.67&2150.35&893.95&50.45&11.38&1840.36&433.24&5.86&4.16&2002.59\\ \hline
Math&CLASS&1513.39&8.12&5.08&62.28&35.90&0.57&14.87&347.63&7.39&0.09&4.48&83.60&6.48&0.06&5.20&635.80&6.26&0.23&13.46&115.00&6.18&0.09&7.98&37.14&1.21&0.95&85.96&53.33&1.67&0.33&33.33&15.00&837.59&102.42&20.65&65.37&11.49&0.43&6.67&26.10&893.95&50.45&11.38&94.72&433.24&5.86&4.16&52.84\\ \hline
Math&METHOD&1513.39&8.12&5.08&10.92&35.90&0.57&14.87&47.41&7.39&0.09&4.48&11.80&6.48&0.06&5.20&13.20&6.26&0.23&13.46&9.47&6.18&0.09&7.98&10.29&1.21&0.95&85.96&34.06&1.67&0.33&33.33&15.00&837.59&102.42&20.65&22.25&11.49&0.43&6.67&12.71&893.95&50.45&11.38&18.03&433.24&5.86&4.16&19.20\\ \hline
Math&STATE&1513.39&8.12&5.08&8.85&35.90&0.57&14.87&45.57&7.39&0.09&4.48&5.60&6.48&0.06&5.20&7.00&6.26&0.23&13.46&5.12&6.18&0.09&7.98&1.57&1.21&0.95&85.96&28.22&1.67&0.33&33.33&1.00&837.59&102.42&20.65&8.49&11.49&0.43&6.67&5.54&893.95&50.45&11.38&10.02&433.24&5.86&4.16&7.20\\ \hline
Time&NORTS&1466.54&6.88&1.22&1806.56&53.91&0.18&3.14&3931.50&5.91&0.27&9.09&3884.33&4.73&0.00&0.00&nan&5.27&0.09&9.09&3893.00&3.50&0.12&12.50&3893.00&2.00&0.33&33.33&3906.00&1.00&0.00&0.00&nan&794.00&36.64&6.06&1764.89&34.40&0.30&2.28&2299.67&989.60&94.50&7.89&1487.41&279.40&1.40&0.21&2602.50\\ \hline
Time&CLASS&1466.54&6.88&1.22&450.35&53.91&0.18&3.14&718.00&5.91&0.27&9.09&832.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&832.00&3.50&0.12&12.50&832.00&2.00&0.33&33.33&1607.00&1.00&0.00&0.00&nan&794.00&36.64&6.06&130.69&34.40&0.30&2.28&972.00&989.60&94.50&7.89&301.65&279.40&1.40&0.21&164.08\\ \hline
Time&METHOD&1466.54&6.88&1.22&41.56&53.91&0.18&3.14&27.00&5.91&0.27&9.09&15.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&15.00&3.50&0.12&12.50&15.00&2.00&0.33&33.33&21.00&1.00&0.00&0.00&nan&794.00&36.64&6.06&62.83&34.40&0.30&2.28&70.67&989.60&94.50&7.89&102.66&279.40&1.40&0.21&64.27\\ \hline
Time&STATE&1466.54&6.88&1.22&34.30&53.91&0.18&3.14&16.00&5.91&0.27&9.09&15.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&15.00&3.50&0.12&12.50&15.00&2.00&0.33&33.33&21.00&1.00&0.00&0.00&nan&794.00&36.64&6.06&21.59&34.40&0.30&2.28&14.67&989.60&94.50&7.89&10.67&279.40&1.40&0.21&6.58\\ \hline
Chart&NORTS&784.88&5.20&2.82&1541.30&68.43&0.09&2.66&1728.00&6.58&0.16&13.16&1687.00&6.33&0.06&5.56&1816.00&5.79&0.21&21.05&1719.25&6.59&0.06&5.88&1625.00&1.00&0.90&90.00&1823.00&nan&nan&nan&nan&682.35&176.87&21.60&1670.83&48.14&1.32&10.40&1652.34&760.12&72.92&11.43&1583.94&347.04&6.58&3.93&1655.42\\ \hline
Chart&CLASS&784.88&5.20&2.82&108.85&68.43&0.09&2.66&60.50&6.58&0.16&13.16&11.33&6.33&0.06&5.56&23.00&5.79&0.21&21.05&14.25&6.59&0.06&5.88&10.00&1.00&0.90&90.00&85.78&nan&nan&nan&nan&682.35&176.87&21.60&170.66&48.14&1.32&10.40&121.11&760.12&72.92&11.43&156.20&347.04&6.58&3.93&105.15\\ \hline
Chart&METHOD&784.88&5.20&2.82&22.89&68.43&0.09&2.66&49.50&6.58&0.16&13.16&2.67&6.33&0.06&5.56&3.00&5.79&0.21&21.05&2.75&6.59&0.06&5.88&1.00&1.00&0.90&90.00&18.44&nan&nan&nan&nan&682.35&176.87&21.60&27.52&48.14&1.32&10.40&17.55&760.12&72.92&11.43&22.67&347.04&6.58&3.93&22.02\\ \hline
Chart&STATE&784.88&5.20&2.82&22.32&68.43&0.09&2.66&49.50&6.58&0.16&13.16&2.67&6.33&0.06&5.56&3.00&5.79&0.21&21.05&2.75&6.59&0.06&5.88&1.00&1.00&0.90&90.00&18.00&nan&nan&nan&nan&682.35&176.87&21.60&15.19&48.14&1.32&10.40&12.25&760.12&72.92&11.43&12.72&347.04&6.58&3.93&8.93\\ \hline
Mockito&NORTS&2307.92&8.36&1.22&444.53&nan&nan&nan&nan&3.75&0.31&26.25&845.80&4.80&0.07&1.33&548.00&4.33&0.20&20.00&980.67&4.62&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&2307.92&8.36&1.22&48.49&nan&nan&nan&nan&3.75&0.31&26.25&301.20&4.80&0.07&1.33&319.00&4.33&0.20&20.00&711.67&4.62&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&2307.92&8.36&1.22&23.61&nan&nan&nan&nan&3.75&0.31&26.25&13.40&4.80&0.07&1.33&16.00&4.33&0.20&20.00&219.33&4.62&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&2307.92&8.36&1.22&22.23&nan&nan&nan&nan&3.75&0.31&26.25&12.60&4.80&0.07&1.33&16.00&4.33&0.20&20.00&16.00&4.62&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&14725.00&63.58&3.55&3026.91&5.71&0.57&41.56&7371.44&3.94&0.05&3.55&6371.20&3.62&0.09&5.63&5283.83&3.90&0.07&6.60&6368.57&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&14725.00&63.58&3.55&1134.79&5.71&0.57&41.56&4046.13&3.94&0.05&3.55&2574.20&3.62&0.09&5.63&2176.17&3.90&0.07&6.60&2594.29&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&14725.00&63.58&3.55&457.52&5.71&0.57&41.56&773.69&3.94&0.05&3.55&43.00&3.62&0.09&5.63&92.83&3.90&0.07&6.60&38.14&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&14725.00&63.58&3.55&178.85&5.71&0.57&41.56&280.72&3.94&0.05&3.55&11.40&3.62&0.09&5.63&4.08&3.90&0.07&6.60&7.71&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&3533.06&15.52&3.09&1733.89&48.95&0.32&13.17&3456.66&6.37&0.18&10.22&2742.96&6.16&0.06&4.23&2532.50&6.08&0.18&13.85&2909.43&5.78&0.07&6.37&2382.47&1.41&0.72&70.18&2410.89&1.22&0.22&22.22&2093.00&803.65&89.77&15.98&1707.13&35.43&0.63&6.53&1945.98&931.68&69.85&10.01&1645.30&389.45&4.91&3.09&2020.26\\ \hline
All &CLASS&3533.06&15.52&3.09&311.47&48.95&0.32&13.17&1040.03&6.37&0.18&10.22&641.46&6.16&0.06&4.23&644.13&6.08&0.18&13.85&719.31&5.78&0.07&6.37&233.04&1.41&0.72&70.18&445.28&1.22&0.22&22.22&32.00&803.65&89.77&15.98&109.26&35.43&0.63&6.53&287.98&931.68&69.85&10.01&149.50&389.45&4.91&3.09&96.71\\ \hline
All &METHOD&3533.06&15.52&3.09&94.09&48.95&0.32&13.17&181.27&6.37&0.18&10.22&15.41&6.16&0.06&4.23&26.81&6.08&0.18&13.85&48.45&5.78&0.07&6.37&8.45&1.41&0.72&70.18&19.12&1.22&0.22&22.22&8.00&803.65&89.77&15.98&29.13&35.43&0.63&6.53&26.51&931.68&69.85&10.01&37.27&389.45&4.91&3.09&27.68\\ \hline
All &STATE&3533.06&15.52&3.09&45.57&48.95&0.32&13.17&79.94&6.37&0.18&10.22&8.64&6.16&0.06&4.23&7.28&6.08&0.18&13.85&8.49&5.78&0.07&6.37&5.64&1.41&0.72&70.18&17.26&1.22&0.22&22.22&1.00&803.65&89.77&15.98&12.20&35.43&0.63&6.53&8.98&931.68&69.85&10.01&9.46&389.45&4.91&3.09&6.44\\ \hline


    \end{tabular}
    \end{adjustbox}
\end{table*} 



\begin{table*}
    \centering
   \caption{Full-(StopP) Average executed tests with different \rts{} on all APR systems  }\label{table:full_nonplausible_at_summary}
   	\begin{adjustbox}{width=2.1\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}\hline
    Subjects & RTS & \prapr{}-Allp & Cp & Pr & AveT & \simfix{}-Allp & Cp & Pr & AveT  & \avatar{}-Allp & Cp & Pr & AveT & \kpar{}-Allp & Cp & Pr & AveT & \tbar{}-Allp & Cp & Pr & AveT & \fixminer{}-Allp & Cp & Pr & AveT & \dynamoth{}-Allp & Cp & Pr & AveT  & \acs{}-Allp & Cp & Pr & AveT   & \arja{}-Allp & Cp & Pr & AveT & \kali{}-Allp & Cp & Pr & AveT & \genprog{}-Allp & Cp & Pr & AveT & \rsrepair{}-Allp & Cp & Pr & AveT  \\ \hline 
    
    Lang&NORTS&376.83&0.56&4.76&1801.39&79.40&0.23&3.69&1838.09&10.63&0.22&4.82&1738.20&11.04&0.15&8.04&1707.50&10.78&0.33&13.49&1747.43&10.54&0.19&15.68&1700.20&1.43&0.71&71.43&1758.60&1.00&0.33&33.33&1822.00&830.22&15.25&16.79&1862.87&46.94&0.83&7.99&1904.38&1058.89&42.19&9.98&1869.40&468.53&3.97&6.09&1850.58\\ \hline
Lang&CLASS&376.83&0.56&4.76&76.39&79.40&0.23&3.69&45.64&10.63&0.22&4.82&56.40&11.04&0.15&8.04&80.50&10.78&0.33&13.49&76.71&10.54&0.19&15.68&66.80&1.43&0.71&71.43&35.00&1.00&0.33&33.33&49.00&830.22&15.25&16.79&92.09&46.94&0.83&7.99&38.29&1058.89&42.19&9.98&54.50&468.53&3.97&6.09&78.44\\ \hline
Lang&METHOD&376.83&0.56&4.76&14.74&79.40&0.23&3.69&7.82&10.63&0.22&4.82&13.20&11.04&0.15&8.04&16.00&10.78&0.33&13.49&10.43&10.54&0.19&15.68&13.20&1.43&0.71&71.43&3.00&1.00&0.33&33.33&1.00&830.22&15.25&16.79&7.78&46.94&0.83&7.99&7.13&1058.89&42.19&9.98&10.27&468.53&3.97&6.09&8.34\\ \hline
Lang&STATE&376.83&0.56&4.76&12.70&79.40&0.23&3.69&7.09&10.63&0.22&4.82&7.60&11.04&0.15&8.04&9.00&10.78&0.33&13.49&6.14&10.54&0.19&15.68&7.40&1.43&0.71&71.43&1.80&1.00&0.33&33.33&1.00&830.22&15.25&16.79&6.58&46.94&0.83&7.99&5.79&1058.89&42.19&9.98&7.90&468.53&3.97&6.09&4.77\\ \hline
Math&NORTS&1141.03&4.27&5.64&2782.79&35.91&0.80&15.59&2518.84&7.39&0.09&4.48&3702.80&6.48&0.06&5.20&3644.00&6.26&0.23&13.46&3343.82&6.18&0.09&7.98&2936.43&1.21&0.95&85.96&2217.33&1.67&0.33&33.33&2364.00&701.81&37.43&19.76&2698.82&10.78&0.25&7.18&3334.41&800.10&28.79&11.61&2705.20&393.51&4.49&7.50&2698.74\\ \hline
Math&CLASS&1141.03&4.27&5.64&120.57&35.91&0.80&15.59&331.84&7.39&0.09&4.48&592.20&6.48&0.06&5.20&635.80&6.26&0.23&13.46&274.12&6.18&0.09&7.98&48.29&1.21&0.95&85.96&57.06&1.67&0.33&33.33&15.00&701.81&37.43&19.76&148.34&10.78&0.25&7.18&56.29&800.10&28.79&11.61&217.75&393.51&4.49&7.50&97.94\\ \hline
Math&METHOD&1141.03&4.27&5.64&39.54&35.91&0.80&15.59&45.68&7.39&0.09&4.48&18.00&6.48&0.06&5.20&13.20&6.26&0.23&13.46&12.06&6.18&0.09&7.98&10.29&1.21&0.95&85.96&35.39&1.67&0.33&33.33&15.00&701.81&37.43&19.76&38.83&10.78&0.25&7.18&21.22&800.10&28.79&11.61&52.62&393.51&4.49&7.50&38.64\\ \hline
Math&STATE&1141.03&4.27&5.64&27.67&35.91&0.80&15.59&43.87&7.39&0.09&4.48&11.80&6.48&0.06&5.20&7.00&6.26&0.23&13.46&7.71&6.18&0.09&7.98&1.57&1.21&0.95&85.96&29.22&1.67&0.33&33.33&1.00&701.81&37.43&19.76&16.72&10.78&0.25&7.18&10.30&800.10&28.79&11.61&19.73&393.51&4.49&7.50&15.26\\ \hline
Time&NORTS&790.08&2.08&1.19&3929.41&57.11&0.22&6.02&3940.00&5.91&0.27&9.09&3893.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&3893.00&3.50&0.12&12.50&3893.00&2.00&0.33&33.33&3906.00&1.00&0.00&0.00&nan&714.90&0.90&2.00&3899.50&39.62&0.25&2.19&3899.50&885.44&49.00&9.28&3893.00&235.44&0.11&0.04&3893.00\\ \hline
Time&CLASS&790.08&2.08&1.19&1318.19&57.11&0.22&6.02&721.50&5.91&0.27&9.09&832.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&832.00&3.50&0.12&12.50&832.00&2.00&0.33&33.33&1607.00&1.00&0.00&0.00&nan&714.90&0.90&2.00&2092.50&39.62&0.25&2.19&1266.50&885.44&49.00&9.28&843.32&235.44&0.11&0.04&832.00\\ \hline
Time&METHOD&790.08&2.08&1.19&391.66&57.11&0.22&6.02&28.50&5.91&0.27&9.09&15.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&15.00&3.50&0.12&12.50&15.00&2.00&0.33&33.33&21.00&1.00&0.00&0.00&nan&714.90&0.90&2.00&170.00&39.62&0.25&2.19&218.50&885.44&49.00&9.28&326.57&235.44&0.11&0.04&298.00\\ \hline
Time&STATE&790.08&2.08&1.19&286.73&57.11&0.22&6.02&17.50&5.91&0.27&9.09&15.00&4.73&0.00&0.00&nan&5.27&0.09&9.09&15.00&3.50&0.12&12.50&15.00&2.00&0.33&33.33&21.00&1.00&0.00&0.00&nan&714.90&0.90&2.00&34.00&39.62&0.25&2.19&30.00&885.44&49.00&9.28&92.85&235.44&0.11&0.04&26.00\\ \hline
Chart&NORTS&656.40&1.00&10.22&1835.11&68.52&0.17&3.33&1782.00&6.58&0.16&13.16&1687.00&6.33&0.06&5.56&1816.00&5.79&0.21&21.05&1719.25&6.59&0.06&5.88&1625.00&1.00&0.90&90.00&1823.00&nan&nan&nan&nan&436.26&0.65&17.78&1847.71&40.50&0.50&10.04&1844.40&682.29&38.04&7.35&1837.00&239.38&0.54&6.54&1862.50\\ \hline
Chart&CLASS&656.40&1.00&10.22&140.61&68.52&0.17&3.33&215.00&6.58&0.16&13.16&11.33&6.33&0.06&5.56&23.00&5.79&0.21&21.05&14.25&6.59&0.06&5.88&10.00&1.00&0.90&90.00&85.78&nan&nan&nan&nan&436.26&0.65&17.78&195.57&40.50&0.50&10.04&134.90&682.29&38.04&7.35&185.99&239.38&0.54&6.54&161.92\\ \hline
Chart&METHOD&656.40&1.00&10.22&26.50&68.52&0.17&3.33&112.67&6.58&0.16&13.16&2.67&6.33&0.06&5.56&3.00&5.79&0.21&21.05&2.75&6.59&0.06&5.88&1.00&1.00&0.90&90.00&18.44&nan&nan&nan&nan&436.26&0.65&17.78&32.14&40.50&0.50&10.04&21.10&682.29&38.04&7.35&29.33&239.38&0.54&6.54&27.67\\ \hline
Chart&STATE&656.40&1.00&10.22&22.03&68.52&0.17&3.33&112.67&6.58&0.16&13.16&2.67&6.33&0.06&5.56&3.00&5.79&0.21&21.05&2.75&6.59&0.06&5.88&1.00&1.00&0.90&90.00&18.00&nan&nan&nan&nan&436.26&0.65&17.78&15.86&40.50&0.50&10.04&12.90&682.29&38.04&7.35&16.03&239.38&0.54&6.54&9.38\\ \hline
Mockito&NORTS&1990.14&6.22&1.33&1096.80&nan&nan&nan&nan&3.75&0.31&26.25&922.00&4.80&0.07&1.33&1102.00&4.33&0.20&20.00&980.67&4.43&0.07&3.57&1324.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&CLASS&1990.14&6.22&1.33&389.01&nan&nan&nan&nan&3.75&0.31&26.25&314.20&4.80&0.07&1.33&866.00&4.33&0.20&20.00&711.67&4.43&0.07&3.57&783.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&METHOD&1990.14&6.22&1.33&220.47&nan&nan&nan&nan&3.75&0.31&26.25&13.80&4.80&0.07&1.33&24.00&4.33&0.20&20.00&219.33&4.43&0.07&3.57&4.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Mockito&STATE&1990.14&6.22&1.33&198.49&nan&nan&nan&nan&3.75&0.31&26.25&13.00&4.80&0.07&1.33&24.00&4.33&0.20&20.00&16.00&4.43&0.07&3.57&4.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&NORTS&nan&nan&nan&nan&5.71&0.57&41.56&7371.44&3.94&0.05&3.55&7262.60&3.62&0.09&5.63&7633.00&3.90&0.07&6.60&7416.14&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&CLASS&nan&nan&nan&nan&5.71&0.57&41.56&4046.13&3.94&0.05&3.55&2897.20&3.62&0.09&5.63&2752.50&3.90&0.07&6.60&3083.43&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&METHOD&nan&nan&nan&nan&5.71&0.57&41.56&773.69&3.94&0.05&3.55&44.80&3.62&0.09&5.63&101.67&3.90&0.07&6.60&45.14&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
Closure&STATE&nan&nan&nan&nan&5.71&0.57&41.56&280.72&3.94&0.05&3.55&13.20&3.62&0.09&5.63&7.67&3.90&0.07&6.60&10.57&2.89&0.00&0.00&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan&nan\\ \hline
All &NORTS&990.90&2.82&4.63&2289.10&49.33&0.40&14.04&3490.07&6.37&0.18&10.22&3200.93&6.17&0.07&4.29&3180.50&6.06&0.19&13.95&3183.39&5.69&0.09&7.60&2295.73&1.41&0.72&70.18&2426.23&1.22&0.22&22.22&2093.00&670.80&13.56&14.08&2577.22&34.46&0.46&6.85&2745.67&856.68&39.51&9.55&2576.15&334.21&2.28&5.04&2576.21\\ \hline
All &CLASS&990.90&2.82&4.63&408.95&49.33&0.40&14.04&1072.02&6.37&0.18&10.22&783.89&6.17&0.07&4.29&871.56&6.06&0.19&13.95&832.03&5.69&0.09&7.60&348.02&1.41&0.72&70.18&446.21&1.22&0.22&22.22&32.00&670.80&13.56&14.08&632.13&34.46&0.46&6.85&374.00&856.68&39.51&9.55&325.39&334.21&2.28&5.04&292.57\\ \hline
All &METHOD&990.90&2.82&4.63&138.58&49.33&0.40&14.04&193.67&6.37&0.18&10.22&17.91&6.17&0.07&4.29&31.57&6.06&0.19&13.95&50.79&5.69&0.09&7.60&8.70&1.41&0.72&70.18&19.46&1.22&0.22&22.22&8.00&670.80&13.56&14.08&62.19&34.46&0.46&6.85&66.99&856.68&39.51&9.55&104.70&334.21&2.28&5.04&93.16\\ \hline
All &STATE&990.90&2.82&4.63&109.52&49.33&0.40&14.04&92.37&6.37&0.18&10.22&10.54&6.17&0.07&4.29&10.13&6.06&0.19&13.95&9.70&5.69&0.09&7.60&5.79&1.41&0.72&70.18&17.51&1.22&0.22&22.22&1.00&670.80&13.56&14.08&18.29&34.46&0.46&6.85&14.75&856.68&39.51&9.55&34.13&334.21&2.28&5.04&13.85\\ \hline


    
    \end{tabular}
    \end{adjustbox}
\end{table*} 

==> tables/revisit.tex <==
\begin{table}
    \centering
   \caption{Revisiting Patch Validation Strategies on  APR systems  }\label{table:revisit}
   	\begin{adjustbox}{width=1\columnwidth}
    \begin{tabular}{r|r|r|r|r|r|r|r|r} 
    \hline
    \multirow{2}{*}{Type} & \multirow{2}{*}{Tool}  & \multirow{2}{*}{Time} & \multirow{2}{*}{Paper} & \multirow{2}{*}{Code} &  \multicolumn{2}{c}{Test Selection Strategy} & \multicolumn{2}{c}{Test Prioritization Strategy} \\ \cline{6-9}
    & & & & & Fail tests & Pass tests & order & ranking criterion \\ \hline
    
    

    Template-based & \tbar{} &  & N & N &  All & All & No & No \\ \hline
    Template-based & \kpar{} &  & N & N &  All & All & No & No \\ \hline
    Template-based & \fixminer{} &  & All & All & No & No \\ \hline
    Template-based & \avatar{} &  & All & All & No & No \\ \hline
    Template-based & \prapr{} &  & ST & ST & Fail-then-pass & Test execution time \\ \hline
    
    Heuristic-based & \genprog{} &  & All & ST & Fail-then-pass  &  killed patch number \\ \hline
    Heuristic-based & \kali{} &   & All & ST & Fail-then-pass  &  killed patch number \\ \hline
    Heuristic-based & \rsrepair{} &  & All & ST & Fail-then-pass  &  killed patch number \\ \hline
    Heuristic-based & \arja{}  &   & All & ST & Fail-then-pass  &  killed patch number \\ \hline
    
    Heuristic-based & \jgenprog{} &  & All & All & No & No \\ \hline
    Heuristic-based & \jKali{}  &  & All & All & No & No \\ \hline
    Heuristic-based & \jmutrepair{}  &  & All & All & No & No \\ \hline
   
    Heuristic-based & \simfix{}  &  & All & All & No & No \\ \hline
    Heuristic-based & \capgen{}  &  & CLASS & CLASS & No & No \\ \hline
    
    Constraint-based & \acs{}  &  & All & All & No & No \\ \hline
    Constraint-based & \dynamoth{} &  & All & All & No & No \\ \hline
    Constraint-based & \cardumen{}  &  & All & All & No & No \\ \hline
    
    
    Learning-based & \coconut{}  &  & All & All & No & No \\ \hline
    Learning-based & \dlfix{}  &  & All & All & No & No \\ \hline
    Learning-based & \coconut{}  &  & All & All & No & No \\ \hline
    
    \end{tabular}
    \end{adjustbox}
\end{table} 


==> tables/rq1_HSD.tex <==
\begin{table*}
    \centering
   \caption{ANOVA analysis and Tukey’s HSD test on \ntave{} among using different \rts{} strategies on all APR systems}\label{table:all_at_HSD}
   	\begin{adjustbox}{width=2.1\columnwidth}
    \begin{tabular}{r|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr}\hline
    
    
    \multirow{2}{*}{}  & \multicolumn{4}{|c}{Lang} & \multicolumn{4}{|c}{Math} & \multicolumn{4}{|c}{Chart} & \multicolumn{4}{|c}{Time} & \multicolumn{4}{|c}{Closure} & \multicolumn{4}{|c}{Mockito} \\ \cline{2-25}
    
    APR  & No & Class & Method & State & No & Class & Method & State  & No & Class & Method & State  & No & Class & Method & State  & No & Class & Method & State  & No & Class & Method & State  \\ \hline
    
    \begin{comment}
     \multirow{3}{*}{Tool} &&&&  &&&&  &&&&   &&&&  &&&&  &&&&   \\ 
     &&&&  &&&&  &&&&   &&&&  &&&&  &&&& \\ \cline{2-25}
    &  \multicolumn{4}{|c}{\#patch=, \textit{pvalue<}}  &  \multicolumn{4}{|c}{\#patch=, \textit{pvalue<}}  &  \multicolumn{4}{|c}{\#patch=, \textit{pvalue<}}  &  \multicolumn{4}{|c}{\#patch=, \textit{pvalue<}}  &  \multicolumn{4}{|c}{\#patch=, \textit{pvalue<}}  &  \multicolumn{4}{|c}{\#patch=, \textit{pvalue<}}  \\ \hline
    \end{comment}
    


\multirow{3}{*}{PraPR}&82.89&2.16&1.30&1.15&121.61&3.57&1.29&1.12&42.81&4.58&1.33&1.32&40.63&4.50&1.24&1.18&221.41&90.36&12.64&1.87&9.97&1.46&1.28&1.28\\
&a&b&b&b&a&b&b&b&a&b&b&b&a&b&b&b&a&b&c&d&a&b&c&c\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=400.66 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=1513.39 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=784.88 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=1466.54 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=14725.00 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=2307.92 ,\textit{pvalue < 0.05}}\\ \hline
\multirow{3}{*}{SimFix}&66.79&1.96&1.22&1.19&384.69&66.56&11.41&11.04&45.64&3.54&3.06&3.06&126.87&7.44&1.85&1.18&3106.31&1662.97&321.93&123.59&nan&nan&nan&nan\\
&a&b&b&b&a&b&b&b&a&a&a&a&a&a&a&a&a&b&c&c&-&-&-&-\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=80.79 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=35.90 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=68.43 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=53.91 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=5.71 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=nan }\\ \hline
\multirow{3}{*}{AvatarFixer}&77.84&2.77&1.25&1.17&122.45&2.61&1.55&1.16&219.45&2.27&1.24&1.24&354.03&76.55&2.27&2.27&246.71&69.98&2.50&1.27&233.75&90.16&4.78&4.53\\
&a&b&b&b&a&b&b&b&a&a&a&a&a&a&a&a&a&ab&b&b&a&ab&b&b\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=10.63 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=7.39 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=6.58 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=5.91 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=3.94 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=3.75 ,\textit{pvalue < 0.05}}\\ \hline
\multirow{3}{*}{kParFixer}&127.94&7.88&1.48&1.46&212.55&40.86&1.76&1.37&101.91&2.29&1.18&1.18&1.00&1.00&1.00&1.00&343.70&142.52&7.04&1.16&8.29&5.24&1.20&1.20\\
&a&a&a&a&a&ab&b&b&a&a&a&a&a&a&a&a&a&ab&b&b&a&ab&a&a\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=11.00 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=6.48 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=6.33 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=4.73 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=3.62 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=4.80 ,\textit{pvalue > 0.05}}\\ \hline
\multirow{3}{*}{TBarFixer}&219.31&8.81&1.29&1.17&459.73&8.62&2.52&1.60&362.76&3.82&1.39&1.39&354.82&76.55&2.27&2.27&469.82&190.08&3.66&1.45&196.93&143.13&44.67&4.00\\
&a&b&b&b&a&b&b&b&a&b&b&b&a&a&a&a&a&ab&b&b&a&ab&a&a\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=10.93 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=6.26 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=5.79 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=5.27 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=3.90 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=4.33 ,\textit{pvalue > 0.05}}\\ \hline
\multirow{3}{*}{FixMiner}&197.21&8.57&1.57&1.47&229.94&3.09&1.67&1.02&96.53&1.53&1.00&1.00&487.50&104.88&2.75&2.75&1.00&1.00&1.00&1.00&1.00&1.00&1.00&1.00\\
&a&b&b&b&a&b&b&b&a&a&a&a&a&a&a&a&a&ab&a&a&a&ab&a&a\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=10.88 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=6.18 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=6.59 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=3.50 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=2.89 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=4.62 ,\textit{pvalue > 0.05}}\\ \hline
\multirow{3}{*}{Dynamoth}&1256.43&25.29&2.43&1.57&1891.11&43.46&26.24&20.93&1640.80&77.30&16.70&16.30&1302.67&536.33&7.67&7.67&nan&nan&nan&nan&nan&nan&nan&nan\\
&a&b&b&b&a&b&b&b&a&b&b&b&a&a&a&a&-&-&-&-&-&-&-&-\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=1.43 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=1.21 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=1.00 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=2.00 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=nan }&  \multicolumn{4}{|c}{\#patch=nan }\\ \hline
\multirow{3}{*}{ACS}&608.00&17.00&1.00&1.00&788.67&5.67&5.67&1.00&nan&nan&nan&nan&1.00&1.00&1.00&1.00&nan&nan&nan&nan&nan&nan&nan&nan\\
&a&a&a&a&a&ab&a&a&-&-&-&-&a&a&a&a&-&-&-&-&-&-&-&-\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=1.00 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=1.67 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=nan }&  \multicolumn{4}{|c}{\#patch=1.00 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=nan }&  \multicolumn{4}{|c}{\#patch=nan }\\ \hline
\multirow{3}{*}{Arja}&250.72&11.62&1.54&1.43&406.64&12.58&3.74&2.23&309.25&29.51&5.27&2.58&44.51&10.25&5.75&3.06&nan&nan&nan&nan&nan&nan&nan&nan\\
&a&b&b&b&a&b&c&c&a&b&c&c&a&b&bc&c&-&-&-&-&-&-&-&-\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=900.67 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=837.59 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=682.35 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=794.00 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=nan }&  \multicolumn{4}{|c}{\#patch=nan }\\ \hline
\multirow{3}{*}{Kali}&113.57&3.67&1.33&1.21&177.09&2.78&1.73&1.25&171.42&11.84&1.88&1.79&47.41&23.87&1.77&1.29&nan&nan&nan&nan&nan&nan&nan&nan\\
&a&b&b&b&a&b&b&b&a&b&b&b&a&a&a&a&-&-&-&-&-&-&-&-\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=47.69 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=11.49 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=48.14 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=34.40 ,\textit{pvalue > 0.05}}&  \multicolumn{4}{|c}{\#patch=nan }&  \multicolumn{4}{|c}{\#patch=nan }\\ \hline
\multirow{3}{*}{GenProg}&136.10&4.14&1.30&1.28&221.55&8.12&2.76&1.77&155.70&12.22&3.81&2.59&118.35&24.74&9.03&1.76&nan&nan&nan&nan&nan&nan&nan&nan\\
&a&b&b&b&a&b&c&c&a&b&b&b&a&b&c&d&-&-&-&-&-&-&-&-\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=1083.03 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=893.95 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=760.12 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=989.60 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=nan }&  \multicolumn{4}{|c}{\#patch=nan }\\ \hline
\multirow{3}{*}{RSRepair}&71.01&2.14&1.20&1.08&113.12&3.07&1.62&1.10&52.81&3.87&1.39&1.26&4.52&1.53&1.20&1.02&nan&nan&nan&nan&nan&nan&nan&nan\\
&a&b&b&b&a&b&b&b&a&b&b&b&a&b&b&b&-&-&-&-&-&-&-&-\\ \cline{2-25}
&  \multicolumn{4}{|c}{\#patch=498.11 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=433.24 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=347.04 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=279.40 ,\textit{pvalue < 0.05}}&  \multicolumn{4}{|c}{\#patch=nan }&  \multicolumn{4}{|c}{\#patch=nan }\\ \hline

    
    
    
    \end{tabular}
    \end{adjustbox}
\end{table*} 


==> tables/rq1_wilcox.tex <==

\begin{table*}
    \centering
   \caption{Wilcox rank analysis on \ntacc{} among using different \rts{} strategies on all APR systems}\label{table:all_allt_wilcox}
   \begin{threeparttable}
   	\begin{adjustbox}{width=2.1\columnwidth}
    \begin{tabular}{r|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr}\hline
    %p{1.4cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.9cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.9cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}|p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}p{0.02cm}p{0.8cm}
      \multirow{2}{*}{}  & \multicolumn{4}{|c}{Lang} & \multicolumn{4}{|c}{Math} & \multicolumn{4}{|c}{Chart} & \multicolumn{4}{|c}{Time} & \multicolumn{4}{|c}{Closure} & \multicolumn{4}{|c}{Mockito} \\ \cline{2-25}
    
    APR  & No & Class & Method & State  & No & Class & Method & State  & No & Class & Method & State  & No & Class & Method & State  & No & Class & Method & State  & No & Class & Method & State  \\ \hline
    
\multirow{2}{*}{PraPR}&2117.61&447.31&414.15&412.59&11879.77&1711.16&1573.21&1557.41&5517.96&1053.80&868.24&863.96&7782.19&2513.88&1848.62&1808.12&86651.19&47374.48&28476.71&21825.07&3753.19&2857.81&2555.61&2547.64\\
&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}\\ \hline
\multirow{2}{*}{SimFix}&424.75&85.96&82.38&82.21&1185.13&158.06&56.41&55.59&218.61&73.61&72.65&72.65&768.55&184.27&58.64&56.64&4239.84&2329.55&449.64&166.45&-&-&-&-\\
&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&.&.&.&\\ \hline
\multirow{2}{*}{AvatarFixer}&321.41&19.48&12.11&11.44&168.78&12.92&8.20&7.81&272.84&8.26&6.89&6.89&1065.00&232.55&9.73&9.73&342.78&140.81&6.17&4.49&267.75&97.56&7.62&7.38\\
&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&\\ \hline
\multirow{2}{*}{kParFixer}&163.19&18.30&11.89&11.59&237.05&46.66&7.25&6.86&107.61&8.00&6.89&6.89&4.73&4.73&4.73&4.73&378.73&154.94&9.90&3.92&41.27&26.00&5.80&5.80\\
&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&.&.&.&&\cellcolor{ggray}>&\cellcolor{ggray}$\thickapprox{}$&\cellcolor{ggray}$\thickapprox{}$&\cellcolor{ggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&\\ \hline
\multirow{2}{*}{TBarFixer}&437.52&24.63&12.63&11.96&640.65&34.66&8.18&7.25&367.74&8.79&6.37&6.37&359.09&80.82&6.55&6.55&478.09&197.02&6.67&4.40&200.27&146.47&48.00&7.33\\
&\cellcolor{ggray}>&\cellcolor{ggray}$\thickapprox{}$&\cellcolor{ggray}$\thickapprox{}$&\cellcolor{ggray}&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&\\ \hline
\multirow{2}{*}{FixMiner}&233.15&18.88&11.88&11.50&239.38&9.47&7.03&6.23&102.12&7.12&6.59&6.59&490.00&107.38&5.25&5.25&2.89&2.89&2.89&2.89&4.62&4.62&4.62&4.62\\
&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&.&.&.&&.&.&.&\\ \hline
\multirow{2}{*}{Dynamoth}&1256.86&25.71&2.86&2.00&2042.74&50.79&32.53&27.00&1640.80&77.30&16.70&16.30&1303.67&537.33&8.67&8.67&-&-&-&-&-&-&-&-\\
&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&.&.&.&&.&.&.&\\ \hline
\multirow{2}{*}{ACS}&608.00&17.00&1.00&1.00&789.33&6.33&6.33&1.67&-&-&-&-&1.00&1.00&1.00&1.00&-&-&-&-&-&-&-&-\\
&.&.&.&&.&.&.&&.&.&.&&.&.&.&&.&.&.&&.&.&.&\\ \hline
\multirow{2}{*}{Arja}&68448.64&1571.25&1196.83&1176.53&104804.90&4828.21&2105.64&1382.11&202236.87&27627.48&6853.48&2356.57&34310.82&7337.91&3822.82&1781.91&-&-&-&-&-&-&-&-\\
&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&.&.&.&&.&.&.&\\ \hline
\multirow{2}{*}{Kali}&799.43&59.54&51.54&50.63&705.64&22.00&15.97&14.10&2035.27&133.45&61.45&56.82&724.00&325.70&55.30&38.50&-&-&-&-&-&-&-&-\\
&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&.&.&.&&.&.&.&\\ \hline
\multirow{2}{*}{GenProg}&86910.25&2746.19&1376.81&1369.64&73174.10&5231.08&1610.38&1419.85&104090.08&5694.38&2645.12&1746.42&141456.00&29401.40&10596.50&1903.60&-&-&-&-&-&-&-&-\\
&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&.&.&.&&.&.&.&\\ \hline
\multirow{2}{*}{RSRepair}&10945.44&620.69&556.39&534.58&9661.55&828.93&498.28&463.63&9552.46&758.38&450.67&386.71&2652.50&635.00&413.90&291.50&-&-&-&-&-&-&-&-\\
&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}>&\cellcolor{ggggray}&\cellcolor{gggray}>&\cellcolor{gggray}>&\cellcolor{gggray}$\thickapprox{}$&\cellcolor{gggray}&$\thickapprox{}$&$\thickapprox{}$&$\thickapprox{}$&&.&.&.&&.&.&.&\\ \hline



    \end{tabular}
    \end{adjustbox}
    
    \begin{tablenotes}
        \footnotesize
       \item ``$>$'': significant greater ($ p < 0.05$).  ``$\thickapprox{}$'': no significant difference ($ p > 0.05$).  ``.'': invalid sample for statistical analysis. ``-'': no generated patch.
      \end{tablenotes}
    \end{threeparttable}


\end{table*} 


==> tables/rq2_codeelements.tex <==

\begin{table*}
    \centering
    \caption{The scale of code elements modified by different APR system}\label{table:codelements}
   	\begin{adjustbox}{width=2\columnwidth}
    \begin{tabular}{r|rrr|rrr|rrr|rrr|rrr|rrr}\hline
    
    \multirow{2}{*}{}  & \multicolumn{3}{|c}{Lang} & \multicolumn{3}{|c|}{Math} & \multicolumn{3}{|c}{Chart} & \multicolumn{3}{|c}{Time} & \multicolumn{3}{|c}{Closure} & \multicolumn{3}{|c}{Mockito} \\ \cline{2-19}
    
    APR & Class & Method & State & Class & Method & State & Class & Method & State & Class & Method & State & Class & Method & State & Class & Method & State \\ \hline
    
    
    PraPR&291.52&28.69&1.00&474.72&37.06&1.00&361.07&28.16&1.00&137.74&7.00&1.00&395.33&33.14&1.00&32.01&6.39&1.00\\ \hline
SimFix&353.22&34.53&7.91&303.64&21.30&5.85&328.86&27.88&7.32&156.10&10.06&5.49&480.70&24.63&4.74&-&-&-\\ \hline
AvatarFixer&271.25&21.66&1.00&246.45&17.40&1.00&315.97&16.27&1.00&216.98&10.57&1.00&482.66&37.36&1.00&46.57&6.10&1.00\\ \hline
kParFixer&274.12&20.84&1.00&250.93&20.64&1.00&354.25&18.89&1.00&215.27&9.94&1.00&539.37&40.47&1.00&44.58&5.35&1.00\\ \hline
TBarFixer&287.58&18.76&1.00&253.96&16.73&1.00&333.17&20.25&1.00&222.28&11.05&1.00&554.21&31.82&1.00&42.62&5.63&1.00\\ \hline
FixMiner&293.06&20.82&1.00&275.35&20.65&1.00&335.64&23.03&1.00&138.82&13.25&1.00&138.44&9.31&1.00&47.62&5.58&1.00\\ \hline
Dynamoth&232.40&44.70&1.00&115.26&26.04&1.00&335.40&24.60&1.00&240.83&8.17&1.00&-&-&-&-&-&-\\ \hline
ACS&373.67&48.67&1.00&222.40&25.20&1.00&-&-&-&44.00&3.00&1.00&-&-&-&-&-&-\\ \hline
Arja&273.62&31.77&1.80&222.75&31.88&1.79&241.09&19.11&1.88&267.13&11.11&1.86&-&-&-&-&-&-\\ \hline
Kali&273.04&35.14&1.00&210.33&19.79&1.00&328.08&21.26&1.00&125.44&5.33&1.00&-&-&-&-&-&-\\ \hline
GenProg&321.01&31.82&2.71&272.65&36.76&3.89&341.73&28.77&4.34&245.68&12.05&1.89&-&-&-&-&-&-\\ \hline
RSRepair&263.51&26.24&1.09&205.89&24.10&1.21&376.53&18.94&1.22&139.39&6.81&1.10&-&-&-&-&-&-\\ \hline



    \end{tabular}
    \end{adjustbox}
    

\end{table*} 

==> tables/rq2_fullmatrix.tex <==

\begin{table*}
    \centering
   \caption{\ntave{} with test execution strategies based on partial and full matrix on all APR systems}\label{table:full_avet}
   	\begin{adjustbox}{width=2\columnwidth}
    \begin{tabular}{r|r|rrrr|rrrr|rrrr|rrrr|rrrr|rrrr}\hline

      \multirow{2}{*}{APR}  & \multirow{2}{*}{matrix} & \multicolumn{4}{|c}{Lang} & \multicolumn{4}{|c}{Math} & \multicolumn{4}{|c}{Chart} & \multicolumn{4}{|c}{Time} & \multicolumn{4}{|c}{Closure} & \multicolumn{4}{|c}{Mockito} \\ \cline{3-26}
    
      & & No & Class & Method & State & No & Class & Method & State & No & Class & Method & State & No & Class & Method & State & No & Class & Method & State & No & Class & Method & State  \\ \hline
     
    \multirow{2}{*}{PraPR} & Partial&82.89&2.16&1.30&1.15&121.61&3.57&1.29&1.12&42.81&4.58&1.33&1.32&40.63&4.50&1.24&1.18&221.41&90.36&12.64&1.87&9.97&1.46&1.28&1.28\\
& Full&1866.29&73.87&15.10&13.87&2831.06&285.36&84.23&75.80&1829.28&116.94&62.70&59.24&3923.62&1192.97&451.33&414.75&7128.70&4141.04&2972.53&2642.84&1128.64&696.64&585.91&571.31\\ \hline
\multirow{2}{*}{SimFix} & Partial&66.79&1.96&1.22&1.19&384.69&66.56&11.41&11.04&45.64&3.54&3.06&3.06&126.87&7.44&1.85&1.18&3106.31&1662.97&321.93&123.59&-&-&-&-\\
& Full&1854.58&63.14&11.11&9.83&2818.73&366.12&60.91&48.09&1835.39&108.38&49.27&48.34&3920.18&1722.05&50.28&42.58&7246.80&4213.12&728.99&264.72&-&-&-&-\\ \hline
\multirow{2}{*}{AvatarFixer} & Partial&77.84&2.77&1.25&1.17&122.45&2.61&1.55&1.16&219.45&2.27&1.24&1.24&354.03&76.55&2.27&2.27&246.71&69.98&2.50&1.27&233.75&90.16&4.78&4.53\\
& Full&1793.33&52.35&6.60&4.18&2798.84&188.06&21.55&9.08&1853.63&83.89&11.89&6.14&3940.27&1248.93&90.36&9.46&7133.26&3749.01&2062.22&1076.41&1005.31&394.65&182.91&15.80\\ \hline
\multirow{2}{*}{kParFixer} & Partial&127.94&7.88&1.48&1.46&212.55&40.86&1.76&1.37&101.91&2.29&1.18&1.18&1.00&1.00&1.00&1.00&343.70&142.52&7.04&1.16&8.29&5.24&1.20&1.20\\
& Full&1801.89&54.13&7.05&4.97&2843.87&233.53&26.61&12.44&1866.33&69.61&12.54&7.06&3941.36&879.82&45.18&10.70&7200.68&4075.31&2112.97&993.20&1048.20&345.37&164.89&27.59\\ \hline
\multirow{2}{*}{TBarFixer} & Partial&219.31&8.81&1.29&1.17&459.73&8.62&2.52&1.60&362.76&3.82&1.39&1.39&354.82&76.55&2.27&2.27&469.82&190.08&3.66&1.45&196.93&143.13&44.67&4.00\\
& Full&1793.33&52.93&6.03&4.28&2786.79&180.81&24.20&7.82&1853.63&71.64&12.33&6.08&3940.27&1059.98&47.56&6.32&7178.36&4147.67&2137.47&924.81&1018.73&427.13&194.85&16.37\\ \hline
\multirow{2}{*}{FixMiner} & Partial&197.21&8.57&1.57&1.47&229.94&3.09&1.67&1.02&96.53&1.53&1.00&1.00&487.50&104.88&2.75&2.75&1.00&1.00&1.00&1.00&1.00&1.00&1.00&1.00\\
& Full&1796.54&55.77&6.40&4.10&2738.60&249.40&25.45&9.92&1873.88&68.01&13.83&6.34&3919.38&733.62&61.62&8.75&7502.06&3419.44&685.57&134.63&1070.31&342.70&126.69&15.68\\ \hline
\multirow{2}{*}{Dynamoth} & Partial&1256.43&25.29&2.43&1.57&1891.11&43.46&26.24&20.93&1640.80&77.30&16.70&16.30&1302.67&536.33&7.67&7.67&-&-&-&-&-&-&-&-\\
& Full&1753.57&37.00&9.57&6.86&2211.26&75.92&34.58&25.91&1805.70&105.00&25.00&24.60&3888.33&1869.33&166.00&163.67&-&-&-&-&-&-&-&-\\ \hline
\multirow{2}{*}{ACS} & Partial&608.00&17.00&1.00&1.00&788.67&5.67&5.67&1.00&-&-&-&-&1.00&1.00&1.00&1.00&-&-&-&-&-&-&-&-\\
& Full&2133.00&69.33&6.00&4.00&2314.33&198.67&89.00&39.67&-&-&-&-&4041.00&139.00&7.00&7.00&-&-&-&-&-&-&-&-\\ \hline
\multirow{2}{*}{Arja} & Partial&250.72&11.62&1.54&1.43&406.64&12.58&3.74&2.23&309.25&29.51&5.27&2.58&44.51&10.25&5.75&3.06&-&-&-&-&-&-&-&-\\
& Full&1942.56&69.94&10.70&8.94&2783.79&137.15&34.60&20.00&1830.78&128.65&24.28&17.43&3878.82&1672.84&475.43&408.40&-&-&-&-&-&-&-&-\\ \hline
\multirow{2}{*}{Kali} & Partial&113.57&3.67&1.33&1.21&177.09&2.78&1.73&1.25&171.42&11.84&1.88&1.79&47.41&23.87&1.77&1.29&-&-&-&-&-&-&-&-\\
& Full&1944.46&65.31&10.81&9.43&2761.57&123.27&24.80&14.34&1835.32&103.64&33.92&30.65&3882.10&1300.98&333.33&314.29&-&-&-&-&-&-&-&-\\ \hline
\multirow{2}{*}{GenProg} & Partial&136.10&4.14&1.30&1.28&221.55&8.12&2.76&1.77&155.70&12.22&3.81&2.59&118.35&24.74&9.03&1.76&-&-&-&-&-&-&-&-\\
& Full&1942.56&69.51&11.01&8.70&2768.45&189.59&37.93&21.06&1829.83&140.35&38.44&24.69&3882.10&1622.07&457.41&407.29&-&-&-&-&-&-&-&-\\ \hline
\multirow{2}{*}{RSRepair} & Partial&71.01&2.14&1.20&1.08&113.12&3.07&1.62&1.10&52.81&3.87&1.39&1.26&4.52&1.53&1.20&1.02&-&-&-&-&-&-&-&-\\
& Full&1942.56&67.02&10.12&8.28&2775.49&136.13&29.53&17.05&1829.83&118.19&36.05&25.73&3882.10&1427.10&355.66&326.74&-&-&-&-&-&-&-&-\\ \hline

    
    
    \end{tabular}
    \end{adjustbox}
    



\end{table*} 


==> tables/rq2_patchratio.tex <==

\begin{table*}
    \centering
   \caption{The ratio of different patch categories on all APR systems}\label{tab:patch_ratio}
   
   	\begin{adjustbox}{width=2.1\columnwidth}
    \begin{tabular}{r|rrr|rrr|rrr|rrr|rrr|rrr}\hline
    
    \multirow{2}{*}{}  & \multicolumn{3}{|c}{Lang} & \multicolumn{3}{|c}{Math} & \multicolumn{3}{|c}{Chart} & \multicolumn{3}{|c}{Time} & \multicolumn{3}{|c}{Closure} & \multicolumn{3}{|c}{Mockito} \\ \cline{2-19}
    
    APR & \stopfpatch{} \% & \stopppatch{} \%& \plausiblepatch{}\%  & \stopfpatch{} \% & \stopppatch{} \%& \plausiblepatch{}\%  & \stopfpatch{} \% & \stopppatch{} \%& \plausiblepatch{}\%  & \stopfpatch{} \% & \stopppatch{} \%& \plausiblepatch{}\%  & \stopfpatch{} \% & \stopppatch{} \%& \plausiblepatch{}\%  & \stopfpatch{} \% & \stopppatch{} \%& \plausiblepatch{}\% \\ \hline
    
    
PraPR&95.32&0.31&4.37&94.92&1.53&3.55&98.78&0.29&0.93&97.18&0.74&2.07&98.78&0.33&0.89&96.45&0.85&2.70\\ \hline
SimFix&96.38&0.00&3.62&85.13&1.02&13.85&96.86&0.11&3.03&97.34&0.00&2.66&-&-&-&58.44&0.00&41.56\\ \hline
AvatarFixer&95.18&0.53&4.29&95.52&0.69&3.80&90.91&6.06&3.03&86.84&0.00&13.16&73.75&1.25&25.00&96.45&0.35&3.19\\ \hline
kParFixer&92.33&0.26&7.41&94.80&0.00&5.20&100.00&0.00&0.00&94.44&0.00&5.56&98.67&1.33&0.00&94.37&1.19&4.44\\ \hline
TBarFixer&87.13&1.35&11.52&86.54&1.17&12.29&90.91&0.00&9.09&78.95&0.00&21.05&80.00&0.00&20.00&93.40&0.21&6.38\\ \hline
FixMiner&88.17&0.30&11.54&92.02&0.19&7.79&87.50&0.00&12.50&94.12&0.00&5.88&100.00&0.00&0.00&100.00&0.00&0.00\\ \hline
Dynamoth&28.57&0.00&71.43&14.04&7.02&78.95&66.67&0.00&33.33&10.00&0.00&90.00&-&-&-&-&-&-\\ \hline
ACS&66.67&0.00&33.33&66.67&0.00&33.33&100.00&0.00&0.00&-&-&-&-&-&-&-&-&-\\ \hline
Arja&84.40&5.60&10.00&79.35&9.28&11.38&93.94&6.06&0.00&78.40&11.94&9.66&-&-&-&-&-&-\\ \hline
Kali&93.24&0.75&6.01&93.33&2.30&4.37&97.72&1.75&0.53&89.60&1.37&9.03&-&-&-&-&-&-\\ \hline
GenProg&90.65&5.54&3.81&88.62&6.23&5.15&92.11&7.89&0.00&88.57&9.84&1.59&-&-&-&-&-&-\\ \hline
RSRepair&95.93&0.82&3.25&95.84&1.45&2.71&99.79&0.21&0.00&96.07&2.12&1.81&-&-&-&-&-&-\\ \hline

    
    
    
    
    \end{tabular}
    \end{adjustbox}
    

\end{table*} 

==> tables/rq3_ourtool.tex <==
\begin{table*}
    \centering
    \caption{\ntacc{} of \ourtool{}on different APR system}\label{table:ourtool}
   	\begin{adjustbox}{width=2\columnwidth}
    \begin{tabular}{r|rrr|rrr|rrr|rrr|rrr|rrr}\hline
    
    \multirow{2}{*}{}  & \multicolumn{3}{|c}{Lang} & \multicolumn{3}{|c|}{Math} & \multicolumn{3}{|c}{Chart} & \multicolumn{3}{|c}{Time} & \multicolumn{3}{|c}{Closure} & \multicolumn{3}{|c}{Mockito} \\ \cline{2-19}
    
    APR & \rtsstate{} & \trp{} & \ourtool{}& \rtsstate{} & \trp{} & \ourtool{} & \rtsstate{} & \trp{} & \ourtool{}& \rtsstate{} & \trp{} & \ourtool{}& \rtsstate{} & \trp{} & \ourtool{}& \rtsstate{} & \trp{} & \ourtool{}\\ \hline
    
    PraPR&412.59&981.80&407.68&1557.41&3131.23&1567.53&863.96&1942.60&812.00&1808.12&3085.38&1615.73&21825.07&21602.46&16519.87&2547.64&2591.31&2436.61\\ \hline
SimFix&82.21&424.75&82.21&55.59&891.87&51.64&72.65&218.61&72.65&56.64&420.09&54.55&166.45&4239.84&166.45&-&-&-\\ \hline
AvatarFixer&11.44&303.15&11.41&7.81&221.01&7.89&6.89&272.84&6.89&9.73&362.18&8.45&4.49&335.05&4.17&7.38&229.31&7.31\\ \hline
kParFixer&11.59&172.07&11.67&6.86&237.05&6.86&6.89&107.61&6.89&4.73&4.73&4.73&3.92&519.16&3.93&5.80&41.60&5.20\\ \hline
TBarFixer&11.96&314.67&11.78&7.25&646.88&7.21&6.37&367.74&6.37&6.55&359.09&6.55&4.40&549.40&4.56&7.33&200.27&7.33\\ \hline
FixMiner&11.50&242.38&11.58&6.23&268.10&6.22&6.59&102.12&6.59&5.25&490.00&5.25&2.89&2.89&2.89&4.62&4.62&4.62\\ \hline
Dynamoth&2.00&1256.86&2.00&27.00&1972.53&23.95&16.30&1640.80&16.30&8.67&1303.67&8.67&-&-&-&-&-&-\\ \hline
ACS&1.00&608.00&1.00&1.67&789.33&1.67&-&-&-&1.00&1.00&1.00&-&-&-&-&-&-\\ \hline
Arja&1176.53&1592.25&1107.03&1382.11&1797.17&1037.68&2356.57&1863.78&1236.70&1781.91&997.18&1232.36&-&-&-&-&-&-\\ \hline
Kali&50.63&319.49&49.63&14.10&516.72&13.31&56.82&600.00&53.50&38.50&520.20&39.10&-&-&-&-&-&-\\ \hline
GenProg&1369.64&1449.78&1215.75&1419.85&1665.65&1024.15&1746.42&1351.29&1074.75&1903.60&1651.50&2425.90&-&-&-&-&-&-\\ \hline
RSRepair&534.58&935.56&519.14&463.63&1232.83&455.65&386.71&982.25&369.71&291.50&296.90&302.30&-&-&-&-&-&-\\ \hline


    \end{tabular}
    \end{adjustbox}
    

\end{table*} 

==> tables/rq4_timecost.tex <==

\begin{table*}
    \centering
    \caption{Time cost with different \rts{} strategies on different APR system}\label{table:time}
   	\begin{adjustbox}{width=2\columnwidth}
    \begin{tabular}{r|rrr|rrr|rrr|rrr|rrr|rrr}\hline
    
    \multirow{2}{*}{}  & \multicolumn{3}{|c}{Lang} & \multicolumn{3}{|c|}{Math} & \multicolumn{3}{|c}{Chart} & \multicolumn{3}{|c}{Time} & \multicolumn{3}{|c}{Closure} & \multicolumn{3}{|c}{Mockito} \\ \cline{2-19}
    
    APR & Class & Method & State & Class & Method & State & Class & Method & State & Class & Method & State & Class & Method & State & Class & Method & State \\ \hline

    \end{tabular}
    \end{adjustbox}
    

\end{table*} 

==> tables/subInfo.tex <==

\begin{table}
	\centering
	\small
	\caption{Benchmark statistics}\label{table:subinfo}
	
	\begin{adjustbox}{width=0.8\columnwidth}
	   	
	\begin{tabular}{|l|l|l|l|l|}
		\hline
        \textbf{ID} & \textbf{Name}&\textbf{\#Bug} & \textbf{\#Test} &\textbf{LoC}\\ \hline\hline
        
        
	    Lang & Apache commons-lang & 65 & 2,245 & 22K \\ 
	    Math & Apache commons-math & 106 & 3,602 & 85K \\ 
	    Time & Joda-Time & 27 & 4,130 & 28K \\ 
	    Chart & JFreeChart & 26 & 2,205 & 96K \\ 
	    Closure & Google Closure compiler & 133 & 7,927 & 90K \\ 
	    Mockito & Mockito framework & 38 & 1,366 & 23K \\ \hline \hline
	    
	   \multicolumn{2}{|c|}{\textbf{\olddefects{}}} & \textbf{395} & \textbf{21,475} & \textbf{344K}\\
		\hline
	\end{tabular}
	\end{adjustbox}
\end{table}





\begin{table}
    \small
    \centering
    \caption{APR systems studied}\label{tab:aprtools}
    	\begin{adjustbox}{width=0.8\columnwidth}
    \begin{tabular}{|l|l|}
        \cline{1-2}
         \textbf{Tool Category} & \textbf{Tools} \\
         \hline \hline
         Constraint-based & \acs{}, \cardumen{}, \dynamoth{} \\          \hline
         Heuristic-based &  \tabincell{l}{\arja, \genprog{}, \kali{}, \simfix{}} \\          \hline
         Template-based & \avatar{}, \fixminer{}, \kpar{}, \prapr{}, \tbar{} \\
                  \hline
    \end{tabular}
    	\end{adjustbox}
\end{table}





